Divide and Conquer Dynamic Programming: An Almost Linear Time Change Point Detection Methodology in High Dimensions

We develop a novel, general and computationally efficient framework, called Divide and Conquer Dynamic Programming (DCDP), for localizing change points in time series data with high-dimensional features. DCDP deploys a class of greedy algorithms that are applicable to a broad variety of high-dimensional statistical models and can enjoy almost linear computational complexity. We investigate the performance of DCDP in three commonly studied change point settings in high dimensions: the mean model, the Gaussian graphical model, and the linear regression model. In all three cases, we derive non-asymptotic bounds for the accuracy of the DCDP change point estimators. We demonstrate that the DCDP procedures consistently estimate the change points with sharp, and in some cases, optimal rates while incurring significantly smaller computational costs than the best available algorithms. Our findings are supported by extensive numerical experiments on both synthetic and real data.

==> 00_overview.tex <==
\section{Overview}
About DCDP:
\begin{enumerate}
    \item DCDP works well with a relatively large parameter $\gamma = C_{\gamma}K\tr\kappa^2$.
    \item Local refinement works well both in theory and in practice, though it is not quite ``novel". Is it good to go? Or should we think about something else?
    \item Next step: consider generalizing to nonlinear models like logistic regression.
    \item Piece-wise linear signals?
\end{enumerate}

About CPD for logistic regression and the Bradley-Terry model:
\begin{enumerate}
    \item Given that the WBS based on loglikelihood performs well in practice, should we try proving some theory for it?
\end{enumerate}


improvement in the computation

compare with others


==> 999_backup_experiment_random_grid.tex <==
\clearpage
\subsection{Results with random grid points}



\begin{table}[h]
 \centering
%  \begin{tabular}{m{2cm}m{2cm}m{2cm}C{1.5cm}C{1.5cm}C{1.5cm}}
%  \begin{tabular}{m{3.6cm}m{2cm}m{2cm}m{2cm}C{1.5cm}C{1.5cm}C{1.5cm}}
 \begin{tabular}{l l l l l l l}
  \hline
 Setting & Method & $H(\hat{\eta},\eta)$ & Time & $\hat{K}<K$ &$\hat{K}=K$ &$\hat{K}>K$
 \\
 \hline
 \multirow{1}{5cm}{$n = 200, p=20, K =3, \delta = 5$} 
 & DCDP & 0.00 (0.00) & 0.7s (0.1) & 0 & 100 & 0 \\
 \hline
 \multirow{1}{5cm}{$n = 200, p=20, K =3, \delta = 1$} 
 & DCDP & 0.51 (0.77) & 0.7s (0.1) & 0 & 100 & 0 \\
 \hline
 \multirow{1}{5cm}{$n = 200, p=20, K =3, \delta = 0.5$} 
 & DCDP & 16.54 (10.33) & 0.2s (0.0) & 10 & 87 & 3 \\
 \hline
 \multirow{1}{5cm}{$n = 200, p=100, K =3, \delta = 5$} 
 & DCDP & 0.0 (0.0) & 0.6s (0.1) & 0 & 100 & 0 \\
 \hline
 \multirow{1}{5cm}{$n = 200, p=100, K =3, \delta = 1$} 
 & DCDP & 0.82 (0.88) & 0.9s (0.1) & 0 & 100 & 0 \\
 \hline
 \multirow{1}{5cm}{$n = 800, p=100, K =3, \delta = 0.5$} 
 & DCDP &  60.78 (31.08) &  2.0s (0.1) & 5  &  95 & 0 \\
 \hline
 \end{tabular}
 \caption{Comparison of DCDP and other methods under the mean model with different simulation settings. 100 trials are conducted in each setting. }
 % \label{tab:mean compare_methods full}
\end{table}






















\begin{table}[H]
 \centering
%  \begin{tabular}{m{2cm}m{2cm}m{2cm}C{1.5cm}C{1.5cm}C{1.5cm}}
%  \begin{tabular}{C{4cm}C{2cm}C{2cm}C{2cm}C{1cm}C{1cm}C{1cm}}
\begin{tabular}{l l l l l l l}
  \hline
 Setting & Method & $H(\hat{\eta},\eta)$ & Time & $\hat{K}<K$ &$\hat{K}=K$ &$\hat{K}>K$
 \\
 \hline
 \multirow{1}{5cm}{$n = 200, p=20, K =3, \delta = 5$} 
 & DCDP & 0.03 (0.17) & 2.4s (0.1) & 0 & 100 & 0 \\
 \hline
 \multirow{1}{5cm}{$n = 200, p=20, K =3, \delta = 1$} 
 & DCDP & 1.57 (7.90) & 2.2s (0.1) & 3 & 97 & 0 \\
 \hline
 \multirow{1}{5cm}{$n = 200, p=100, K =3, \delta = 5$} 
 & DCDP & 0.12 (0.38) & 14.1s (0.5) & 0 & 100 & 0 \\
 \hline
 \multirow{1}{5cm}{$n = 200, p=100, K =3, \delta = 1$} 
 & DCDP & 2.20 (10.10) & 5.7s (0.2) & 4 & 96 & 0 \\
 \hline
 \end{tabular}
 \caption{Comparison of DCDP and other methods under the linear model with different simulation settings. 100 trials are conducted in each setting. }
 % \label{tab:linear compare_methods full}
\end{table}







\begin{table}[h]
 \centering
%  \begin{tabular}{m{2cm}m{2cm}m{2cm}C{1.5cm}C{1.5cm}C{1.5cm}}
%  \begin{tabular}{C{4cm}C{2cm}C{2cm}C{2cm}C{1cm}C{1cm}C{1cm}}
\begin{tabular}{l l l l l l l}
  \hline
 Setting & Method & $H(\hat{\eta},\eta)$ & Time & $\hat{K}<K$ &$\hat{K}=K$ &$\hat{K}>K$
 \\
 \hline
 \multirow{1}{7cm}{$n = 2000, p=5, K =3, \delta_1 = 2,\delta_2 = 0.3$} 
 & DCDP & 5.10 (6.22) &  0.9s (0.2) & 0 & 100 & 0 \\
 \hline
 \multirow{1}{7cm}{$n = 2000, p=10, K =3, \delta_1 = 5,\delta_2 = 0.3$} 
 & DCDP & 0.27 (0.49) & 1.1s (0.1) & 0 & 100 & 0 \\
 \hline
 \multirow{1}{7cm}{$n = 2000, p=20, K =3, \delta_1 = 5,\delta_2 = 0.3$} 
 & DCDP & 0.03 (0.17) & 2.5s (0.3) & 0 & 100 & 0 \\
 \hline
 \multirow{1}{7cm}{$n = 400, p=10, K =3, \delta_1 = 5,\delta_2 = 0.3$} 
 & DCDP & 0.38 (0.60) & 0.6s (0.1) & 0& 100& 0 \\
 \hline
 \multirow{1}{7cm}{$n = 400, p=20, K =3, \delta_1 = 5,\delta_2 = 0.3$} 
 & DCDP & 0.68 (5.07) & 0.9s (0.1) & 0 & 100 & 0 \\
 \hline
 \end{tabular}
 \caption{Comparison of DCDP and other methods under the covariance model with different simulation settings. 100 trials are conducted in each setting. }
 % \label{tab:covariance compare_methods full}
\end{table}



==> backup_version/00_overview.tex <==
\section{Overview}
About DCDP:
\begin{enumerate}
    \item DCDP works well with a relatively large parameter $\gamma = C_{\gamma}K\tr\kappa^2$.
    \item Local refinement works well both in theory and in practice, though it is not quite ``novel". Is it good to go? Or should we think about something else?
    \item Next step: consider generalizaing to nonlinear models like logistic regression.
    \item Piece-wise linear signals?
\end{enumerate}

About CPD for logistic regression and Bradley-Terry model:
\begin{enumerate}
    \item Given that the WBS based on loglikelihood performs well in practice, should we try proving some theory for it?
\end{enumerate}


improvement in the computation

compare with others


==> backup_version/01_introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Change point detection is a classical problem in statistics that can date back to 1940s \citep{wald1945, page1954}. In 1980s people established asymptotic theory for change point detection methods \citep{vostrikova1981,james1987,yao_au1989}. Most of these classical papers study the univariate mean model. Recently with more advanced theoretical tools developed in modern statistics, more delicate analysis of change point detection came out in univariate mean models \citep{wang2018univariate}, in high-dimensional mean models \citep{cho2015,jirak2015,aston2018,wang_samworth2018}, in covariance models \citep{aue2009, avanesov2018, wang_yi_rinaldo_2021_cov}, in high-dimensional regression models \citep{rinaldo2021cpd_reg_aistats, wang2021_jmlr}, in network models \citep{wang2021network_cpd}, and in temporally-correlated times series \citep{lavielle2000, davis2006, aue2009, wang2020sepp}.

Suppose we observe $Z_t$ at time $t$ for $t\in [T]$ and all observations are independent. Each $Z_t$ follows the same family of distribution $\mathbb{P}(\theta_t)$ where $\theta_t$ is a parameter that can change over time. We are interested in capturing abrupt changes in the distributions and equivalently in the parameters. Towards that goal, we assume that there is a collection of change points $ 0=\eta_0 <  \eta_1  < \eta_2 < \ldots <\eta_K < \eta _{K+1}= n  $ such that $\theta_{t}\neq \theta_{t + 1}$ only when $t \in \{\eta_{k}\}_{k\in [K]}$. Define the spacing and jump size as
\begin{equation}
    \Delta_k = \eta_{k+1} -\eta_{k},\ \kappa_k 
	  : =   \|\theta_{\eta_{k}+1} - \theta_{\eta_k}\|_2,
\end{equation}
where $\|\cdot \|$ is some norm in the parameter space $\Theta$, and let $\Delta = \min_{k\in [K] } \Delta_k$, $\kappa = \min_{k\in [K]}\kappa_k$. Change point detection aims to provide \textit{consistent} estimates $\{\hat{\eta}_k\}$.

It is well-known that the dynamic programming algorithm can solve the $\ell_0$ penalization problem for change point detection with $O(T^2 \mclC(T, p))$ time complexity, where $\mclC(T,p)$ is the time complexity for getting the estimator $\hat{\theta}(\mclI)$. 

The main concern upon the dynamic programming approach is that DP is more expensive to execute in practice compared to the wild binary segmentation. This motivates our project on improving the computational efficiency of DP with theoretical guarantee on the localization rate.

Improving the computational efficiency of change point detection algorithms is an important research direction. \cite{kovacs2020seeded} propose an algorithm called seeded binary segmentation that can reduce the computational complexity of Wild Binary Segmentation from $O(TM\mclC(T))$ to $O(T\log(T)\mclC(T))$ where $M$ is the number of initial intervals in the WBS algorithm and $\mclC(T)$ is the time complexity of fitting an estimator on samples of order $T$ which depends on the model.

We propose a new algorithm for retrospective change point detection called divide and conquer dynamic programming (DCDP) that can greatly improve the computational efficiency of the dynamic programming method that are currently used in the literature. We show by theory and numerical experiments that this algorithm works well for a broad range of problems and thus serve as a unified framework for change point detection.

Our contributions:
\begin{enumerate}
    \item A new efficient algorithm for change point detection with guarantee
    \item It's a unified method	for change point detection problems. We establish theoretical guarantee for high-dimensional mean model and high-dim linear model.
\end{enumerate}



==> backup_version/02_algorithm_and_complexity.tex <==
\section{Methodology}
We first discuss the general form of DCDP and its time  complexity of it.

Suppose we have $T$ observations and for any interval $\mclI \subset (0,T]$, we have some loss function $L(\theta,\mclI)$ and some goodness of fit function $\mclF(\theta,\mclI)$ that are defined according to the setting of the problem. For instance, when considering change points in high-dimensional linear models, we have $L(\beta,\mclI) = \sum_{i \in \mathcal I}   (y_i -X_i^\top \beta) ^2 + \lambda\sqrt{|\I|} \|\beta\|_1$, where
\begin{equation}
    \widehat \beta _{ \mathcal I } = \arg\min_{\beta \in \mathbb R^p } \sum_{i \in \mathcal I}   (y_i -X_i^\top \beta) ^2 + \lambda \sqrt{|\I|} \|\beta\|_1,
\end{equation}
and
\begin{equation}
    \mathcal F  (\beta, \I) := \begin{cases}
    \sum_{i \in \I } (y_i - X_i^\top \beta)^2, &\text{ when } |\I|\geq C_\mclF\s\log(np),\\
    0, &\text{otherwise}.
    \end{cases}.
\end{equation}
DCDP contains two steps: divide and conquer. In the divide step, we randomly sample $\mclQ$ integer points $\{s_i\}_{i\in [\mclQ]}\subset [n]$ and find best approximations to the true change points by \Cref{algorithm:DP}. The conquer step aims to further improve the localization accuracy based on the output of the divide step. It applies the local refinement in \Cref{algo:local_refine_general} to the output of the divide step.
\begin{algorithm}[htbp]
	\textbf{INPUT:} Data $\{ y_i, X_i \}_{i =1}^{n }$, tuning parameters $\lambda, \gamma,  \mclQ  > 0$.
 
 Randomly uniformly  sample $\mclQ $ points $\{ s_1, \ldots, s_ \mclQ \}$ from $(0, n)$.
 	  
(Divide) Get $\{\tilde{\eta}_k\}_{k\in [\tilde{K}]}$ with DP $(\{y_i, X_i\}_{i =1}^{n},\{s_i\}_{i\in [\mclQ]}, \lambda, \gamma)$.

(Conquer) $\{\hat{\eta}_k\}_{k\in [\hat{K}]}\leftarrow {\rm Refinement}(\{\tilde{\eta}_k\}_{k\in [\tilde{K}]})$. 
	
\textbf{OUTPUT:}  The estimated change points $\{\hat{\eta}_k\}_{k\in [\hat{K}]}$.
 	
 \caption{Divide and Conquer Dynamic Programming. DCDP $(\{y_i, X_i\}_{i =1}^{n}, \lambda, \gamma ,  \mclQ)$}
\label{algorithm:DCDP_divide}
\end{algorithm} 

\begin{algorithm}[htbp]
	\textbf{INPUT:} Data $\{ y_i, X_i \}_{i =1}^{n }$, tuning parameters $\lambda, \gamma$, grid $\{s_i\}_{i\in [m]}$ to search over.
 	 
 	 Set $\mathcal P= \emptyset$,  $\mathfrak{ p} =\underbrace{(-1,\ldots, -1)}_{ n }  $,  $B =\underbrace{( \gamma, \infty , \ldots,  \infty)}_{n } $.  Denote $B_i$ to be  the $i$-$th$ entry of $B$. 
 	 
 	\For {$r  $ in $\{s_i\}_{i\in [m]}$} {
 	 \For {$l  $ in $\{s_i\}_{i\in [m]}$, $ l<r  $} {
 	 $$ b \leftarrow B_{l}+ \gamma + \mathcal F (\hat{\theta}_\mclI, \mclI)  \quad \text{where} \quad \mclI=( l, \ldots, r]  ;$$
 	 \If {$b <  B_r $} {
 	 $B_r \leftarrow  b $;
 	 $\mathfrak{p}_r  \leftarrow l  $.
 	 } 
 	}
 	}

 To compute  the change point estimates from $  \mathfrak{p}  \in \mathbb N^n $, 	
 $ k \leftarrow  n  $.
 
 	  \While {$k >1$} {
 
  $ h  \leftarrow \mathfrak{p}_ k  $;
  $\mathcal P = \mathcal P \cup  h $;
  $ k  \leftarrow h $.
 	  }
	\textbf{OUTPUT:}  The estimated change points $\mathcal P$. 
 
 \caption{Dynamic Programming. DP $(\{y_i, X_i\}_{i =1}^{n},\{s_i\}_{i\in [m]}, \lambda, \gamma)$}
\label{algorithm:DP}
\end{algorithm} 


\begin{algorithm}[htbp]
	\textbf{INPUT:} Data $\{(Z_i)\}_{i=1}^{n}$, $\{\widetilde{\eta}_k\}_{k = 1}^{\widetilde{K}}$ ,  $\zeta > 0$.

	Let $(\widetilde{\eta}_0, \widetilde{\eta}_{\widetilde{K} + 1}) \leftarrow (0, n)$, $n_0\leftarrow C_{\mclF}\s\log(np)$.
	
	\For{$k = 1, \ldots, \widetilde{K}$} { 
	$(s_k, e_k) \leftarrow (2\widetilde{\eta}_{k-1}/3 + \widetilde{\eta}_{k}/3, \widetilde{\eta}_{k}/3 + 2\widetilde{\eta}_{k+1}/3)$


		\begin{align}
			\left(\hat{\eta},\hat{\theta}^{(1)},\hat{\theta}^{(2)}\right) &\leftarrow \argmin_{\substack{\eta \in \{s_k + n_0, \ldots, e_k - n_0\} \\ \theta^{(1)}, \theta^{(2)} \in \mathbb{R}^{p},\, \theta^{(1)} \neq \theta^{(2)}}}   \Bigg\{\mclF(\theta^{(1)},(s_k,\eta)) + \mclF(\theta^{(2)}, [\eta,e_k)) \nonumber \\
		    & \hspace{1.5cm} + \zeta  \sum_{i = 1}^p \sqrt{(\eta - s_k)(\theta^{(1)})_{i}^2 + (e_k - \eta)(\theta^{(2)})_{i}^2}\Bigg\} \label{eq-g-lasso}
		\end{align}
	}
	\textbf{OUTPUT:} $\{\widehat{\eta}_k\}_{k = 1}^{\widetilde{K}}$.
\caption{Local Refinement. }%LR$(\{(x_t, y_t)\}_{t=1}^{n}, \{\widetilde{\eta}_k\}_{k = 1}^{\widetilde{K}}, \zeta)$}
\label{algo:local_refine_general}
\end{algorithm} 


In general, the computational complexity of the divide step is $O(\mclQ^2 \mclC(n))$ where $\mclC(n)$ is the computational complexity of getting $\hat{\theta}(\mclI)$ where $|\mclI|\asymp n$. In contrast, the standard DP costs $O(n^2 \mclC(n))$. Thus we want smaller $\mclQ$ to make the improvement significant. As we will show later, in the current framework of DCDP, when the minimal spacing is $\Delta\geq \mclB_n \Delta_0$, we need $\mclQ \geq \frac{n}{\Delta}\mclB_n \log(n)$ to guarantee consistency. Here $\{\mclB_n\}$ is any diverging sequence and $\Delta_0$ is usually the minimal sample size for the estimator of the model to have $o(1)$ estimation error. Therefore, the complexity of the divide step is in general
\[
O(\left(\frac{n}{\Delta}\right)^2\log^3(n) \cdot \mclC(n)).
\]
The reduction in complexity gets bigger as $\Delta$ gets bigger. For models with linear structures such as linear regression and covariance estimation, by some pre-calculation step that costs $O(n)$, we can further reduce $\mclC(n)$ to be free of $n$, as we will discuss next. However, for nonlinear models like logistic regression, $\mclC(n)$ is generally at least of order $n$. In either case, when $\Delta\asymp n$, the complexity will be of order $O(n\log^3(n))$, which is a big improvement compared to the standard DP.

==> backup_version/03_main_results.tex <==
\section{Theoretical analysis}
We present some results on the localization error of DCDP in the case of mean model and high dimensional linear regression. Briefly, with the reduction on the computational complexity, the localization error with a single divide step will be larger than that of the vanilla DP by a term $\htr$. As is shown in \Cref{cor:mean local refinement} and \Cref{cor:regression local refinement}, this extra term can be removed by applying a local refinement algorithm to the output of the divide step.

Consider a generic interval $\I = (s,e)$ containing a single change point $\eta$ and let $\I_1 = (s,\eta]$, $\I_2 = (\eta,e)$. In the proof of DP, a key property to prove is
\begin{equation}
    L(\widehat{\theta}_{\I},\I) - L(\theta_1^*,\I_1) - L(\theta_1^*,\I_1) \geq {\rm signal}(\I_1,\I_2) + {\rm noise},
\end{equation}
and when $|\I_1|,|\I_2|$ are large enough,
\begin{equation}
    \gamma < {\rm signal}(\I_1,\I_2) - |{\rm noise}|,\ {\rm signal}(\I_1,\I_2) > |{\rm noise}|.
\end{equation}
For DCDP, we need to prove that in addition,
\begin{equation}
    L(\widehat{\theta}_{\I},\I) - L(\theta_1^*,\I_1) - L(\theta_1^*,\I_1) \leq {\rm approx}(\I_1,\I_2) + {\rm noise},
\end{equation}
and when $|\I_1|,|\I_2|$ are small enough,
\begin{equation}
    \gamma > {\rm approx}(\I_1,\I_2) + |{\rm noise}|.
\end{equation}




\subsection{Change in the mean}

\bnassum[Mean model]
\label{assp: DCDP_mean}
   Suppose  for $1 \le i \le n$, the data  $\{X_{i } \}_{1\le i \le n }   $ satisfy mean model $X_{i} =    \mu _i    +\epsilon_i\in \mathbb{R}^p$ with a collection of change points $ 0=\eta_0 <  \eta_1  < \eta_2 < \ldots <\eta_K < \eta _{K+1}= n  $ and that  the following conditions hold.   
\begin{enumerate}
     \item The measurement errors are independent mean-zero subgaussian random variables with $\sigma_{\epsilon} =\sup_{i} \|\epsilon_i\|_{\psi_2}<\infty$.
    %  $\mathbb{E}[\epsilon_t\epsilon_t^\top] = \Sigma_{\epsilon}$ and denote $\sigma_{\epsilon}$ as the largest eigenvalue of $\Sigma_{\epsilon}$.
     \item For each $i \in \{ 1,\ldots, n\}$,    there exists a collection of subsets  $  S_i \subset\{1, \ldots, p \}$,  such that 
	  $$  \mu _ { i,j} =0 \text{ if } j \not \in S_i.$$
	  In addition the  cardinality  of the support satisfies $|S_i|\leq \mathfrak{s} $. 
	 \item Denote 
	 $ \kappa_k 
	  : =   \| \mu_{\eta_{k}+1}^* - \mu_{\eta_k}^* \|_2 $.   Suppose that 
	 $  \kappa _k \asymp  \kappa$ for all $1\le k \le K$.
	 \item Denote   
	  $\Delta_k = \eta_{k+1} -\eta_{k}. $ 
	 and 
	 $\Delta = \min_{1\le k \le K } \Delta_k$. Let $\Bt$ be any diverging sequence.  Suppose that
	  $ \Delta \kappa^2  \ge \Bt \sigma_{\epsilon}^2 \s \log(np)  $.
\end{enumerate}
\enassum

\bnthm \label{thm:DCDP mean}
Suppose  \Cref{assp: DCDP_mean} holds and $\gamma\ge C_\gamma K\tr\kappa^2$  for sufficiently large constant $C_\gamma$. Let 
 $\widehat { \mathcal P }  $ denote the output of  \Cref{algorithm:DP} with 
 \begin{equation}
    \mathcal F  (\widehat{\mu}_\I,\I) := \begin{cases}
    \sum_{i \in \I } \|X_i - \widehat \mu_\I \|_2 ^2, &\text{ when } |\I|\geq C_\mclF\sigma_{\epsilon}^2\s\log(np),\\
    0, &\text{otherwise},
    \end{cases}.
\end{equation}
where $\widehat{\mu}_{\I}$ is given by
\begin{equation}
    \widehat{\mu}_{\I} = \argmin_{\mu\in \mathbb{R}^p}\|X_i - \mu\|_2^2 + \lambda \sqrt{|\I|}\|\mu\|_1,
\end{equation}
with $\lambda = C_{\lambda}\sqrt{\log(np)}$. Here $C_{\lambda}$ and $C_{\mclF}$ are sufficiently large universal constants. Let $\{ \widehat \eta_k\}_{k=1}^{\widehat K } $ be  the collection of change points induced by $\widehat { \mathcal P}$.
 Then
 with probability  at least $1 - C n ^{-3}$, $\widehat K = K$ and that
 \[ 
 \max_{ 1\le k \le K } |\eta_k-\widehat \eta_k|   \lesssim   \sigma_{\epsilon}^2\frac{  \log(n) +\gamma }{\kappa^2 } + \htr .
 \]
 \enthm
 
\bncor
\label{cor:mean local refinement}
Under the conditions of \Cref{thm:DCDP mean}, let $\{\widehat{\eta}_k\}_{k = 1}^{K}$ be a set of time points satisfying $\widehat K = K$ and
	\begin{equation}\label{eq-lr-cond-1}
		\max_{k = 1, \ldots, K} |\widehat{\eta}_k - \eta_k| \leq \Delta/5.
	\end{equation}
	Let $\{\widetilde{\eta}_k\}_{k = 1}^{\widehat{K}}$ be the change point estimators generated from \Cref{algo:local_refine_general} with $\{\widehat{\eta}_k\}_{k = 1}^{K}$ and $\zeta = 0$. Then
	\[ 
 \max_{ 1\le k \le K } (\eta_k-\widehat \eta_k)\kappa^2   = O_P(\sigma_{\epsilon}^2).
 \]
\encor

\subsection{Change in the covariance}

\bnassum[Covariance model]
\label{assp:DCDP_covariance}
  Suppose  for $i\in [n]$,    the data  $\{X _{i } \}_{i\in [n]}   $ are mean-zero Gaussian variables in $\mathbb{R}^p$ with non-singular covariance matrix $\Sigma_i = \mathbb{E}[X_iX_i^\top]$ and Orlicz norm $g_X = \sup_{i\geq 1}\|X_i\|_{\psi_2}<\infty$. Assume there is a collection of change points $ 0=\eta_0 <  \eta_1  < \eta_2 < \ldots <\eta_K < \eta _{K+1}= n  $ and that  the following conditions hold.   
\begin{enumerate}
    \item For $i\in [n]$, $c_XI_p \preceq \Sigma_i \preceq C_X I_p$ where $c_X>0, C_X<\infty$ are universal constants.
	 \item Denote 
	 $ \kappa_k 
	  : =   \|\Sigma^{-1}_{\eta_{k}+1} - \Sigma^{-1}_{\eta_k}\|_F$.   Suppose that 
	 $  \kappa _k \asymp  \kappa$ for all $1\le k \le K$.
	 \item Denote   
	  $\Delta_k = \eta_{k+1} -\eta_{k}. $ 
	 and 
	 $\Delta = \min_{1\le k \le K } \Delta_k$. Let $\Bt$ be any diverging sequence.  Suppose that
	  $ \Delta \kappa^2  \geq \Bt \frac{g_X^4}{c_X^4} p^2\log(np)$.
\end{enumerate}
\enassum

\bnrmk
Since $\{X_i\}_{i\in [n]}$ are Gaussian, we can make $g_X = C_X$ since $\|X_i\|_{\psi_2} = \lambda_{\max}(\Sigma_{X})$. I am trying to generalize to subgaussian variables with convex concentration property.
\enrmk


\bnthm
\label{thm:DCDP covariance}
Suppose \Cref{assp:DCDP_covariance} holds and $\gamma\ge C_\gamma K\tr\kappa^2$  for sufficiently large constant $C_\gamma$. Let 
 $\widehat { \mathcal P }  $ denote the output of  \Cref{algorithm:DP} with 
 \begin{equation}
    \mathcal F  (\widehat{\Omega}_\I,\I) := \begin{cases}
    \sum_{i \in \I } {\rm Tr}[\widehat{\Omega}^\top X_iX_i^\top] - |\I|\log|\widehat{\Omega}| , &\text{ when } |\I|\geq C_\mclF\frac{g_X^4}{c_X^2}p\log(np),\\
    0, &\text{otherwise},
    \end{cases}.
\end{equation}
where $\widehat{\Omega}_{\I}$ is given by
\begin{equation}
    \widehat{\Omega}_{\I} = \argmin_{\Omega\in \mathbb{S}^p_+} \sum_{i \in \I } {\rm Tr}[{\Omega}^\top X_iX_i^\top] - |\I|\log|\Omega|.
\end{equation}
Here $C_{\mclF}$ is a sufficiently large universal constant. Let $\{ \widehat \eta_k\}_{k=1}^{\widehat K } $ be  the collection of change points induced by $\widehat { \mathcal P}$.
 Then
 with probability  at least $1 - C n ^{-3}$, $\widehat K = K$ and that
 \[ 
 \max_{ 1\le k \le K } |\eta_k-\widehat \eta_k|   \lesssim   \frac{g_X^4C_X^2}{c_X^6}\frac{ p^2 \log(np) +\gamma }{\kappa^2 } + \htr .
 \]
\enthm



\bncor
\label{cor:covariance local refinement}
Under the conditions of \Cref{thm:DCDP covariance}, let $\{\widehat{\eta}_k\}_{k = 1}^{K}$ be a set of time points satisfying $\widehat K = K$ and
	\begin{equation}\label{eq-lr-cond-1}
		\max_{k = 1, \ldots, K} |\widehat{\eta}_k - \eta_k| \leq \Delta/5.
	\end{equation}
	Let $\{\widetilde{\eta}_k\}_{k = 1}^{\widehat{K}}$ be the change point estimators generated from \Cref{algo:local_refine_general} with
	$$
	\mclF(\theta, \I) = \|\theta - \frac{1}{|\I|}\sum_{i\in \I}X_iX_i^\top\|_F^2,
	$$
	$\{\widehat{\eta}_k\}_{k = 1}^{K}$ and $\zeta = 0$. Then  
 \[ 
 \max_{ 1\le k \le K } (\eta_k-\widehat \eta_k)\kappa^2  = O_P(\log(n)).
 \]
\encor



% \bncor[Local refinement]
% \label{cor:covariance local refinement}
% Under \Cref{assp:DCDP_covariance}, let $\{\widehat{\eta}_k\}_{k = 1}^{K}$ be a set of time points satisfying
% 	\begin{equation}\label{eq-lr-cond-1}
% 		\max_{k = 1, \ldots, K} |\widehat{\eta}_k - \eta_k| \leq \Delta/5.
% 	\end{equation}
% 	Let $\{\widetilde{\eta}_k\}_{k = 1}^{\widehat{K}}$ be the change point estimators generated from the local refinement algorithm with $\{\widehat{\eta}_k\}_{k = 1}^{K}$ as inputs. Then
%  with probability at least $1 - C n ^{-3}$, $\widehat K = K$ and that
%  \[ 
%  \max_{ 1\le k \le K } |\eta_k-\widehat \eta_k|   \lesssim   \frac{\|X\|_{\psi_2}^4}{c_{X}^4}\frac{ d^2\log(nd)}{\kappa^2}.
%  \]
% \encor



\subsection{Change in the linear model}


 \bnassum[High-dimensional linear regression]\label{assp:dcdp_linear_reg}
   Suppose  for $1 \le i \le n$,    $\{X_{i } \}_{1\le i \le n }  \subset \mathbb R^p   $ and $ \{ y_i\}_{i=1}^n \subset \mathbb R  $ satisfy the regression model
	$y_{i  } =   X_i^\top \beta ^* _i     +\epsilon_i  $ with a collection of change points $ 0=\eta_0 <  \eta_1  < \eta_2 < \ldots <\eta_K < \eta _{K+1}=n $
and that  the following conditions hold.   
\begin{enumerate}
    \item Suppose that $\{ X_i\}_{i=1}^n \overset{i.i.d.}{\sim} N_p(0, \Sigma )$  and that the minimal and the maximal eigenvalues of  $\Sigma$ satisfy 
	  $$  0< c_x \le  \Lambda_{\min}   (\Sigma) \le    \Lambda_{\max} (\Sigma ) \le C_x < \infty .   $$ In addition, suppose that $ \{ \epsilon_i \}_{i=1}^n  \overset{i.i.d.}{\sim}  N(0, \sigma^2_ \epsilon)$ is a collection of  random  errors independent of $\{ X_i\}_{i=1}^n $.
	  \item For each $i \in \{ 1,\ldots, n\}$,    there exists a collection of subsets  $  S_i \subset\{1, \ldots, p \}$,  such that 
	  $$  \beta^* _ { i,j} =0 \text{ if } j \not \in S_i.$$
	  In addition the  cardinality  of the support satisfies $|S_i|\leq \mathfrak{s} $. 
	  \item There exists a parameter  $\kappa>0$ such that for each  $ k \in \{ 0,\ldots, K\}   $,  it holds that
	 $$  
	   \| \beta^* _{\eta_k+1} - \beta_{\eta_k} ^* \|_2 \asymp \kappa  .$$
	   In addition,  suppose that $ \kappa  < C_\kappa$  for some universal constant $C_{\kappa}<\infty$.
	   \item Denote the spacing of change points as
	  $\Delta_k = \eta_{k+1} -\eta_{k}. $ 
	 and 
	 $\Delta = \min_{1\le k \le K } \Delta_k$. It holds that $\Delta  \kappa ^2 \geq \Bt (\sigma_{\epsilon}^2\vee 1)\mathfrak{s}\log(np) $.
\end{enumerate}
\enassum


 \bnthm \label{thm:DCDP regression}
Suppose \Cref{assp:dcdp_linear_reg} holds and $\gamma\ge C_\gamma K \tr\kappa^2$  for sufficiently large constant $C_\gamma$. Let 
 $\widehat { \mathcal P }  $ denote the output of  \Cref{algorithm:DCDP_divide} and
 \[
 \mathcal F  (\hat{\beta}_{\I},\mclI) :  = \begin{cases} 
 \sum_{i \in \mclI } (y_i - X_i^\top \widehat \beta _\mclI ) ^2  &\text{if } |\mclI|\ge C_\mclF \s\log(np),
 \\ 
 0 &\text{otherwise,}  
 \end{cases}   
 \]
 where $C_{\mclF}$ is a universal constant. Let 
$ \{ \widehat \eta_k\}_{k=1}^{\widehat K } $ be  the collection of change points induced by $\widehat { \mathcal P}$.
 Then
 with probability  at least $1 - C n ^{-3}$, $\widehat K = K$ and that
 $$ \max_{ 1\le k \le K } |\eta_k-\widehat \eta_k|   \lesssim  (\sigma_{\epsilon}^2\vee 1)\bigg( \frac{  \mathfrak{s} \log(np) +\gamma }{\kappa^2 }\bigg) +  \htr$$
 \enthm
 
 Once we get the output $\{\hat{\eta}_k\}_{k\in [\hat{K}]}$ from the DP, we can apply the local refinement algorithm and get refined estimates $\{\widetilde{\eta}_k\}_{k\in [\hat{K}]}$ that further reduce the term $\htr$ in the localization error.
 
\bncor
 \label{cor:regression local refinement}
Under the conditions of \Cref{thm:DCDP regression}, let $\{\widehat{\eta}_k\}_{k = 1}^{K}$ be a set of time points satisfying $\widehat K = K$ and
	\begin{equation}\label{eq-lr-cond-1}
		\max_{k = 1, \ldots, K} |\widehat{\eta}_k - \eta_k| \leq \Delta/5.
	\end{equation}
	Let $\{\widetilde{\eta}_k\}_{k = 1}^{\widehat{K}}$ be the change point estimators generated from \Cref{algo:local_refine_general} with $\{\widehat{\eta}_k\}_{k = 1}^{K}$  and $\zeta = 0$. Then
	\begin{align*}
	 \max_{k = 1, \ldots, K}(\widetilde{\eta}_k - \eta_k)\kappa^2 = O_P(\sigma_{\epsilon}^2\vee 1).
	\end{align*}
\encor

==> backup_version/04_experiment.tex <==
\section{Numerical experiments}
\subsection{Run time and localization error of the divide step}
\label{sec:experiment_time_error_divide}
In the first experiemnt, we generate $T=4\Delta$ samples from the univariate Gaussian mean model $y_t = \mu^*_t + \epsilon_t$ with 3 change points at $\eta_{k} = k\Delta + 1$ for $k = 1,2,3$ and $\mu_{\eta_0} = 0$, $\mu_{\eta_1} = 5$, $\mu_{\eta_2} = 0$, $\mu_{\eta_3} = 5$. In \Cref{fig:loc_vs_n_grid} and \Cref{fig:runtime_n_grid}, we present the localization error rate and run time of DCDP with $\mclR = 5$ as $\mclQ$, the number of random samples in the grid changes from 25 to 200. The localization error rate is defined as $H(\{\hat{\eta}\},\{\eta\})/T$ where $H(\cdot,\cdot)$ is the Hausdorff distance between two sets.




We show results for $\Delta = 500$ and $\Delta = 5000$. For the tuning parameter $\gamma$, we search over a list from $0.2\Delta$ to $0.4\Delta$. To tune $\gamma$, we run DCDP on each value of $\gamma$ on the training data and get estimates of mean values on induced intervals, then check the goodness-of-fit of the testing data on the estimated mean values, and pick the $\gamma$ with the best goodness-of-fit value. Here the training and testing data are generated from the same model above. In practice, one can do a odd-even split on the data. In experiments, $60$ trials are run for each value of $\mclQ$.
\begin{figure}[H]
    \centering
    \includegraphics[width = 0.46 \textwidth]{Figure/Delta500_loc_error_grid_num.png}
    \includegraphics[width = 0.47
    \textwidth]{Figure/Delta5000_loc_error_grid_num.png}
    \caption{Localization error vs. number of points $\mclQ$ in the grid. Left: $\Delta = 500$; right: $\Delta = 5000$. The line is the average and the shaded area shows the upper and lower 0.1 quantiles from 60 trials. Blue: only divide step; orange: dvide step followed by a local refinement.}
    \label{fig:loc_vs_n_grid}
\end{figure}

\Cref{fig:runtime_n_grid} illustrates the efficiency of DCDP in the sense that the original DP with the grid set to be $[T]$ corresponds to $\mclQ = T$, which will take much longer time to run. As a reference, the WBS method implemented by our own takes 0.14 and 10.79 seconds with average error $5.6$ and $0.0$ for $\Delta = 500, 5000$.
\begin{figure}[H]
    \centering
    \includegraphics[width = 0.46 \textwidth]{Figure/Delta500_runtime_grid_num.png}
    \includegraphics[width = 0.47
    \textwidth]{Figure/Delta5000_runtime_grid_num.png}
    \caption{Run time vs. number of points $\mclQ$ in the grid. Left: $\Delta = 500$; right: $\Delta = 5000$. The line is the average and the shaded area shows the upper and lower 0.1 quantiles from 60 trials. Blue: only divide step; orange: dvide step followed by a local refinement.}
    \label{fig:runtime_n_grid}
\end{figure}


\subsection{Comparison with other methods}
In this section, we will compare the performance of DCDP with several competitors in the literature. Apart from the standard Wild Binary Segmentation \citep{Fryzlewicz2014} and the standard Dynamic Programming \citep{pelt2012, rinaldo2021cpd_reg_aistats}, we also consider serveral competitors that were developed recently, including the Seeded WBS \citep{kovacs2020seeded}, the Block Fused Lasso \citep{unify_sinica2022}, and the Change Forest \citep{changeforest2022}.

==> backup_version/05_proof.tex <==
\section{Proof}
\label{sec:proof}
\subsection{Fundamental lemma}
In the proof of localization error of the standard dynamic programming, we frequently compare the goodness-of-fit $\mclF(\mclI)$ over an interval $\mclI = (s,e]$ with
\[
\mclF((s,\eta_{i + 1}]) + \cdots + \mclF((\eta_{i + m},e]) + m\gamma
\]
where $\{\eta_{i + j}\}_{j\in [m]} = \{\eta_{\ell}\}_{\ell\in [K]}\cap \mclI$ is the collection of true change points within interval $\mclI$ and $\gamma$ is the penalty coefficient in the DP. 

However, for DCDP, we only search over the random grid $\{s_{\ell}\}_{\ell\in [\mclQ]}$ that does not contain any true change points in general. Therefore, we need two fundamental lemmas that guarantee the existence of some reference points that are close to true change points, and the deviation of goodness-of-fit evaluated at the output of DCDP compared to those reference points.

\paragraph{Reference points.} Suppose  the sample points $\{ s_q\}_{q=1}^\Q $ are uniformly and independently  sampled from $(0,n)$. 
 Let 
$ \{ \eta_k\}_{k=1}^{K}$ be the collection of change points and denote 
\begin{align*} 
  \mathcal L _k (\delta)  : = \bigg  \{    \{ s_q\}_{q=1}^\Q \cap   [\eta_k -\delta ,\eta_k  ]  \not  =\emptyset \bigg  \} , \quad \text{and} \quad    \mathcal R  _k (\delta)  : = \bigg  \{    \{ s_q\}_{q=1}^\Q \cap   [\eta_k ,\eta_k + \delta   ]  \not  =\emptyset \bigg  \}  .
\end{align*} 
Denote 
\begin{align} 
\label{eq:left and right approximation of change points}  \mathcal L(\delta)  : = \bigcap_{k=1}^{K}   \mathcal L _k  \big  (   \delta   \big  )  
\quad \text{and} \quad 
\mathcal R (\delta)  : = \bigcap_{k=1}^{K}   \mathcal R _k  \big  (  \delta  \big  ) .   
\end{align}  
\bnlem Suppose  the sample points $\{ s_q\}_{q=1}^\Q $ are uniformly and independently  sampled from $(0,n)$. 
It holds that 
\[
\p \bigg (    \bigcap_{k=1}^{K}   \mathcal  L _k (\delta)  \bigg ) \ge 1 -  \exp( - 2\delta \Q / n+ \log(K)  ) 
\quad \text{and} \quad 
 \p \bigg (    \bigcap_{k=1}^{K}   \mathcal  R  _k (\delta)  \bigg ) \ge 1 -  \exp( - 2\delta \Q / n+ \log(K)  ).
\]
If in addition that   $\Q\ge 4 (  n/\Delta ) \log(n)  \Bn   $ for some slowly diverging sequence $\Bn$, then 
\[
\p \bigg (        \mathcal L   (  \tr   \big  )  \bigg )     \ge 1 - \frac{1}{n} \quad \text{and}  \quad  \p \bigg (      \mathcal R   \big  (  \tr   \big  )  \bigg )     \ge 1 - \frac{1}{n}  .
\]
\enlem

\begin{proof} 
Note that 
\[
\p( \mathcal L _k (\delta) ^c  ) =  \bigg( 1-  \frac{ \delta }{ n } \bigg)^ \Q \le \exp( -  \delta \Q / n ).
\]
Consequently,
\[
\p \bigg (    \bigg\{  \bigcap_{k=1}^{K}   \mathcal  L _k (\delta)  \bigg\}^c  \bigg ) \le  \sum_{k=1}^K \p ( \mathcal  L _k (\delta) ^c  )  
\le K \exp( - \delta \Q / n ) =  \exp( -  \delta \Q / n+ \log(K)  ) . 
\]
Setting $\delta =  \tr  $ and noting that $K\le n/\Delta$, it follows that if $\Q\ge 4 (  n/\Delta ) \Bn \log(n)   $, then 
\[
\p \bigg (     \bigcap_{k=1}^{K}   \mathcal  L _k  \big  (\tr   \big  )  \bigg )  \ge 1- \exp \bigg( -  4 \log (n )  + \log( n/\Delta )\bigg)  \ge 1 - \frac{1}{n^3} .
\]
\end{proof} 









%%%% location indicator %%%%
%%%% start of regression part %%%%



\paragraph{Goodness-of-fit.} For different models, the deviation of the goodness-of-fit has different orders. We need to analyze each model separately.

\bnlem[Mean model]
\label{lem:mean one change deviation bound}
Let $\mathcal I =(s,e] $ be any generic interval and $\widehat \mu_\I = \argmin_{\mu}[\frac{1}{|\mclI|}\sum_{i\in \mclI}\|X_i - \mu\|_2^2 + \frac{\lambda}{\sqrt{|\mclI|}}\|\mu\|_1]$. 

{\bf a.} If $\I$ contains no change points. Then it holds that 
$$\p \bigg( \bigg|   \sum_{ i  \in \I } \|X_i   -\widehat \mu_\I   \|_2^2  - \sum_{ i   \in \I } \|X_i      - \mu^*_i   \|_2^2  \bigg|  \ge C \sigma_{\epsilon}^2\mathfrak{s}\log(np)  \bigg)  \le  (np)^{-3}. $$

{\bf b.}  Suppose that the interval $ \I=(s,e]$ contains one and only one change point $ \eta_k $. Denote
$$  \mathcal J = (s,\eta_k] \quad \text{and} \quad  \mathcal J' =  (\eta_k, e]  .$$   Then it holds that 
$$\p \bigg( \bigg|   \sum_{ i  \in \I } \|X_i   -\widehat \mu_\I   \|^2  - \sum_{ i   \in \I } \|X_i      - \mu^*_i    \|^2  \bigg|  \geq \frac{ | \J||\J'| }{ |\I| }  \kappa_k ^2  +C \sigma_{\epsilon}^2\mathfrak{s}\log(np)  \bigg)   \le  (np)^{-3}. $$
\enlem
\begin{proof} 
We show {\bf b} as {\bf a} immediately follows from {\bf b} with $ |\J'| =0$. Denote 
$$  \mathcal J = (s,\eta_k] \quad \text{and} \quad  \mathcal J' =  (\eta_k, e]  .$$ 
Denote  $\mu_\I = \frac{1}{|\I | } \sum_{i\in \I } \mu^*_i $.
The it holds that 
\begin{equation*}
    \begin{split}
        &\sum_{i\in \I} \|X_i -\widehat \mu_\I\|_2^2  - \sum_{i\in \I} \|X_i - \mu^*_i\|_2^2  \\
        =& \sum_{i \in \I } \|\widehat \mu_\I-\mu^*_i \|_2^2  -2 \sum_{i \in \I } \epsilon_i^\top  (\widehat \mu_\I  - \mu^*_i)\\
        \leq& \sum_{i \in \I } \|\widehat \mu_\I-\mu^*_\I \|_2^2 + \sum_{i \in \I } \|\mu^*_\I-\mu^*_i \|_2^2  -2 \sum_{i \in \I } \epsilon_i^\top  (\widehat \mu_\I  - \mu^*_\I) - 2 \sum_{i \in \I } \epsilon_i^\top  (\mu^*_\I  - \mu^*_i).
    \end{split}
\end{equation*} 
Observe that 
\begin{equation*}
    \p \bigg(\|\sum_{i\in \I } \epsilon_i \|_{\infty}  \geq C\sigma_{\epsilon}\sqrt {\log(np)|\I |   }\bigg) \leq (np)^{-5 } 
\end{equation*}
Suppose this event holds.

{\bf Step 1.} By the event and \Cref{lem:estimation_high_dim_mean}, we have
\begin{equation*}
    \begin{split}
        \sum_{i \in \I } \|\widehat \mu_\I-\mu^*_\I \|_2^2 &\leq C\sigma_{\epsilon}^2\s\log(np),\\
        |2 \sum_{i \in \I } \epsilon_i^\top  (\widehat \mu_\I  - \mu^*_\I)| &\leq |\I|\|\sum_{i\in \I}\epsilon_i\|_{\infty}\|\widehat \mu_\I-\mu^*_\I\|_1\leq C\sigma_{\epsilon}^2\s\log(np).
    \end{split}
\end{equation*}
{\bf Step 2.} Notice that 
\begin{align*} 
    \sum_{   i \in \I } \|\mu^*_\I-\mu^*_i\| ^2  =  
        & \sum_{   i \in \I }  \| \frac{ | \J | \mu^*_\J + | \J'| \mu^*_{ \J ' }}{|\I| } -\mu^*_i  \|_2 ^2\\
 =  &     \sum_{i\in \J }   \| \frac{ |\J '|  (\mu^*_\J  - \mu^*_{\J'} ) }{|\I| }  \|_2^2 + 
     \sum_{i\in \J' }   \| \frac{ |\J  |  (\mu^*_\J  - \mu^*_{\J'} ) }{|\I| }  \|_2^2
  \\ = &  \frac{|\J | | \J'| }{|\I|  }(\mu^*_\J  - \mu^*_{\J'} ) ^2 = \frac{|\J | | \J'| }{|\I|  }    \kappa_k  ^2.
    \end{align*}
Meanwhile, it holds that 
\begin{align*} 
\sum_{  i     \in \I } \epsilon_i ^\top (\mu^*_\I  - \mu^*_i  ) =
& \sum_{   i \in \I }  \epsilon_i^\top  \bigg ( \frac{ | \J | \mu^*_\J + | \J'| \mu^*_{ \J ' }}{|\I| }-\mu^*_i  \bigg )  
\\
=&  \frac{|\J'|}{|\I|}\sum_{i\in \J }   \epsilon_i^\top(    \mu^*_{\J'}-\mu^*_\J  ) + 
   \frac{|\J|}{|\I|}\sum_{i\in \J' }   \epsilon_i^\top(    \mu^*_{\J}-\mu^*_{\J'}  )
   \\
   \le &    C_2\sigma_{\epsilon}\sqrt {   \frac{|\J | | \J'| }{|\I|  }     \kappa_k  ^2  \log(np) }
   \le \frac{|\J | | \J'| }{|\I|}   \kappa_k  ^2    +  C\sigma_{\epsilon}^2\log(np)  ,
\end{align*}
where the first inequality follows from the fact that the variance is upper bounded by
$$\sum_{i\in \J }  \sigma_{\epsilon}^2 \frac{ |\J '|^2 }{|\I|^2 } \|\mu^*_\J  - \mu^*_{\J'} \|_2^2 + \sum_{i\in \J' }  \sigma_{\epsilon}^2 \frac{ |\J|^2 }{|\I|^2 } \|\mu^*_\J  - \mu^*_{\J'} \|_2^2 =    \frac{|\J | | \J'| }{|\I|  }\sigma_{\epsilon}^2 \kappa_k^2 . $$
\end{proof} 




\bnlem
\label{lem:estimation_high_dim_mean}
For any interval $\mclI\subset [1, n]$ with $|\mclI|\geq C_0\mathfrak{s}\log(np)$ that might contain change points. Let
\begin{equation*}
    \hat{\mu}_{\mclI}\defined \argmin_{\mu\in \mathbb{R}^p}\frac{1}{|\mclI|}\|X_i - \mu\|_2^2 + \frac{\lambda}{\sqrt{|\mclI|}}\|\mu\|_1,
\end{equation*}
for $\lambda = C_{\lambda}\sigma_{\epsilon}\sqrt{\log(np)}$ for sufficiently large constant $C_{\lambda}$. Then it holds with probability at least $1 - (np)^{-5}$ that
\begin{equation}
    \begin{split}
    \|\widehat{\mu}_{\I}-\mu^*_{\I}\|_{2}^{2} &\leq \frac{C\sigma_{\epsilon}^2 \s \log (np)}{\I} \\
\left\|\widehat{\mu}_{\I}-\mu^*_{\I}\right\|_{1} &\leq C \sigma_{\epsilon}\s \sqrt{\frac{\log (np)}{|\I|}} \\
\|\left(\widehat{\mu}_{\I}-\mu^*_{\I}\right)_{S^{c}}\|_{1} &\leq 3\|\left(\widehat{\mu}_{\I}-\mu^{*}_{\I}\right)_{S}\|_{1},
    \end{split}
\end{equation}
where $\mu_\mclI = \frac{1}{|\I|}\sum_{i\in \I}\mu^*_i$.
\enlem


\begin{proof}
By definition, we have $L(\widehat{\mu}_{\I},\I)\leq L({\mu}_{\I},\I)$, that is
\begin{align}
\nonumber
    &\sum_{i\in \I}\|Y_i - \widehat{\mu}_{\I}\|_2^2 + \lambda\sqrt{|\I|}\|\widehat{\mu}_{\I}\|_1\leq \sum_{i\in \I}\|Y_i - {\mu}^*_{\I}\|_2^2 + \lambda\sqrt{|\I|}\|{\mu}^*_{\I}\|_1\\
\nonumber
    \Rightarrow & \sum_{i\in \I}(\widehat{\mu}_{\I} - \mu^*_{\I})^\top (2Y_i - \mu^*_{\I} - \widehat{\mu}_{\I}) + \lambda\sqrt{|\I|}[\|{\mu}^*_{\I}\|_1 - \|\widehat{\mu}_{\I}\|_1]\geq 0 \\
    \nonumber
    \Rightarrow & (\widehat{\mu}_{\I} - \mu^*_{\I})^\top (\sum_{i\in \I}\epsilon_i) + 2(\widehat{\mu}_{\I} - \mu^*_{\I})^\top\sum_{i\in \I}(\mu^*_i - \mu^*_{\I}) - |\I|\sum_{i\in \I}\|\widehat{\mu}_{\I} - \mu^*_{\I}\|_2^2 + \lambda\sqrt{|\I|}[\|{\mu}^*_{\I}\|_1 - \|\widehat{\mu}_{\I}\|_1]\geq 0\\
    \Rightarrow & \|\widehat{\mu}_{\I} - \mu^*_{\I}\|_1 \|\sum_{i\in \I}\epsilon_i\|_{\infty} + \lambda\sqrt{|\I|}[\|{\mu}^*_{\I}\|_1 - \|\widehat{\mu}_{\I}\|_1]\geq |\I|\sum_{i\in \I}\|\widehat{\mu}_{\I} - \mu^*_{\I}\|_2^2.
    \label{tmp_eq:mean_concentration}
\end{align}
By a union bound, we know that for some universal constant $C>0$, with probability at least $1 - (np)^{-5}$,
$$
\|\sum_{i\in \I}\epsilon_i\|_{\infty}\leq C\sigma_{\epsilon}\sqrt{|\I|\log(np)}\leq \frac{\lambda}{2}\sqrt{|\I|},
$$
as long as $C_{\lambda}$ is sufficiently large. Therefore, based on the sparsity assumption in \Cref{assp: DCDP_mean}, it holds that
\begin{align*}
    &\frac{\lambda}{2}\|\widehat{\mu}_{\I} - \mu^*_{\I}\|_1 + \lambda[\|{\mu}^*_{\I}\|_1 - \|\widehat{\mu}_{\I}\|_1]\geq 0 \\
    \Rightarrow & \frac{\lambda}{2}\|\widehat{\mu}_{\I} - \mu^*_{\I}\|_1 + \lambda[\|({\mu}^*_{\I})_S\|_1 - \|(\widehat{\mu}_{\I})_S\|_1]\geq \lambda \|(\widehat{\mu}_{\I})_{S^c}\|_1\\
    \Rightarrow & \frac{\lambda}{2}\|\widehat{\mu}_{\I} - \mu^*_{\I}\|_1 + \lambda\|({\mu}^*_{\I}-\widehat{\mu}_{\I})_S\|_1 \geq \lambda \|(\mu^*_{\I} - \widehat{\mu}_{\I})_{S^c}\|_1\\
    \Rightarrow & 3\|({\mu}^*_{\I}-\widehat{\mu}_{\I})_S\|_1\geq \|({\mu}^*_{\I}-\widehat{\mu}_{\I})_{S^c}\|_1.
\end{align*}
Now from \Cref{tmp_eq:mean_concentration} we can get
\begin{align*}
    |\I|\|\widehat{\mu}_{\I} - \mu^*_{\I}\|_2^2\leq &\frac{3\lambda}{2}\sqrt{|\I|}\|\widehat{\mu}_{\I} - \mu^*_{\I}\|_1\\
    \leq & \frac{12\lambda}{2}\sqrt{|\I|}\|(\widehat{\mu}_{\I} - \mu^*_{\I})_S\|_1\\
    \leq & 6\lambda \sqrt{\s} \sqrt{|\I|}\|(\widehat{\mu}_{\I} - \mu^*_{\I})_S\|_2\\
    \leq & 6\lambda \sqrt{\s} \sqrt{|\I|}\|\widehat{\mu}_{\I} - \mu^*_{\I}\|_2,
\end{align*}
which implies that
$$
\|\widehat{\mu}_{\I} - \mu^*_{\I}\|_2\leq 6C_{\lambda}\sigma_{\epsilon}\sqrt{\frac{\s\log(np)}{|\I|}}.
$$
The other inequality follows accordingly.
\end{proof}


















\subsection{Mean model}
In this section we show the proof of \Cref{thm:DCDP mean} and \Cref{cor:mean local refinement}. Throughout this section, for any generic interval $\I\subset [1,n]$, denote $\mu^*_{\I} = \frac{1}{|\I|}\sum_{i\in \I}\mu^*_i$ and
$$ \widehat \mu_\I = \argmin_{\mu}\frac{1}{|\mclI|}\sum_{i\in \mclI}\|X_i - \mu\|_2^2 + \frac{\lambda}{\sqrt{|\mclI|}}\|\mu\|_1. $$
Also, unless specially mentioned, in this section, we set the goodness-of-fit function $\mathcal F  (\I)$ in \Cref{algorithm:DCDP_divide} to be
\begin{equation}
    \mathcal F  (\I) := \begin{cases}
    \sum_{i \in \I } \|X_i - \widehat \mu_\I \|_2 ^2, &\text{ when } |\I|\geq C_\mclF\sigma_{\epsilon}^2\s\log(np),\\
    0, &\text{otherwise},
    \end{cases}.
\end{equation}
where $C_\mclF$ is a universal constant.
 
 \begin{proof}[Proof of \Cref{thm:DCDP mean}]
 By  \Cref{prop:mean local consistency}, $K \leq |\widehat{\mathcal{P}}| \leq 3K$.  This combined with \Cref{prop:change points partition size consistency} completes the proof.
 \end{proof}
 

 \bnprop\label{prop:mean local consistency}
 Suppose  \Cref{assp: DCDP_mean} holds. Let 
 $\widehat { \mathcal P }  $ denote the output of  \Cref{algorithm:DCDP_divide}.
 Then with probability  at least $1 - C n ^{-3}$, the following conditions hold.
	\begin{itemize}
		\item [(i)] For each interval  $ \I = (s, e] \in \widehat{\mathcal{P}}$    containing one and only one true 
		   change point $ \eta_k $, it must be the case that
 $$\min\{ \eta_k -s ,e-\eta_k \}  \lesssim  \sigma_{\epsilon}^2\bigg( \frac{  \s\log(np) +\gamma }{\kappa_k^2 }\bigg) +  \tr      .$$
		\item [(ii)] For each interval  $  \I = (s, e] \in \widehat{\mathcal{P}}$ containing exactly two true change points, say  $\eta_ k  < \eta_ {k+1} $, it must be the case that
			\begin{align*} 
 \eta_k -s    \lesssim      \htr    \quad \text{and} \quad 
 e-\eta_{k+1}  \lesssim   \htr     . 
 \end{align*} 
		 
\item [(iii)] No interval $\I \in \widehat{\mathcal{P}}$ contains strictly more than two true change points; and 


	\item [(iv)] For all consecutive intervals $ \I_1 $ and $ \I_2 $ in $\widehat{ \mathcal P}$, the interval 
		$ \I_1 \cup  \I_2 $ contains at least one true change point.
				
	 \end{itemize}
\enprop 

%The four cases in \Cref{proposition:dp step 1} are proved in Lemmas~\ref{lemma:one change point}, \ref{lemma:two change point}, \ref{lemma:no change point} and \ref{lemma:three change point}, respectively, and \Cref{proposition:dp step 1} is proved consequently.

\bnprop\label{prop:change points partition size consistency}
Suppose  \Cref{assp: DCDP_mean} holds. Let 
 $\widehat { \mathcal P }  $ be the output of  \Cref{algorithm:DCDP_divide}.
 Suppose 
$ \gamma \ge C_\gamma K\tr \kappa^2 $  for sufficiently large constant $C_\gamma$. Then
 with probability  at least $1 - C n ^{-3}$,  $| \widehat { \mathcal P} | =K $.
\enprop



\begin{proof}[Proof of   \Cref{prop:change points partition size consistency}] 
Denote $\mathfrak{G} ^*_n = \sum_{ i =1}^n \|X_i  -  \mu^*_i\|_2^2$.  Given any collection $\{t_1, \ldots, t_m\}$, where $t_1 < \cdots < t_m$, and $t_0 = 0$, $t_{m+1} = n$, let 
\begin{equation}\label{eq-sn-def}
	\G _n(t_1, \ldots, t_{m}) = \sum_{k=1}^{m} \sum_{ i = t_k +1}^{t_{k+1}} \mclF(\widehat \mu_  {(t_{k}, t_{k+1}]}, (t_{k}, t_{k+1}]).
\end{equation}
For any collection of time points, when defining \eqref{eq-sn-def}, the time points are sorted in an increasing order.

Let $\{ \widehat \eta_{k}\}_{k=1}^{\widehat K}$ denote the change points induced by $\widehat {\mathcal P}$.  Suppose we can justify that 
	\begin{align}
		\G^*_n + K\gamma  \ge  &\G _n(s_1,\ldots,s_K)   + K\gamma - C_1 ( K +1)\sigma_{\epsilon}^2 \s  \log(np) - C_1\sum_{k\in [K]}\kappa_k^2\tr  \label{eq:K consistency step 1} \\ 
		\ge & \G_n (\widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } ) +\widehat K \gamma - C_1 ( K +1)  \sigma_{\epsilon}^2 \s  \log(np) - C_1\sum_{k\in [K]}\kappa_k^2\tr  \label{eq:K consistency step 2} \\ 
		\ge &  \G _n ( \widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K ) + \widehat K \gamma    - C_1' ( K +1)  \sigma_{\epsilon}^2 \s  \log(np)- C_1'\sum_{k\in [K]}\kappa_k^2\tr  \label{eq:K consistency step 3}
	\end{align}
	and that 
	\begin{align}\label{eq:K consistency step 4}
		\G ^*_n   -\G _n ( \widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K ) \le C_2 (K + \widehat{K} + 2) \sigma_{\epsilon}^2 \s  \log(np).
	\end{align}
	Then it must hold that $| \hatp | = K$, as otherwise if $\widehat K \ge K+1 $, then  
	\begin{align*}
		C _2 (K + \widehat{K} + 2)  \sigma_{\epsilon}^2 \s  \log(np)  & \ge   \G ^*_n  -\G _n ( \widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K ) \\
		& \ge      (\widehat K - K)\gamma  -C_1 ( K +1)  \sigma_{\epsilon}^2 \s  \log(np) - C_1\sum_{k\in [K]}\kappa_k^2\tr.
	\end{align*} 
	Therefore due to the assumption that $| \hatp|  =\widehat K\le 3K $, it holds that 
	\begin{align} \label{eq:Khat=K} 
		[C_2 (4K + 2) + C_1(K+1)] \sigma_{\epsilon}^2 \s  \log(np) +C_1\sum_{k\in [K]}\kappa_k^2\tr \ge  (\widehat K - K)\gamma \geq \gamma,
	\end{align}
	Note that \eqref{eq:Khat=K} contradicts the choice of $\gamma$.


\
\\
{\bf Step 1.} Note that \eqref{eq:K consistency step 1}  is implied by 
	\begin{align}\label{eq:step 1 K consistency}  
		\left| 	\G ^*_n - \G_n(s_1,\ldots,s_K)    \right| \le  C_3(K+1) \sigma_{\epsilon}^2 \s  \log(np) + C_3\sum_{k\in [K]}\kappa_k^2\tr,
	\end{align}
	which is  an  immediate consequence  of \Cref{lem:mean one change deviation bound}. 
	\
	\\
	\\
	{\bf Step 2.} Since $\{ \widehat \eta_{k}\}_{k=1}^{\widehat K}$ are the change points induced by $\widehat {\mathcal P}$, \eqref{eq:K consistency step 2} holds because $\hatp$ is a minimizer.
\\
\\
	{\bf Step 3.}
For every $ \I  =(s,e]\in \hatp$, by \Cref{prop:mean local consistency}, we know that $\I$ contains at most two change points. We only show the proof for the two-change-points case as the other case is easier. Denote
	\[
		 \I =  (s ,\eta_{q}]\cup (\eta_{q},\eta_{q+1}] \cup  (\eta_{q+1} ,e]  = \J_1 \cup \J_2 \cup \J_{3},
	\]
where $\{ \eta_{q},\eta_{q+1}\} =\I \, \cap \, \{\eta_k\}_{k=1}^K$. 

For each $ m=1,2,3$, if $|\J_m|\geq C_\mclF\sigma_{\epsilon}^2\s\log(np)$, then by \Cref{lem:mean one change deviation bound}, it holds that
$$
\sum_{ i \in \J_m }\|y_ i - \widehat\mu_{\J_m}\|_2^2   \leq \sum_{ i \in \J_ m } \|y_ i - \mu^*_i\|_2^2 + C\sigma_{\epsilon}^2\s\log(np). 
$$
Thus, we have
\begin{equation}
    \mclF(\widehat\mu_{\J_m},\J_m)\leq \mclF(\mu^*_{\J_m},\J_m) + C\sigma_{\epsilon}^2\s\log(np).
\end{equation}
On the other hand, by \Cref{lem:mean loss deviation no change point}, we have
$$
\mclF(\widehat\mu_{\I},\J_m)   \geq \mclF(\mu^*_{\J_m},\J_m) - C\sigma_{\epsilon}^2\s\log(np). 
$$
Therefore the last two inequalities above imply that 
\begin{align} 
\label{eq:K consistency step 3 inequality 3}  
\sum_{i \in \I }  \mclF(\widehat \mu_\I,\I) \geq & \sum_{m=1}^{3} \sum_{ i \in \J_m }\mclF(\widehat \mu_\I,\J_m) \\
\geq & \sum_{m=1}^{3}   \sum_{ i \in \J_m}\mclF(\widehat \mu_{\J_m},\J_m) - C\sigma_{\epsilon}^2\s\log(np).
\end{align}
Note that \eqref{eq:K consistency step 3} is an immediate consequence of   \eqref{eq:K consistency step 3 inequality 3}.

{\bf Step 4.}
Finally, to show \eqref{eq:K consistency step 4},   let  $\widetilde { \mathcal P}$ denote    the partition induced by $\{\widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K\}$. Then 
$| \widetilde { \mathcal P} | \le K + \widehat K+2   $ and that $\mu^*_i$ is unchanged in every interval $\I \in \widetilde { \mathcal P}$. 
	So  \Cref{eq:K consistency step 4} is an immediate consequence of   \Cref{lem:mean one change deviation bound}.
\end{proof} 






\begin{proof}[Proof of \Cref{cor:mean local refinement}]
For each $k\in [K]$, let $\hat{\mu}_t = \hat{\mu}^{(1)}$ if $s_k<t< \hat{\eta}_k$ and $\hat{\mu}_t =\hat{\mu}^{(2)}$ otherwise, and ${\mu}^*_t$ be the true parameter at time point $t$. First we show that under conditions $\tilde{K} = K$ and $\max_{k\in [K]}|\tilde{\eta}_k - \eta_k|\leq \Delta / 5$, there is only one true change point $\eta_k$ in $(s_k, e_k)$. It suffices to show that
\begin{equation}
    |\tilde{\eta}_k - \eta_k|\leq \frac{2}{3}(\tilde{\eta}_{k+1} - \tilde{\eta}_{k}),\ \text{and}\ |\tilde{\eta}_{k+1} - \eta_{k+1}|\leq \frac{1}{3}(\tilde{\eta}_{k+1} - \tilde{\eta}_{k}).
    \label{tmp_eq:goal_lr}
\end{equation}
Denote $R = \max_{k\in [K]}|\tilde{\eta}_k - \eta_k|$, then
\begin{align*}
    \tilde{\eta}_{k+1} - \tilde{\eta}_{k} &= \tilde{\eta}_{k+1} - {\eta}_{k+1} + {\eta}_{k+1} - {\eta}_{k} + {\eta}_{k} - \tilde{\eta}_{k} \\
    &= ({\eta}_{k+1} - {\eta}_{k}) + (\tilde{\eta}_{k+1} - {\eta}_{k+1}) + ({\eta}_{k} - \tilde{\eta}_{k})\in [{\eta}_{k+1} - {\eta}_{k} - 2R,{\eta}_{k+1} - {\eta}_{k} + 2R].
\end{align*}
Therefore, \Cref{tmp_eq:goal_lr} is guaranteed as long as
\begin{equation*}
    R\leq \frac{1}{3}(\Delta - 2R),
\end{equation*}
which is equivalent to $R\leq \Delta/5$.

Now without loss of generality, assume that $s_k<\eta_k<\hat{\eta}_k<e_k$. Denote $\mclI_k = \{s_k + 1, \cdots, e_k\}$. Consider two cases:

\textbf{Case 1} If
\begin{equation*}
    \hat{\eta}_k - \eta_k < \max\{C\sigma_{\epsilon}^2\s\log(np), C\sigma_{\epsilon}^2\s\log(np)/\kappa^2\},
\end{equation*}
then the proof is done.

\textbf{Case 2} If
\begin{equation*}
    \hat{\eta}_k - \eta_k \geq \max\{C\sigma_{\epsilon}^2\s\log(np), C\sigma_{\epsilon}^2\s\log(np)/\kappa^2\},
\end{equation*}
then we proceed to prove that $|\hat{\eta}_k - \eta_k|\leq C\sigma_{\epsilon}^2\s\log(np)/\kappa^2$ with probability at least $1 - (Tn)^{-3}$. Then we either prove the result or get an contradiction, and complete the proof in either case.

By definition, we have
\begin{equation*}
    \sum_{t\in \I}\|y_t - \hat{\mu}_t\|_2^2 + \zeta\sum_{i = 1}^p \sqrt{\sum_{i\in \I}(\hat{\mu}_t)_i^2}\leq \sum_{t\in \I}\|y_t - {\mu}^*_t\|_2^2 + \zeta\sum_{i = 1}^p \sqrt{\sum_{i\in \I}({\mu}^*_t)_i^2},
\end{equation*}
which implies that
\begin{equation*}
    \sum_{t\in \I}\|\mu^*_t - \hat{\mu}_t\|_2^2 + \zeta\sum_{i = 1}^p \sqrt{\sum_{i\in \I}(\hat{\mu}_t)_i^2}\leq 2\sum_{t\in \I}(y_t - \mu^*_t)^\top (\hat{\mu}_t - \mu^*_t) + \zeta\sum_{i = 1}^p \sqrt{\sum_{i\in \I}({\mu}^*_t)_i^2}.
\end{equation*}
Denote $\delta_t = \hat{\mu}_t - \mu^*_t$. Notice that
\begin{align*}
    & \sum_{i  \in [p]} \sqrt{\sum_{i\in \I}({\mu}^*_t)_i^2} - \sum_{i  \in [p]} \sqrt{\sum_{i\in \I}(\hat{\mu}_t)_i^2} \\ 
    =& \sum_{i \in [p]} \sqrt{\sum_{i\in \I}({\mu}^*_t)_i^2} - \sum_{i \in S} \sqrt{\sum_{i\in \I}(\hat{\mu}_t)_i^2} - \sum_{i \in S^c} \sqrt{\sum_{i\in \I}(\hat{\mu}_t)_i^2} \\
    \leq & \sum_{i \in S} \sqrt{\sum_{i\in \I}(\delta_t)_i^2} - \sum_{i \in S^c} \sqrt{\sum_{i\in \I}(\delta_t)_i^2}.
\end{align*}
Now we check the cross term. Notice that the variance of $\sum_{t\in \I}(\epsilon_t)_i(\delta_t)_i$ is $\sum_{t\in \I}(\delta_t)_i^2$, so with probability at least $1 - (np)^{-5}$,
\begin{equation*}
    \sum_{t\in \I}(y_t - \mu^*_t)^\top (\hat{\mu}_t - \mu^*_t)\leq C\sigma_{\epsilon}\sqrt{\log(np)}\sum_{i \in [p]}\sqrt{\sum_{t\in \I}(\delta_t)_i^2}\leq \frac{\zeta}{4}\sum_{i \in [p]}\sqrt{\sum_{t\in \I}(\delta_t)_i^2},
\end{equation*}
since $\zeta = C_{\zeta}\sigma_{\epsilon}\sqrt{\log(np)}$ with sufficiently large constant $C_{\zeta}$. Combining inequalities above, we can get
\begin{align*}
    \sum_{t\in \I}\|\delta_t\|_2^2 +\frac{\zeta}{2}\sum_{i\in S^c}\sqrt{\sum_{t\in \I}(\delta_t)_i^2}
    \leq & \frac{3\zeta}{2}\sum_{i\in S}\sqrt{\sum_{t\in \I}(\delta_t)_i^2} \\
    \leq & \frac{3\zeta}{2}\sqrt{\s}\sqrt{\sum_{t\in \I}\|(\delta_t)_S\|_2^2} \\
    \leq & \frac{3\zeta}{2}\sqrt{\s}\sqrt{\sum_{t\in \I}\|\delta_t\|_2^2},
\end{align*}
which implies that
\begin{equation}
    \sum_{t\in \I}\|\delta_t\|_2^2\leq \frac{9}{4}\s\zeta^2\leq C\s\sigma_{\epsilon}^2\log(np).
    \label{tmp_eq:upper_bound_delta_local_refine}
\end{equation}
Without loss of generality, assume that $\hat{\eta}>\eta_k$ and denote
$$
\J_1 = [s_k, \eta_k), \J_2 = [\eta_k, \hat{\eta}_k), \J_3 = [\hat{\eta}_k, e_k),
$$
and $\mu^{(1)} = \mu^*_{\eta_k - 1}$, $\mu^{(2)} = \mu^*_{\eta_k}$. Then \Cref{tmp_eq:upper_bound_delta_local_refine} is equivalent to
\begin{equation*}
    \J_1\|\hat{\mu}^{(1)} - \mu^{(1)}\|_2^2 + \J_2\|\hat{\mu}^{(1)} - \mu^{(2)}\|_2^2 + \J_3\|\hat{\mu}^{(2)} - \mu^{(2)}\|_2^2 \leq C\s\sigma_{\epsilon}^2\log(np).
\end{equation*}
Since $|\mclJ_1|=\eta_k - s_k\geq c_0\Delta$ with some constant $c_0$ under \Cref{assp: DCDP_mean}, we have
\begin{equation}
    \Delta \|\hat{\mu}^{(1)} - \mu^{(1)}\|_2^2\leq c_0|\mclJ_1|\|\hat{\mu}^{(1)} - \mu^{(1)}\|_2^2 \leq C \sigma_{\epsilon}^2\s\log(np)\leq c_2\Delta \kappa^2,
\end{equation}
with some constant $c_2\in (0,1/4)$, where the last inequality is due to the fact that $\Bn \rightarrow \infty$. Thus we have
\begin{equation*}
    \|\hat{\mu}^{(1)} - \mu^{(1)}\|_2^2\leq c_2\kappa^2.
\end{equation*}
Triangle inequality gives
\begin{equation*}
    \|\hat{\mu}^{(1)} - \mu^{(2)}\|_2\geq \|\mu^{(1)} - \mu^{(2)}\|_2 - \|\hat{\mu}^{(1)} - \mu^{(1)}\|_2 \geq \kappa/2.
\end{equation*}
Therefore, $\kappa^2|\mclJ_2|/4\leq |\mclJ_2|\|\hat{\mu}^{(1)} - \mu^{(2)}\|_2^2\leq C \sigma_{\epsilon}^2\s\log(np)$ and
\begin{equation*}
    |\hat{\eta}_k - \eta_k| = |\mclJ_2|\leq \frac{C \sigma_{\epsilon}^2\s\log(np)}{\kappa^2}.
\end{equation*}
\end{proof}






\subsubsection{Technical lemmas and proofs}
Throughout this section, let $\widehat { \mathcal P }  $ denote the output of  \Cref{algorithm:DCDP_divide}.
 
 
 





\bnlem
\label{lem:mean loss deviation no change point}
Let $\I\subset [1,T]$ be any interval that contains no change point. Then for any interval $\J \supset \I$, it holds with probability at least $1 - (np)^{-5}$ that
\begin{equation*}
    \mclF(\mu^*_{\I},\I)\leq \mclF(\widehat{\mu}_\J,\I) + C\sigma_{\epsilon}^2\s\log(np).
\end{equation*}
\enlem
\begin{proof}
{\bf Case 1}. If $|\I|< C_\mclF\sigma_{\epsilon}\s\log(np)$, then by definition, we have $\mclF(\mu^*_{\I},\I) = \mclF(\widehat \mu^*_{\J},\I) = 0$ and the inequality holds.

{\bf Case 2}. If $|\I|\geq  C_\mclF\sigma_{\epsilon}\s\log(np)$, then take difference and we can get
\begin{align*}
    &\sum_{i\in \I}\|X_i - \mu^*_i\|_2^2 - \sum_{i\in \I}\|X_i - \widehat{\mu}_\J\|_2^2 \\
    =& 2(\widehat \mu_{\J} - \mu^*_{\I})^\top\sum_{i\in \I}\epsilon_i -|\I|\|\mu^*_{\I} - \widehat \mu_{\J}\|_2^2\\
    \leq & 2(\|(\widehat \mu^*_{\J} - \mu^*_{\I})_S\|_1 + \|(\widehat \mu_{\J} - \mu^*_{\I})_{S^c}\|_1)\|\sum_{i\in \I}\epsilon_i\|_{\infty} -|\I|\|\mu^*_{\I} - \widehat \mu^*_{\J}\|_2^2\\
    \leq& c_1\|\widehat \mu_{\J} - \mu^*_{\I}\|_2\sigma_{\epsilon}\sqrt{\s|\I|\log(np)} + c_2\sigma_{\epsilon}\sqrt{\frac{\log(np)}{|\I|}}\cdot c_1\sigma_{\epsilon}\sqrt{|\I|\log(np)} - |\I|\|\mu^*_{\I} - \widehat \mu_{\J}\|_2^2 \\
    \leq & \frac{1}{2}|\I|\|\mu^*_{\I} - \widehat \mu_{\J}\|_2^2 + 2c_1^2\sigma_{\epsilon}^2\s\log(np) + c_2\sigma_{\epsilon}^2\s\log(np) - |\I|\|\mu^*_{\I} - \widehat \mu_{\J}\|_2^2\\
    \leq & C\sigma_{\epsilon}^2\s\log(np),
\end{align*}
where in the second inequality we use the definition of the index set $S$ and \Cref{lem:estimation_high_dim_mean}.
\end{proof}






 
\bnlem
\label{lem:mean single cp}
Suppose the good events 
$\mathcal L (\tr ) $ and  $\mathcal R (\tr) $ defined  in \Cref{eq:left and right approximation of change points} hold. 
Let   $ \I=(s,e] \in \mathcal {\widehat P}  $  be such that $\I$ contains exactly  one    change point $ \eta_k $. 
 Then  with probability  at least $1-(np)^{-3}$,   it holds that 
 $$\min\{ \eta_k -s ,e-\eta_k \}  \lesssim    \sigma_{\epsilon}^2\bigg( \frac{ \s\log(np) +\gamma }{\kappa_k^2 }\bigg)  +  \tr    .$$
  \enlem
\begin{proof}   
If either $ \eta_k -s \le \tr  $ or $e-\eta_k\le \tr$, then there is nothing to show. So assume that 
$$  \eta_k -s  > \tr \quad \text{and} \quad   e-\eta_k  > \tr . $$
By event $\mathcal R (\tr )$, there exists  $ s_ u  \in \{ s_q\}_{q=1}^\Q$ such that 
$$0\le s_u - \eta_k \le \tr. $$
 So 
$$ \eta_k \le s_ u \le e .$$
Denote 
$$ \I_ 1 = (s,s_u] \quad \text{and} \quad \I_2 = (s_u, e] .$$
Since 
$s, e,  s_u \in  \{ s_q\}_{q=1}^\Q  $,   it follows that 
\begin{align}\nonumber
\sum_{i \in \I }\|X_i - \widehat \mu_\I \|_2 ^2 \le &  \sum_{i \in \I_1 }\|X_i - \widehat \mu_{\I_1}  \|_2 ^2  + \sum_{i \in \I_2 }\|X_i - \widehat \mu_{\I_2}  \|_2 ^2   + \gamma 
\\\nonumber 
\le &  \sum_{i \in \I_1 }\|X_i -  \mu^*_i \|_2 ^2 + C_1 \big (  \sigma_{\epsilon}^2\s\log(np) + (s_u -\eta_k) \kappa_k^2 \big )  
\\ \nonumber
& + \sum_{i \in \I_1 }\|X_i -  \mu^*_i \|_2 ^2 + C_1\sigma_{\epsilon}^2\s\log(np)  + \gamma
\\ \nonumber 
=&  \sum_{i \in \I }\|X_i -  \mu^*_i  \|_2 ^2  +C_2 \big (  \sigma_{\epsilon}^2\s\log(np) + (s_u -\eta_k)   \kappa_k^2 \big )+ \gamma 
\\
\le &  \sum_{i \in \I }\|X_i -  \mu^*_i \|_2 ^2  +C_2 \big (  \sigma_{\epsilon}^2\s\log(np) +  \tr    \kappa_k^2   \big ) + \gamma  , \label{eq:one change point step 1}
\end{align}
where the first inequality follows from the fact that $ \I =(s ,e ] \in \widehat { \mathcal P} $ and so it is the local minimizer, the second inequality follows from \Cref{lem:mean one change deviation bound} {\bf a} and {\bf b} and the observation that 
$$  \eta_k -s > \tr  \ge s_u -\eta_k $$ 
Denote 
$$ \J_1  = (s,\eta_k ] \quad \text{and} \quad \J_2 = (\eta_k , e] .$$
\Cref{eq:one change point step 1}  gives 
\begin{align*}
\sum_{i \in \J_1 }\|X_i - \widehat \mu_\I \|_2 ^2 +\sum_{i \in \J_2 }\|X_i - \widehat \mu_\I \|_2 ^2  
 \le \sum_{i \in \J_1  }\|X_i -  \mu^*_{ \J_1 } \|_2 ^2   +\sum_{i \in \J_2  }\|X_i -  \mu^*_{ \J_2  } \|_2 ^2  +C_2  \big (\sigma_{\epsilon}^2\s\log(np) +   \tr \kappa_k^2  \big )  + \gamma 
\end{align*}
which leads to 
\begin{align*}
&\sum_{i \in \J_1 }\|\widehat \mu_\I  - \mu^*_{\J_1 }\|_2^2 +\sum_{i \in \J_2 }\|\widehat \mu_\I  - \mu^*_{\J_2  } \|_2^2  
\\
 \leq  & 2 \sum_{i \in \J_1  } \epsilon_i^\top (\widehat \mu_\I  -  \mu^*_{ \J_1 } )     +2 \sum_{i \in \J_2  } \epsilon_i^\top (\widehat \mu_\I  -  \mu^*_{ \J_2 } )      +C_2  \big (\sigma_{\epsilon}^2\s\log(np) +  \kappa_k^2  \tr    \big )  + \gamma 
 \\
 \leq & 2\sigma_{\epsilon}\sum_{j = 1,2}\|\widehat \mu_\I  -  \mu^*_{ \J_j }\|_2 \sqrt{|\J_j|\log(np)}+   C_2  \big( \sigma_{\epsilon}^2\s\log(np) +  \kappa_k^2\tr\big ) + \gamma  \\
 \leq & \frac{1}{2} \sum_{j = 1,2}|\J_j|\|\widehat \mu_\I  -  \mu^*_{ \J_j }\|_2^2 + C_3  \big (\sigma_{\epsilon}^2\s\log(np) +  \kappa_k^2  \tr    \big )  + \gamma,
\end{align*} 
where the second inequality holds because the variance of $\sum_{i \in \J_1  } \epsilon_i^\top (\mu_\I  -  \mu^*_{ \J_1 } )$ is upper bounded by $|\J_1|\sigma^2_{\epsilon}\|\mu_\I  -  \mu^*_{ \J_1 }\|_2^2$.

It follows that 
$$ |\J_1 |\|  \widehat \mu_\I  - \mu^*_{\J_1 }\|_2 ^2 + |\J_2 |\|  \widehat \mu_\I  - \mu^*_{\J_2 }\|_2 ^2  =  \sum_{i \in \J_1 }\|  \widehat \mu_\I  - \mu^*_{\J_1 }\|_2 ^2 +\sum_{i \in \J_2 }\| \widehat \mu_\I  - \mu^*_{\J_2  }  \|_2^2    \le C_4\big ( \sigma_{\epsilon}^2\s\log(np) +\tr \kappa_k^2    \big )+ 2\gamma  .$$
Note that 
$$ \inf_{ a \in \mathbb R  }  |\J_1 |\|  a - \mu^*_{\J_1 }\|_2 ^2 + |\J_2 |\| a  - \mu^*_{\J_2 }\| ^2  = \kappa_k ^2  \frac{|\J_1| |\J_2|}{| \I| }   \ge \frac{ \kappa_k^2 }{2} \min\{ |\J_1| ,|\J_2| \}    . $$ 
This leads to 
$$  \frac{ \kappa_k^2 }{2}\min\{ |\J_1| ,|\J_2| \}    \le  C_4\big ( \sigma_{\epsilon}^2\s\log(np) +\tr  \kappa_k^2   + \gamma  \big )  ,$$
which is 
$$ \min\{ |\J_1| ,|\J_2| \}   \le C_5 \bigg( \frac{\sigma_{\epsilon}^2\s\log(np) + \gamma  }{\kappa_k^2 } +  \tr  \bigg) .$$
 \end{proof} 
 
 
 \bnlem 
Suppose the good events 
$\mathcal L (\tr ) $ and  $\mathcal R ( \tr ) $ defined  in  \Cref{eq:left and right approximation of change points} hold. 
Let   $ \I=(s,e] \in \mathcal {\widehat P}  $  be an interval that contains  exactly two  change points $ \eta_k,\eta_{k+1}  $.  Suppose in addition that 
\begin{align} \label{eq:1D two change points snr}
\Delta \kappa^2 \ge C   \Bn^{1/2}  \big(\sigma_{\epsilon}^2\s\log(np) + \gamma)    
\end{align} 
for sufficiently large constant $C $. 
 Then  with probability  at least $1-(np)^{-3}$,   it holds that 
\begin{align*} 
 \eta_k -s    \lesssim      \htr    \quad \text{and} \quad 
 e-\eta_{k+1}  \lesssim   \htr     . 
 \end{align*} 
 \enlem 
\begin{proof} 
Since the events $\mathcal L ( \tr  ) $ and  $\mathcal R ( \tr ) $ hold, let $ s_u, s_v$ be such that 
 $\eta_k \le s_u \le s_v \le \eta_{k+1} $ and that 
 $$ 0 \le s_u-\eta_k \le   \tr ,  \quad  0\le  \eta_{k+1} - s_v \le \tr   .    $$

 \begin{center}
 \begin{tikzpicture} 
\draw[ - ] (-10,0)--(1,0);
 \node[color=black] at (-8,-0.3) {\small s};
 \draw[  (-, ultra thick, black] (-8,0) -- (-7.99,0);
  \draw[ { -]}, ultra thick, black] (-1.0002,0) -- (-1,0);

   \node[color=black] at (-7,-0.3) {\small $\eta_k$};
\draw(-7 ,0)circle [radius=2pt] ;

  \node[color=black] at (-6.5,-0.3) {\small $s_u$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-6.5,0)  }; 
 

  \node[color=black] at (-2.3,-0.3) {\small $\eta_{k+1}$};
\draw(-2.3 ,0)circle [radius=2pt] ;
  \node[color=black] at (-3 ,-0.3) {\small $s_v$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-3,0)  }; 
  
   \node[color=black] at (-1,-0.3) {\small $e$};

 
\end{tikzpicture}
\end{center} 

Denote 
$$ \mathcal I_ 1= (  s, s _u], \quad \I_2  =(s_u, s_v] \quad \text{and} \quad \I_3  = (s_v,e]. $$
In addition, denote 
$$ \J_1  = (s,\eta_k ], \quad \J_2=(\eta_k, \eta_{k} + \frac{ \eta_{k+1}   -\eta_k  }{2}], \quad \J_3 =  ( \eta_k+ \frac{ \eta_{k+1}   -\eta_k  }{2},\eta_{k+1 } ]  \quad \text{and} \quad \J_4 = (\eta_{k+1}  , e] .$$
Since 
$s, e,  s_u ,s_v  \in  \{ s_q\}_{q=1}^\Q  $, then it follows from the definition of $\hat{\mclP}$ that 
\begin{align}\nonumber
& \sum_{i \in \I }\|X_i - \widehat \mu_\I \|_2^2
\\  \nonumber 
\le &  \sum_{i \in \I_1 }\|X_i - \widehat \mu_{\I_1} \|_2 ^2  + \sum_{i \in \I_2 }\|X_i - \widehat \mu_{\I_2}\|_2^2  + \sum_{i \in \I_3 }\|X_i - \widehat \mu_{\I_3}\|_2^2  +2 \gamma 
\\\nonumber 
\le &  \sum_{i \in \I_1 }\|X_i -  \mu^*_i\|_2^2 + C_1 \bigg ( \sigma_{\epsilon}^2 \s\log(np) +  \frac{|\J_1| (s_u -\eta_k ) }{ |\J_1| + (s_u -\eta_k )  }\kappa_k^2 \bigg )  +
 \sum_{i \in \I_2 }\|X_i -  \mu^*_i\|_2^2    +C_1   \sigma_{\epsilon}^2 \s\log(np)
 \\ \nonumber 
  + &  \sum_{i \in \I_3 }\|X_i -  \mu^*_i\|_2^2 + C_1 \bigg( \sigma_{\epsilon}^2 \s\log(np)+  \frac{|\J_4 | (\eta_{k+1} -s_v   )  }{ |\J_4 | + (\eta_{k+1} -s_v   )   } \kappa_{k+1} ^2   \bigg)   +2  \gamma
\\ 
\le  &  \sum_{i \in \I }\|X_i -  \mu^*_i\|_2^2  +C_1' \bigg (  \sigma_{\epsilon}^2 \s\log(np) +  \frac{|\J_1| (s_u -\eta_k ) }{ |\J_1| + (s_u -\eta_k )  }\kappa_k^2     +  \frac{|\J_4 | (\eta_{k+1} -s_v   )  }{ |\J_4 | + (\eta_{k+1} -s_v   )   }  \kappa_{k+1} ^2        \bigg )+2  \gamma 
  \label{eq:two change points step 1}
\end{align}
where the first inequality follows from the fact that $ \I =(s ,e ] \in \widehat { \mathcal P} $, the second inequality follows from \Cref{lem:mean one change deviation bound} {\bf a} and {\bf b}. 
\Cref{eq:two change points step 1}  gives 
\begin{align} \nonumber 
& \sum_{i \in \J_1 }\|X_i - \widehat \mu_\I\|_2^2 +\sum_{i \in \J_2 }\|X_i - \widehat \mu_\I\|_2^2  +\sum_{i \in \J_3 }\|X_i - \widehat \mu_\I\|_2^2 +\sum_{i \in \J_4 }\|X_i - \widehat \mu_\I\|_2^2   
\\ \nonumber  
 \le& \sum_{i \in \J_1  }\|X_i -  \mu^*_{ \J_1 }\|_2^2   +\sum_{i \in \J_2  }\|X_i -  \mu^*_{ \J_2  }\|_2^2 +\sum_{i \in \J_3  }\|X_i -  \mu^*_{ \J_3 }\|_2^2   +\sum_{i \in \J_4  }\|X_i -  \mu^*_{ \J_4  }\|_2^2  \\
 + & C_1' \bigg (\sigma_{\epsilon}^2 \s\log(np) +   \frac{|\J_1| (s_u -\eta_k ) }{ |\J_1| + (s_u -\eta_k )  }\kappa_k^2     + \frac{|\J_4 | (\eta_{k+1} -s_v   )  }{ |\J_4 | + (\eta_{k+1} -s_v   )   }  \kappa_{k+1}    ^2  \bigg )  + 2\gamma.  \label{eq:1D two change points first}
\end{align}
Note that for $\ell\in \{1,2,3,4 \}$,
\begin{align}\nonumber  
  &\sum_{i \in \J_\ell }\|X_i - \widehat \mu_\I\|_2^2  
 -   \sum_{i \in \J_\ell   }\|X_i -  \mu^*_{ \J_ \ell }\|_2^2  -\sum_{i \in \J_ \ell   }\|\widehat \mu_\I  - \mu^*_{\J_ \ell }\|_2^2 
\\
=& \nonumber 
 2 \sum_{i \in \J_ \ell   } \epsilon_i^\top ( \mu^*_{ \J_\ell  }-\widehat \mu_\I    )      
\\\nonumber   
\ge  & -  C\sigma_{\epsilon} \|\widehat \mu_\I  -  \mu^*_{ \J_\ell }\|_2 \sqrt{|\J_\ell|\log(np)}
\\
\ge  &  -\frac{1}{2}|\J_\ell| \|\widehat \mu_\I  -  \mu^*_{ \J_\ell }\|_2^2 - C'\sigma_{\epsilon}^2 \s\log(np). \nonumber  
\end{align} 
which gives 
\begin{align} \label{eq:1D two change points second}
  &\sum_{i \in \J_\ell }\|X_i - \widehat \mu_\I \|^2  
 -   \sum_{i \in \J_\ell   }\|X_i -  \mu^*_{ \J_ \ell }\|^2  \ge \frac{1}{2}\sum_{i \in \J_ \ell   }\| \widehat \mu_\I  - \mu^*_{\J_ \ell }\| ^2
-   C_2\sigma_{\epsilon}^2 \s\log(np) .
\end{align} 
\Cref{eq:1D two change points first} and 
\Cref{eq:1D two change points second} together implies that
 
\begin{align} \label{eq:1D two change points third}   \sum_{l=1}^ 4 
   |\J_l | (\widehat \mu_\I  -  \mu^*_{ \J_\ell } ) ^2        \le C_3 \bigg ( \sigma_{\epsilon}^2 \s\log(np) +\frac{|\J_1| (s_u -\eta_k ) }{ |\J_1| + (s_u -\eta_k )  }  \kappa_k^2    +\frac{|\J_4 | (\eta_{k+1} -s_v   )  }{ |\J_4 | + (\eta_{k+1} -s_v   )   } \kappa_{k+1} ^2    \bigg ) +4 \gamma  .  
   \end{align}
Note that 
\begin{align}  \label{eq:1D two change points signal lower bound} \inf_{ a \in \mathbb R  }  |\J_1 |(  a - \mu^*_{\J_1 }) ^2 + |\J_2 |( a  - \mu^*_{\J_2 }) ^2  =&     \frac{|\J_1| |\J_2|}{ |\J_1| +  |\J_2| } \kappa_k ^2.
\end{align} 
Similarly
\begin{align} \label{eq:1D two change points signal lower bound 2} \inf_{ a \in \mathbb R  }  |\J_3 |(  a - \mu^*_{\J_3 }) ^2 + |\J_4 |( a  - \mu^*_{\J_4 }) ^2   =     \frac{|\J_3| |\J_4|}{|\J_3| + |\J_4| }       \kappa_{k+1}  ^2  ,\end{align} 
\Cref{eq:1D two change points third} together with 
\Cref{eq:1D two change points signal lower bound} and \Cref{eq:1D two change points signal lower bound 2} leads to 
\begin{align}
\label{eq:conclusion of two change points} 
  \frac{|\J_1| |\J_2|}{ |\J_1| +  |\J_2| }  \kappa_k ^2   +   \frac{|\J_3| |\J_4|}{|\J_3| + |\J_4| } \kappa_{k+1}  ^2  \le C_3 \bigg (\sigma_{\epsilon}^2 \s\log(np) +\frac{|\J_1| (s_u -\eta_k ) }{ |\J_1| + (s_u -\eta_k )  }  \kappa_k^2    +\frac{|\J_4 | (\eta_{k+1} -s_v   )  }{ |\J_4 | + (\eta_{k+1} -s_v   )   } \kappa_{k+1} ^2    \bigg ) +4 \gamma  .
  \end{align}
 Note that 
$$ 0\le s_u -\eta_k \le \tr \quad \text{and} \quad 
0 \le \eta_{k+1} -s_v \le \tr,
 $$ 
and so there are four possible cases.  

{\bf case a.} 
If 
$$|\J_1| \le \htr  \quad \text{and} \quad  
 |\J_4|   \le \htr , $$ 
 then the desired result  follows immediately. 

{\bf case b.}   $|\J_1|   >  \htr    $ and  $|\J_4|     \le \htr     $. Then since $|\J_2| \ge \Delta /2  $, it holds that 
$$   \frac{|\J_1| |\J_2|}{ |\J_1| +  |\J_2| }  \ge  \frac{1}{2 }\min\{|\J_1| , |\J_2|  \} \ge  \frac{1}{2 }\htr.  $$
In addition,
$$\frac{|\J_1| (s_u -\eta_k ) }{ |\J_1| + (s_u -\eta_k )  }  \le s_u -\eta_k \le \tr  \quad   \text{and} \quad  \frac{|\J_4 | (\eta_{k+1} -s_v   )  }{ |\J_4 | + (\eta_{k+1} -s_v   )   }  \le \eta_{k+1} -s_v     \le \tr . 
$$
So  \Cref{eq:conclusion of two change points}  leads to 
\begin{align}\label{eq:conclusion of two change points case two} 
\frac{1}{2 }\htr   \kappa_k ^2   +   \frac{|\J_3| |\J_4|}{|\J_3| + |\J_4| } \kappa_{k+1}  ^2  \le C_3 \bigg (\sigma_{\epsilon}^2 \s\log(np) + \tr \kappa_k^2    + \tr \kappa_{k+1} ^2    \bigg ) +4 \gamma  .
  \end{align} 
Since $ \kappa_k \asymp \kappa$ and $ \kappa_{k+1}  \asymp \kappa$, \Cref{eq:conclusion of two change points case two} gives 
$$ \frac{1}{2 }\htr   \kappa  ^2  \le C_4 \bigg ( \sigma_{\epsilon}^2 \s\log(np) + \tr \kappa ^2    + \tr \kappa ^2    \bigg ) +4 \gamma   . $$
Since $\Bn $ is a diverging sequence, the above display gives 
$$ \Delta \kappa ^2  \le C_5\Bn^{1/2 } (\log(n) + \gamma ).$$
This contradicts \Cref{eq:1D two change points snr}.

{\bf case c.}  $|\J_1|    \le   \htr    $ and 
$|\J_4|     >  \htr     $. Then the same argument  as that in  {\bf case b} leads to the same contradiction.

 {\bf case d.}     $|\J_1|   >  \htr    $ and  $|\J_4|     >  \htr     $. Then since $|\J_2|\ge \Delta /2 , |\J_4| \ge \Delta /2  $, it holds that 
$$   \frac{|\J_1| |\J_2|}{ |\J_1| +  |\J_2| }  \ge  \frac{1}{2 }\min\{|\J_1| , |\J_2|  \} \ge  \frac{1}{2 }\htr\quad \text{and} \quad 
 \frac{|\J_3| |\J_4|}{ |\J_3| +  |\J_4| }  \ge  \frac{1}{2 }\min\{|\J_3| , |\J_4|  \} \ge  \frac{1}{2 }\htr   $$
In addition, 
$$\frac{|\J_4 | (\eta_{k+1} -s_v   )  }{ |\J_4 | + (\eta_{k+1} -s_v   )   }  \le \eta_{k+1} -s_v     \le \tr  \quad  
\frac{|\J_1| (s_u -\eta_k ) }{ |\J_1| + (s_u -\eta_k )  }  \le s_u -\eta_k \le \tr . 
$$
So  \Cref{eq:conclusion of two change points}  leads to 
\begin{align}\label{eq:conclusion of two change points case four} 
\frac{1}{2 }\htr   \kappa_k ^2   +   \frac{1}{2 }\htr     \kappa_{k+1}  ^2  \le C_6 \bigg (\sigma_{\epsilon}^2 \s\log(np) + \tr \kappa_k^2    + \tr \kappa_{k+1} ^2    \bigg ) +4 \gamma  .
  \end{align} 
Note that $\Bn $ is a diverging sequence. So the above display gives 
$$ \Delta \big  ( \kappa_{k}   ^2+ \kappa_{k+1}^2  \big)   \le C_ 7 \Bn^{1/2 } (\sigma_{\epsilon}^2 \s\log(np) + \gamma ) $$
Since   $ \kappa_k \asymp \kappa$ and  $ \kappa_{k+1}  \asymp \kappa$. This contradicts \Cref{eq:1D two change points snr}. 
 \end{proof}



 \bnlem 
Suppose the good events 
$\mathcal L (\tr ) $ and  $\mathcal R ( \tr ) $ defined  in  \Cref{eq:left and right approximation of change points} hold. 
 Suppose in addition that 
\begin{align} \label{eq:1D three change points snr}
\Delta \kappa^2 \ge C   \Bn  \big(\sigma_{\epsilon}^2 \s\log(np) + \gamma)    
\end{align} 
for sufficiently large constant $C $. 
 Then  with probability  at least $1-(np)^{-3}$,    there is no interval  $  \widehat { \mathcal P}  $  containing three or more true change points.   
 \enlem  
 


\begin{proof} 
For  contradiction,  suppose    $ \I=(s,e] \in \mathcal {\widehat P}  $  be such that $ \{ \eta_1, \ldots, \eta_M\} \subset \I $ with $M\ge 3$. Throughout the proof, $M$ is assumed to be a parameter that can potentially change with $n$. 
Since the events $\mathcal L ( \tr  ) $ and  $\mathcal R ( \tr ) $ hold, by relabeling $\{ s_q\}_{q=1}^\Q  $ if necessary,   let $ \{ s_m\}_{m=1}^M $ be such that 
 $$ 0 \le s_m  -\eta_m  \le \tr    \quad \text{for} \quad 1 \le m \le M-1  $$ and that
 $$ 0\le \eta_M  - s_M \le \tr .$$ 
 Note that these choices ensure that  $ \{ s_m\}_{m=1}^M  \subset \I . $
 
 \begin{center}
 \begin{tikzpicture} 
\draw[ - ] (-10,0)--(1,0);
 \node[color=black] at (-8,-0.3) {\small s};
 \draw[  (-, ultra thick, black] (-8,0) -- (-7.99,0);
  \draw[ { -]}, ultra thick, black] (-1.0002,0) -- (-1,0);

   \node[color=black] at (-7,-0.3) {\small $\eta_1$};
\draw(-7 ,0)circle [radius=2pt] ;

  \node[color=black] at (-6.5,-0.3) {\small $s_1$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-6.5,0)  }; 

  \node[color=black] at (-5,-0.3) {\small $\eta_2$};
\draw(-5 ,0)circle [radius=2pt] ;
  \node[color=black] at (-4.5,-0.3) {\small $s_2$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-4.5,0)  }; 
 

  \node[color=black] at (-2.5,-0.3) {\small $\eta_3$};
\draw(-2.5 ,0)circle [radius=2pt] ;
  \node[color=black] at (-3 ,-0.3) {\small $s_3$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-3,0)  }; 
  
   \node[color=black] at (-1,-0.3) {\small $e$};

 
\end{tikzpicture}
\end{center}

{\bf Step 1.}
 Denote 
 $$ \mathcal I_ 1= (  s, s _1], \quad \I_m   =(s_{m-1} , s_m] \text{ for }  2 \le m \le M     \quad \text{and} \quad \I_{M+1}   = (s_M,e]. $$
Then since 
$ s , e,  \{ s_m \}_{m=1}^M  \subset   \{ s_q\}_{q=1}^\Q  $,   it follows that 
\begin{align}\nonumber
& \sum_{i \in \I }\|X_i - \widehat \mu_\I\|_2^2
\\  \nonumber 
\le &  \sum _{m=1}^{M+1 } \sum_{i \in \I_m}\|X_i - \widehat y_{\I_m }  \|_2^2   + M  \gamma 
\\  \label{eq: 1D three change points deviation term 1}
\le &  \sum_{i \in \I_1 }\|X_i -  \mu^*_i\|_2^2 + C_1 \bigg ( \sigma_{\epsilon}^2 \s\log(np) +  \frac{ (\eta_1 -s ) ( s_1-\eta_ 1)  }{  s_1-s  }\kappa_1^2 \bigg )
\\   \label{eq: 1D three change points deviation term 2} 
+ & 
 \sum_{m=2}^{M-1} \sum_{i \in \I_m  }\|X_i -  \mu^*_i\|_2^2    +C_1  \bigg(\sigma_{\epsilon}^2 \s\log(np)+     \frac{(\eta_m -s_{m-1} )(s_m-\eta_{m } ) }{ s _{m}-s _{m-1}  }  \kappa_m^2 \bigg ) 
 \\  \label{eq: 1D three change points deviation term 3}
  + &    C_1 \sigma_{\epsilon}^2 \s\log(np)
\\ \label{eq: 1D three change points deviation term 4}
+ & \sum_{i\in \I_{M+1}}\|X_i-\mu^*_i\|_2^2+ C_1  \bigg( \sigma_{\epsilon}^2 \s\log(np) + \frac{(\eta_M -s_{M} )(e-\eta_{M} ) }{ e-s _{M}  }  \kappa_{M} ^2 \bigg ) + M\gamma, 
 \end{align}  
 where Equations \eqref{eq: 1D three change points deviation term 1}, \eqref{eq: 1D three change points deviation term 2}
 \eqref{eq: 1D three change points deviation term 3} and \eqref{eq: 1D three change points deviation term 4} follow from \Cref{lem:mean one change deviation bound} and in particular,   \Cref{eq: 1D three change points deviation term 3} corresponds to the interval $\I _M = (s_{M-1},s_M] $ which by assumption  containing no change points. 
 Note that 
\begin{align*} & \frac{ (\eta_1 -s ) ( s_1-\eta_ 1)  }{  s_1-s  } \le s_1-\eta_1  \le \tr ,
\\ 
&   \frac{(\eta_m -s_{m-1} )(s_m-\eta_{m } ) }{ s _{m}-s _{m-1}  } \le  s_m-\eta_m  \le \tr ,   \ \text{ and } 
\\
&   \frac{(\eta_M -s_{M} )(e-\eta_{M} ) }{ e-s _{M}  } \le \eta_M-s_m  \le \tr  
 \end{align*} 
 and  that 
 $ \kappa_k \asymp \kappa $ for all $ 1\le k \le K$. Therefore 
\begin{equation}
    \label{eq:1D three change points step 1}
  \sum_{i \in \I }\|X_i - \widehat \mu_\I\|_2^2 \le  \sum _{ i \in \I } \|X_i - \mu^*_i\|_2^2 +  C_2  \bigg( M \sigma_{\epsilon}^2 \s\log(np)+   M \tr \kappa^2
+  M\gamma \bigg),
\end{equation}
where $ C_2$ is some large constant independent of $M$.

{\bf Step 2.}  Let 
$$  \J_1 =(s,  \eta_1], \ \J_m = (\eta_{m-1}, \eta_m]  \text{ for } 2 \le m \le M , \ \J_{M+1}  =(\eta_M, e]. $$
Note that $\mu^*_i$ is unchanged in any of $\{ \J_m\}_{m=0}^{M+1}$.  
So  for $ 1 \le m \le M+1  $,
\begin{align}\nonumber  
  &\sum_{i \in  \J_m  }\|X_i - \widehat \mu_\I\|_2^2  
 -   \sum_{i \in \J_  m    }\|X_i -  \mu^*_{ \J_  m }\|_2^2  -\sum_{i \in \J_  m   }\|\widehat \mu_\I  - \mu^*_{\J_  m }\|_2^2 
\\
=& \nonumber 
 2 \sum_{i \in \J_  m} \epsilon_i^\top (\mu^*_{\J_ m}-\widehat \mu_\I)   
\\\nonumber   
\ge  & - C\sigma_{\epsilon}\|\widehat \mu_\I  -  \mu^*_{ \J_ m  }\|_2\sqrt{|\J_m|\log(np)}  
\\
\ge &   -  C_3  \sigma_{\epsilon}^2 \s\log(np) - \frac{1 }{2 } |\J_  m |\|\widehat \mu_\I  -  \mu^*_{ \J_ m  }\|_2^2   \nonumber  
\end{align} 
which gives 
\begin{align} \label{eq:1D three change points second}
  &\sum_{i \in \J_m  }\|X_i - \widehat \mu_\I\|_2^2 
 -   \sum_{i \in \J_ m   }\|X_i -  \mu^*_{ \J_  m }\|_2^2  \geq \frac{1}{2}\sum_{i \in \J_  m   }\|\widehat \mu_\I  - \mu^*_{\J_  m  }\|_2 ^2 - C_3\sigma_{\epsilon}^2 \s\log(np).
\end{align} 
Therefore
\begin{align} \label{eq:1D three change points third} \sum_{ m=1}^{M+1}   |\J_m |\|\widehat \mu_\I  - \mu^*_{\J_  m  }\|_2^2 = \sum_{ m=1 }^{M+1}  \sum_{i \in \J_  m   }\|\widehat \mu_\I  - \mu^*_{\J_  m  }\|_2^2 \le  C_4  M\bigg(\sigma_{\epsilon}^2 \s\log(np)  +    \tr \kappa^2
+   \gamma \bigg),
\end{align}
where the equality follows from the fact that  $\mu^*_i$ is unchanged in any of $\{ \J_m\}_{m=0}^{M+1}$, and
 the inequality follows from \Cref{eq:1D three change points step 1} and 
\Cref{eq:1D three change points second}.
\\
\\
{\bf Step 3.}
For any $  m \in\{2, \ldots, M\}$, it holds that
\begin{align}  \label{eq:1D three change points signal lower bound} \inf_{ a \in \mathbb R  }  |\J_{m-1} |\|a - \mu^*_{\J_{m-1} }\|_2^2 + |\J_{m} |\|a  - \mu^*_{\J_{m} }\|_2^2  =&     \frac{|\J_{m-1}| |\J_m|}{ |\J_{m-1}| +  |\J_m| } \kappa_m ^2  \ge \frac{1}{2} \Delta \kappa^2,
\end{align}  
where the last inequality follows from the assumptions that $\eta_k - \eta_{k-1}\ge \Delta  $ and $ \kappa_k \asymp \kappa$  for all $1\le k \le K$. So
\begin{align}   \nonumber &2 \sum_{ m=1}^{M }   |\J_m |\|\widehat \mu_\I  - \mu^*_{\J_  m  }\|_2^2   
\\ 
\ge &  \nonumber    \sum_{m=2}^M  \bigg(  |\J_{m-1}  | \|\widehat \mu_\I  - \mu^*_{\J_ { m-1}  }\|_2^2   + |\J_m |\|\widehat \mu_\I  - \mu^*_{\J_  m  }\|_2^2   \bigg) 
\\ \label{eq:1D three change points signal lower bound two} 
\ge & (M-1)  \frac{ 1}{2} \Delta \kappa^2  \ge \frac{M}{4} \Delta \kappa^2 ,
\end{align} 
where the second inequality follows from  \Cref{eq:1D three change points signal lower bound} and the last inequality follows from $M\ge 3$. \Cref{eq:1D three change points third} and  \Cref{eq:1D three change points signal lower bound two} together imply that 
\begin{align}\label{eq:1D three change points signal lower bound three} 
 \frac{M}{4} \Delta \kappa^2 \le 2  C_4  M\bigg(\sigma_{\epsilon}^2 \s\log(np) + \tr \kappa^2 + \gamma \bigg) .
\end{align}
Since $\Bn\to \infty $, it follows that for sufficiently large $n$,   \Cref{eq:1D three change points signal lower bound three} gives 
$$ \Delta\kappa^2 \le C_5 \big(\sigma_{\epsilon}^2 \s\log(np) +\gamma),$$  
which contradicts \Cref{eq:1D three change points snr}.
 \end{proof} 
 
 
 
 \bnlem Suppose $ \gamma \ge C_\gamma K\tr \kappa^2 $ for sufficiently large constant $C_\gamma $. 
With probability  at least $1-(np)^{-3}$,    there are no  two consecutive intervals $\I_1= (s,t ] \in \widehat {\mathcal  P}  $,   $ \I_2=(t, e]  \in   \widehat  {\mathcal  P}  $    such that $\I_1 \cup \I_2$ contains no change points.  
 \enlem 
 \begin{proof} 
 For contradiction, suppose that 
 $$ \I :  =\I_1\cup  \I_2 $$
 contains no change points. 
 Since 
 $ s,t,e \in \{ s_q\}_{q=1}^\Q $, it follows that
 $$ \sum_{i\in \I_1} \|X_i - \widehat \mu_{\I_1}\|^2  +\sum_{i\in \I_2} \|X_i - \widehat \mu_{\I_2}\|_2^2 +\gamma  \le \sum_{i\in \I } \|X_i - \widehat \mu_{\I }\|_2^2. $$
 By \Cref{lem:mean one change deviation bound}, it follows that 
\begin{align*} 
& \sum_{i\in \I_1} \|X_i - \mu^*_i\|_2^2 \le  C_1 \sigma_{\epsilon}^2\s\log(np) +  \sum_{i\in \I_1} \|X_i - \widehat \mu_{\I_1}\|_2^2 ,
 \\
 & \sum_{i\in \I_2} \|X_i - \mu^*_i\|_2^2 \le  C_1 \sigma_{\epsilon}^2\s\log(np) +  \sum_{i\in \I_2} \|X_i - \widehat \mu_{\I_2}\|_2^2
  \\
  & \sum_{i\in \I} \|X_i - \widehat{\mu}_{\I}\|_2^2 \le  C_1 \sigma_{\epsilon}^2\s\log(np) + \sum_{i\in \I} \|X_i - \mu_{i}^*\|_2^2.
 \end{align*} 
 So 
 $$\sum_{i\in \I_1} \|X_i - \mu^*_i\|_2^2  +\sum_{i\in \I_2}\|X_i - \mu^*_i\|_2^2 -2C_1 \sigma_{\epsilon}^2\s\log(np) +\gamma    \le \sum_{i\in \I }\|X_i - \mu^*_i\|_2^2 +C_1\sigma_{\epsilon}^2\s\log(np) .  $$
 Since $\mu^*_i$ is unchanged when $i\in \I$, it follows that 
 $$ \gamma \le 3C_1\sigma_{\epsilon}^2\s\log(np).$$
 This is a contradiction when $C_\gamma> 3C_1. $
 \end{proof} 
 


























%%%% location indicator %%%%
%%%% start of covariance part %%%%
\clearpage
\subsection{Covariance model}


\bnprop\label{prop:covariance local consistency}
 Suppose  \Cref{assp:DCDP_covariance} holds. Let 
 $\widehat { \mathcal P }  $ denote the output of DP.
 Then with probability  at least $1 - C n ^{-3}$, the following conditions hold.
	\begin{itemize}
		\item [(i)] For each interval  $ \I = (s, e] \in \widehat{\mathcal{P}}$    containing one and only one true 
		   change point $ \eta_k $, it must be the case that
 $$\min\{ \eta_k -s ,e-\eta_k \}  \lesssim  C_{\gamma} \|X\|_{\psi_2}^4\frac{C_X^2}{c_X^6}\frac{p^2\log(np)}{\kappa_k^2} +\|X\|_{\psi_2}^4\frac{C_X^6}{c_X^6}\tr .$$
		\item [(ii)] For each interval  $  \I = (s, e] \in \widehat{\mathcal{P}}$ containing exactly two true change points, say  $\eta_ k  < \eta_ {k+1} $, it must be the case that
			\begin{align*} 
 \eta_k -s    \lesssim \htr    \quad \text{and} \quad 
 e-\eta_{k+1}  \lesssim  \htr. 
 \end{align*} 
		 
\item [(iii)] No interval $\I \in \widehat{\mathcal{P}}$ contains strictly more than two true change points; and 


	\item [(iv)] For all consecutive intervals $ \I_1 $ and $ \I_2 $ in $\widehat{ \mathcal P}$, the interval 
		$ \I_1 \cup  \I_2 $ contains at least one true change point.
				
	 \end{itemize}
\enprop 
\bprf
The four cases are proved in \Cref{lem:cov no cp}, \Cref{lem:cov single cp}, \Cref{lem:cov two cp}, and \Cref{lem:cov two consecutive interval}.
\eprf








\bnprop\label{prop:change points partition size consistency}
Suppose  \Cref{assp:DCDP_covariance} holds. Let 
 $\widehat { \mathcal P }  $ be the output of DP. Suppose 
$ \gamma \ge C_\gamma K\tr \kappa^2 $  for sufficiently large constant $C_\gamma$. Then
 with probability  at least $1 - C n ^{-3}$,  $| \widehat { \mathcal P} | =K $.
\enprop



\begin{proof}[Proof of   \Cref{prop:change points partition size consistency}] 
Denote $\mathfrak{G} ^*_n = \sum_{ i =1}^n [{\rm Tr}[(\Omega_i^*)^\top X_iX_i^\top] - \log|\Omega_i^*|]$. Given any collection $\{t_1, \ldots, t_m\}$, where $t_1 < \cdots < t_m$, and $t_0 = 0$, $t_{m+1} = n$, let 
\begin{equation}\label{eq-sn-def}
	\G _n(t_1, \ldots, t_{m}) = \sum_{k=1}^{m} \sum_{ i = t_k +1}^{t_{k+1}} \mclF(\widehat {\Omega}_{(t_{k}, t_{k+1}]}, (t_{k}, t_{k+1}]).
\end{equation}
For any collection of time points, when defining \eqref{eq-sn-def}, the time points are sorted in an increasing order.

Let $\{ \widehat \eta_{k}\}_{k=1}^{\widehat K}$ denote the change points induced by $\widehat {\mathcal P}$.  Suppose we can justify that 
	\begin{align}
		\G^*_n + K\gamma  \ge  &\G _n(s_1,\ldots,s_K)   + K\gamma - C(K + 1)\frac{\|X\|_{\psi_2}^2}{c_{X}^4}\frac{ p^2\log(np)}{\kappa^2} - C\sum{k\in [K]}\kappa_k^2\mclB_n^{-1}\Delta \label{eq:cov K consistency step 1} \\ 
		\ge & \G_n (\widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } ) +\widehat K \gamma - C_1'(K + 1)\frac{\|X\|_{\psi_2}^2}{c_{X}^4}\frac{ p^2\log(np)}{\kappa^2} - C_1'\sum{k\in [K]}\kappa_k^2\mclB_n^{-1}\Delta  \label{eq:cov K consistency step 2} \\ 
		\ge &  \G _n ( \widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K ) + \widehat K \gamma    - C_1(K + 1)\frac{\|X\|_{\psi_2}^2}{c_{X}^4}\frac{ p^2\log(np)}{\kappa^2} - C_1\sum{k\in [K]}\kappa_k^2\mclB_n^{-1}\Delta \label{eq:cov K consistency step 3}
	\end{align}
	and that 
	\begin{align}\label{eq:cov K consistency step 4}
		\G ^*_n   -\G _n ( \widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K ) \le C_2 (K + \widehat{K} + 2) \frac{\|X\|_{\psi_2}^4}{c_X^2} p^2\log(np).
	\end{align}
	Then it must hold that $| \widehat{\mclP} | = K$, as otherwise if $\widehat K \geq K+1 $, then  
	\begin{align*}
		C _2 (K + \widehat{K} + 2)  \frac{\|X\|_{\psi_2}^4}{c_X^2} p^2\log(np)  & \ge   \G ^*_n  -\G _n ( \widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K ) \\
		& \ge      (\widehat K - K)\gamma  -C_1 ( K +1)  \frac{\|X\|_{\psi_2}^4}{c_X^2} p^2\log(np).
	\end{align*} 
	Therefore due to the assumption that $| \widehat{\mclP}|=\widehat K\leq 3K $, it holds that 
	\begin{align} \label{eq:cov Khat=K} 
		[C_2 (4K + 2) + C_1(K+1)] \frac{\|X\|_{\psi_2}^4}{c_X^2} p^2\log(np) \geq  (\widehat K - K)\gamma \geq \gamma.
	\end{align}
	Note that \eqref{eq:cov Khat=K} contradicts the choice of $\gamma$. Therefore, it remains to show \Cref{eq:cov K consistency step 1} to \Cref{eq:cov K consistency step 4}.

{\bf Step 1.} \Cref{eq:cov K consistency step 1} holds because $\widehat{\Omega}_{\I}$ is (one of) the minimizer of $\F(\Omega, \I)$ for any interval $\I$.

{\bf Step 2.} \Cref{eq:cov K consistency step 2} is guaranteed by the definition of $\widehat{\mclP}$.

{\bf Step 3.} For every $ \I  =(s,e]\in \widehat{\mclP}$, by \Cref{prop:covariance local consistency}, we know that $\I$ contains at most two change points. We only show the proof for the two-change-points case as the other case is easier. Denote
	\[
		 \I =  (s ,\eta_{q}]\cup (\eta_{q},\eta_{q+1}] \cup  (\eta_{q+1} ,e]  = \J_1 \cup \J_2 \cup \J_{3},
	\]
where $\{ \eta_{q},\eta_{q+1}\} =\I \, \cap \, \{\eta_k\}_{k=1}^K$. 

For each $ m=1,2,3$, by definition it holds that
\begin{equation}
    \mclF(\widehat\Omega_{\J_m},\J_m)\leq \mclF(\Omega^*_{\J_m},\J_m).
\end{equation}
On the other hand, by \Cref{lem:cov loss deviation no change point}, we have
$$
\mclF(\widehat\Omega_{\I},\J_m)   \geq \mclF(\Omega^*_{\J_m},\J_m) - C\frac{\|X\|_{\psi_2}^4}{c_X^2}p^2\log(np). 
$$
Therefore the last two inequalities above imply that 
\begin{align} 
\sum_{i \in \I }  \mclF(\widehat \Omega_\I,\I) \geq & \sum_{m=1}^{3} \sum_{ i \in \J_m }\mclF(\widehat \Omega_\I,\J_m) \nonumber \\
\geq & \sum_{m=1}^{3}   \sum_{ i \in \J_m}\mclF(\widehat \Omega_{\J_m},\J_m) - C\frac{\|X\|_{\psi_2}^4}{c_X^2}p^2\log(np). \label{eq:cov K consistency step 3 inequality 3}
\end{align}
Then \eqref{eq:cov K consistency step 3} is an immediate consequence of \eqref{eq:cov K consistency step 3 inequality 3}.

{\bf Step 4.}
Finally, to show \eqref{eq:cov K consistency step 4},   let  $\widetilde { \mathcal P}$ denote    the partition induced by $\{\widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K\}$. Then 
$| \widetilde { \mathcal P} | \le K + \widehat K+2   $ and that $\Omega^*_i$ is unchanged in every interval $\I \in \widetilde { \mathcal P}$. So \Cref{eq:cov K consistency step 4} is an immediate consequence of \Cref{lem:cov no cp}.
\end{proof} 








\subsubsection{Technical lemmas}





\bnlem
\label{lem:estimation covariance}
Let $\{X_i\}_{i\in [n]}$ be a sequence of subgaussian vectors in $\mathbb{R}^{p}$ with orlitz norm upper bounded $\|X\|_{\psi_2}<\infty$. Suppose $\mathbb{E}[X_i] = 0$ and $\mathbb{E}[X_iX_i^\top] = \Sigma_i$ for $i\in [n]$. Consider the change point setting in \Cref{assp:DCDP_covariance} and consider a generic interval $\I\subset [1,n]$. Let $\widehat{\Sigma}_{\I} = \frac{1}{|\I|}\sum_{i \in \I} X_i X_i^\top$ and $\Sigma_{\I} = \frac{1}{|\I|}\Sigma^*_i$. Then for any $u>0$, it holds with probability at least $1 - \exp(-u)$ that
\begin{equation}
    \|\widehat{\Sigma}_{\I} - \Sigma_{\I}\|_2\lesssim \|X\|_{\psi_2}^2(\sqrt{\frac{p + u}{n}}\vee \frac{p + u}{n}).
\end{equation}
As a corollary, when $n\geq C_s p\log(np)$ for some universal constant $C_s>0$, it holds with probability at least $1 - (np)^{-7}$ that
\begin{equation}
    \|\widehat{\Sigma}_{\I} - \Sigma_{\I}\|_2\leq C\|X\|_{\psi_2}^2\sqrt{\frac{p\log(np)}{|\I|}},
\end{equation}
where $C$ is some universal constant that does not depend on $n, p, \|X\|_{\psi_2}$, and $C_s$. In addition let $\widehat{\Omega}_{\I} = \argmin_{\Omega\in \mathbb{S}_+}L(\Omega,\I)$ and $\widetilde{\Omega}_{\I} = (\frac{1}{|\I|}\sum_{i\in\I}\Sigma^*_i)^{-1}$. if $|\I|\geq C_s p\log(np)\|X\|_{\psi_2}^4 / c_X^2$ for sufficiently large constant $C_s>0$, then it holds with probability at least $1 - (np)^{-7}$ that
\begin{equation}
    \|\widehat{\Omega}_{\I} -\widetilde{\Omega}_{\I}\|_2\leq C \frac{\|X\|_{\psi_2}^2}{c_X^2}\sqrt{\frac{p\log(np)}{|\I|}}.
\end{equation}
\enlem
\bprf
Vanishing the gradient of the loss function $L(\Omega, \I)$ gives
\begin{equation*}
    \widehat{\Omega}_{\I} = (\widehat{\Sigma}_{\I})^{\dagger}.
\end{equation*}
\eprf









\bnlem[Covariance model]
\label{lem:cov one change deviation bound}
Let $\mathcal I =(s,e] $ be any generic interval, and define the loss function $L(\Omega, \I) = \sum_{i\in \I}{\rm Tr}[\Omega^\top (X_iX_i^\top)] - |\I|\log|\Omega|$ and goodness-of-fit function $\mclF(\Omega, \I) = L(\Omega,\I)$. Define $\widehat{\Omega}_{\I} = \argmin_{\Omega\in \mathbb{S}_+}L(\Omega,\I)$ and $\mclF^*(\I) = \sum_{i\in \I}[{\rm Tr}((\Omega_i^*)^\top (X_iX_i^\top)) - \log|\Omega_i^*|]$.

{\bf a.} If $\I$ contains no change points. Then it holds that 
$$\mathbb{P} \bigg( |   \mclF(\widehat{\Omega}_{\I},\I)  - \mclF^*(\I) |  \ge C \frac{\|X\|_{\psi_2}^4}{c_X^2}p^2\log(np)  \bigg)  \le  (np)^{-3}. $$

{\bf b.}  Suppose that the interval $ \I=(s,e]$ contains one and only one change point $ \eta_k $. Denote
$$  \mathcal J = (s,\eta_k] \quad \text{and} \quad  \mathcal J' =  (\eta_k, e].$$ 
Then it holds that 
$$\mathbb{P} \bigg( | \mclF(\widehat{\Omega}_{\I},\I) - \mclF^*(\I)  | \geq \frac{C_X^2p}{c_X^8}\frac{|\J||\J '| }{|\I|}\kappa_k^2 +  C\frac{\|X\|_{\psi_2}^4 C_X^2}{c_X^4}p^2\log(np) \bigg)   \le  (np)^{-3}. $$
\enlem
\begin{proof} 
We show {\bf b} as {\bf a} immediately follows from {\bf b} with $ |\J'| =0$. Denote 
$$  \mathcal J = (s,\eta_k] \quad \text{and} \quad  \mathcal J' =  (\eta_k, e]  .$$ 
Let $\widetilde{\Omega}_{\I} = (\frac{1}{|\I|}\sum_{i\in\I}\Sigma_i^*)^{-1}$.
Then by Taylor expansion and \Cref{lem:estimation covariance}, we have
\begin{align}
    & |\mclF(\widehat{\Omega}_{\I},\I)-\mclF(\widetilde{\Omega}_{\I},\I)| \nonumber \\
    \leq & |{\rm Tr}[(\widehat{\Omega}_{\I} - \widetilde{\Omega}_{\I})^\top (\sum_{i\in\I} X_iX_i^\top - |\I|\widetilde{\Omega}_{\I}^{-1})]| + \frac{C_X^2}{2}|\I|\|\widehat{\Omega}_{\I} - \widetilde{\Omega}_{\I}\|_F^2 \nonumber \\
    \leq & |\I|\|\widehat{\Omega}_{\I} - \widetilde{\Omega}_{\I}\|_F \|\widehat{\Sigma}_{\I} - \widetilde{\Omega}_{\I}^{-1}\|_F + \frac{C_X^2}{2}|\I|\|\widehat{\Omega}_{\I} - \widetilde{\Omega}_{\I}\|_F^2 \nonumber\\
    \leq & C\frac{\|X\|_{\psi_2}^4}{c_X^2}p^2\log(np) + C\frac{\|X\|_{\psi_2}^4 C_X^2}{c_X^4}p^2\log(np)\leq C\frac{\|X\|_{\psi_2}^4 C_X^2}{c_X^4}p^2\log(np). \label{eq:cov mixed deviation 1}
\end{align}
On the other hand, it holds that
\begin{align}
    & |\mclF(\widetilde{\Omega}_{\I},\I)-\mclF^*(\I)| \nonumber \\
    \leq & |{\rm Tr}[(\widetilde{\Omega}_{\I} - {\Omega}_{\J})^\top (\sum_{i\in\J} X_iX_i^\top - |\J|\Omega_{\J}^{-1})]| + \frac{C_X^2}{2}|\J|\|\widetilde{\Omega}_{\I} - {\Omega}_{\J}\|_F^2 \nonumber\\
     & + |{\rm Tr}[(\widetilde{\Omega}_{\I} - {\Omega}_{\J '})^\top (\sum_{i\in\J'} X_iX_i^\top - |\J '|\Omega_{\J '}^{-1})]| + \frac{C_X^2}{2}|\J '|\|\widetilde{\Omega}_{\I} - {\Omega}_{\J '}\|_F^2.\label{eq:cov mixed deviation 2}
\end{align}
To bound $\|\widetilde{\Omega}_{\I} - {\Omega}_{\J}\|_F$ and $\|\widetilde{\Omega}_{\I} - {\Omega}_{\J '}\|_F$, notice that for two positive definite matrices $\Sigma_1,\Sigma_2\in \mathbb{S}_+$ and two positive numbers $w_1,w_2$ such that $w_1 + w_2 = 1$, we have
\begin{align*}
    & \|(w_1\Sigma_1 + w_2\Sigma_2)^{-1} - \Sigma_1^{-1}\|_F\\
    \leq &\sqrt{p}\|(w_1\Sigma_1 + w_2\Sigma_2)^{-1} - \Sigma_1^{-1}\|_2\\
    = &\sqrt{p}\|(w_1\Sigma_1 + w_2\Sigma_2)^{-1}[\Sigma_1 - (w_1\Sigma_1 + w_2\Sigma_2)]\Sigma_1^{-1}\|_2\\
    \leq & \sqrt{p}\|(w_1\Sigma_1 + w_2\Sigma_2)^{-1}\|_2\|\Sigma_1 - (w_1\Sigma_1 + w_2\Sigma_2)\|_2\|\Sigma_1^{-1}\|_2\\
    \leq & \|(w_1\Sigma_1 + w_2\Sigma_2)^{-1}\|_2\|\Sigma_1^{-1}\|_2\cdot\sqrt{p}w_2\|\Sigma_1 - \Sigma_2\|_2 \\
    \leq & \|(w_1\Sigma_1 + w_2\Sigma_2)^{-1}\|_2\|\Sigma_1^{-1}\|_2\|\Sigma_1\|_2\|\Sigma_2\|_2\cdot\sqrt{p}w_2\|\Sigma_1^{-1} - \Sigma_2^{-1}\|_2.
\end{align*}
Therefore, under \Cref{assp:DCDP_covariance}, it holds that
\begin{equation}
    \|\widetilde{\Omega}_{\I} - {\Omega}_{\J}\|_F\leq \frac{C_X^2}{c_X^2}\frac{|\J '|}{|\I|}\sqrt{p}\kappa_k, \|\widetilde{\Omega}_{\I} - {\Omega}_{\J '}\|_F\leq \frac{C_X^2}{c_X^2}\frac{|\J|}{|\I|}\sqrt{p}\kappa_k,
\end{equation}
where in the second inequality we use the fact that $2ab\leq a^2+ b^2$. As a consequence, \Cref{eq:cov mixed deviation 2} can be bounded as
\begin{align}
     & |\mclF(\widetilde{\Omega}_{\I},\I)-\mclF^*(\I)| \nonumber \\
    \leq & C\frac{\|X\|_{\psi_2}^2p\sqrt{\log(np)}}{c_X^2C_X^{-2}}\kappa_k(\frac{|\J '||\J|^{\frac{1}{2}}}{|\I|} + \frac{|\J '|^{\frac{1}{2}}|\J|}{|\I|}) + \frac{C_X^6 p}{2c_X^4}\kappa_k^2(\frac{|\J||\J '|^2 }{|\I|^2} + \frac{|\J '||\J|^2 }{|\I|^2}) \nonumber\\
    \leq & C\frac{\|X\|_{\psi_2}^4p^2{\log(np)}}{C_X^2} + \frac{C_X^6p}{c_X^4}\frac{|\J||\J '| }{|\I|}\kappa_k^2.\label{eq:cov mixed deviation 3}
\end{align}
Combine \Cref{eq:cov mixed deviation 1} and \Cref{eq:cov mixed deviation 3} and we can get
\begin{equation*}
    \begin{split}
        |\mclF(\widehat{\Omega}_{\I},\I) - \mclF^*(\I)|
        \leq & |\mclF(\widehat{\Omega}_{\I},\I)-\mclF({\Omega}_{\I},\I)| +|\mclF({\Omega}_{\I},\I) - \mclF^*(\I)|\\
        \leq& C\frac{\|X\|_{\psi_2}^4 C_X^2}{c_X^4}p^2\log(np) + \frac{C_X^6 p}{c_X^4}\frac{|\J||\J '| }{|\I|}\kappa_k^2.
    \end{split}
\end{equation*}
\end{proof} 

\bnrmk
It can be seen later that the $p$ factor in the signal term $\frac{C_X^6 p}{c_X^4}\frac{|\J||\J '| }{|\I|}\kappa_k^2$ will require an additional $p$ factor in the number of points in the grid for DCDP, leading to an additional $p^2$ factor in the computation time.

This factor is hard to remove because it is rooted in the approximation error
$$
\|(w_1\Sigma_1 + w_2\Sigma_2)^{-1} - \Sigma_1^{-1}\|_F.
$$
We can try another slightly neater way of bounding this term. As is mentioned in \cite{kereta2021ejs}, for two matrices $\mathbf{G}, \mathbf{H}\in \mathbb{R}^{d_1\times d_2}$, it holds that
$$
\left\|\mathbf{H}^{\dagger}-\mathbf{G}^{\dagger}\right\|_F \leq \min \left\{\left\|\mathbf{H}^{\dagger}\right\|_2\left\|\mathbf{G}^{\dagger} (\mathbf{H}-\mathbf{G})\right\|_F,\left\|\mathbf{G}^{\dagger}\right\|_2\left\|\mathbf{H}^{\dagger} (\mathbf{H}-\mathbf{G})\right\|_2\right\},
$$
if $\operatorname{rank}(\mathbf{G})=\operatorname{rank}(\mathbf{H})=\min \left\{d_1, d_2\right\}$. Therefore, we have
\begin{align*}
    \|(w_1\Sigma_1 + w_2\Sigma_2)^{-1} - \Sigma_1^{-1}\|_F\leq & \|(w_1\Sigma_1 + w_2\Sigma_2)^{-1}\|_2\|\Sigma_{1}^{-1}(w_1\Sigma_1 + w_2\Sigma_2 - \Sigma_1)\|_F\\
    \leq & \|(w_1\Sigma_1 + w_2\Sigma_2)^{-1}\|_2\|\Sigma_{1}^{-1}\|w_2\|\Sigma_2 - \Sigma_1\|_F.
\end{align*}
However, to relate $\|\Sigma_2 - \Sigma_1\|_F$ to $\|\Sigma_2^{-1} - \Sigma_1^{-1}\|_F$, we need to proceed in the following way:
\begin{align*}
    \|\Sigma_2 - \Sigma_1\|_F\leq & \sqrt{d}\|\Sigma_2 - \Sigma_1\|_2 \\
    \leq & \|\Sigma_1\|_2\|\Sigma_2\|_2 \cdot \sqrt{d}\|\Sigma_2^{-1} - \Sigma_1^{-1}\|_2\\
    \leq & \|\Sigma_1\|_2\|\Sigma_2\|_2 \cdot \sqrt{d}\|\Sigma_2^{-1} - \Sigma_1^{-1}\|_F,
\end{align*}
which leads to the same bound in \Cref{lem:cov one change deviation bound}.
\enrmk

















\bnlem[No change point]
\label{lem:cov no cp}
For interval $\mclI$ containing no change point, it holds with probability at least $1 - n^{-5}$ that
\begin{equation}
    \F(\widehat{\Omega}_{\I}, \mclI) -\F({\Omega}^*, \mclI) \geq -\|X\|_{\psi_2}^4 p^2\log(np)\max_{k\in[K + 1]}\|\Omega^*_{\eta_k}\|_2^2.
\end{equation}
\enlem
\bprf
If $\I< C_s\frac{\|X\|_{\psi_2}^4}{c_X^2}p\log(np)$, then $\F(\widehat{\Omega}_{\I}, \mclI) =\F({\Omega}^*, \mclI)=0$ and the conclusion holds automatically. If $\I\geq C_s\frac{\|X\|_{\psi_2}^4}{c_X^2}p\log(np)$, then by \Cref{lem:estimation covariance}, it holds with probability at least $1 - n^{-7}$ that
\begin{align}
\F(\widehat{\Omega}_{\I}, \mclI) -\F({\Omega}^*, \mclI) \geq & |\mclI|{\rm Tr}[(\widehat{\Omega}_{\I} - \Omega^*)^\top (\widehat{\Sigma}_{\I} - \Sigma^*)] + \frac{c|\mclI|}{2\|\Omega^*\|_2^2}\|\widehat{\Omega}_{\I} - \Omega^*\|_F^2.    \\
\geq & -|\mclI|\|\widehat{\Omega}_{\I} - \Omega^*\|_F \|\widehat{\Sigma}_{\I} - \Sigma^*\|_F \\
\geq & -|\mclI|p \|\widehat{\Omega}_{\I} - \Omega^*\|_2 \|\widehat{\Sigma}_{\I} - \Sigma^*\|_2\\
\geq & -\|X\|_{\psi_2}^4 p^2\log(np)\|\Omega^*\|_2^2.
\end{align}
\eprf




\bnlem
\label{lem:cov loss deviation no change point}
Let $\I\subset [1,T]$ be any interval that contains no change point. Then for any interval $\J \supset \I$, it holds with probability at least $1 - (np)^{-5}$ that
\begin{equation*}
    \mclF(\Omega^*_{\I},\I)\leq \mclF(\widehat{\Omega}_\J,\I) + C\frac{\|X\|_{\psi_2}^4}{c_X^2}p^2\log(np).
\end{equation*}
\enlem
\begin{proof}
The conclusion is guaranteed by \Cref{lem:cov no cp} and the fact that $\F(\Omega,\I) = L(\Omega,\I)$ and $\widehat{\Omega}_{\I}$ is (one of) the minimizer of $L(\Omega,\I)$.
\end{proof}









\bnlem[Single change point]
\label{lem:cov single cp}
Suppose the good events 
$\mathcal L (\tr ) $ and  $\mathcal R (\tr) $ defined  in \Cref{eq:left and right approximation of change points} hold. 
Let   $ \I=(s,e] \in \mathcal {\widehat P}  $  be such that $\I$ contains exactly  one    change point $ \eta_k $. 
 Then  with probability  at least $1-(np)^{-3}$,   it holds that 
\begin{equation}
    \min\{ \eta_k -s ,e-\eta_k \} \leq CC_{\gamma} \|X\|_{\psi_2}^4\frac{C_X^2}{c_X^6}\frac{p^2\log(np)}{\kappa_k^2} + C\|X\|_{\psi_2}^4\frac{C_X^6}{c_X^6}\tr.
\end{equation}
\enlem
\bprf
If either $ \eta_k -s \le \tr  $ or $e-\eta_k\le \tr$, then there is nothing to show. So assume that 
$$  \eta_k -s  > \tr \quad \text{and} \quad   e-\eta_k  > \tr . $$
By event $\mathcal R (p^{-1}\tr )$, there exists  $ s_ u  \in \{ s_q\}_{q=1}^\Q$ such that 
$$0\le s_u - \eta_k \le p^{-1}\tr. $$
 So 
$$ \eta_k \le s_ u \le e .$$
Denote 
$$ \I_ 1 = (s,s_u] \quad \text{and} \quad \I_2 = (s_u, e],$$
and $\mclF^*(\J) = \sum_{i\in \J}[{\rm Tr}((\Omega^*_i)^\top X_iX_i^\top) -\log|\Omega_i^*|]$. Since
$s, e,  s_u \in  \{ s_q\}_{q=1}^\Q  $, by the definition of $\widehat{P}$ and $\widehat{\Omega}$, and \Cref{lem:cov one change deviation bound}, it holds that
\begin{align}
    \mclF(\widehat{\Omega}_{\I},\I)\leq& \mclF(\widehat{\Omega}_{\I_1},\I_1) + \mclF(\widehat{\Omega}_{\I_2},\I_2) + \gamma \nonumber \\
    \leq & \mclF^*(\I_1) + \frac{C_X^6 p}{c_X^4}(s_u - \eta_k)\kappa_k^2 +  C\frac{\|X\|_{\psi_2}^4 C_X^2}{c_X^4}p^2\log(np) + \mclF^*(\I_2) + \gamma \nonumber \\
    \leq & \mclF^*(\I) + \frac{C_X^6}{c_X^4}\mclB_n^{-1}\Delta\kappa_k^2 +  C\frac{\|X\|_{\psi_2}^4 C_X^2}{c_X^4}p^2\log(np) +  \gamma,
\end{align}
where the last inequality is due to $s_u - \eta_k\leq \mclB_n^{-1}\Delta$. Let 
$$\widetilde{\gamma} = \frac{C_X^6}{c_X^4}\mclB_n^{-1}\Delta\kappa_k^2 +  C\frac{\|X\|_{\psi_2}^4 C_X^2}{c_X^4}p^2\log(np) +  \gamma.$$ 
Then by Taylor expansion and \Cref{lem:estimation covariance} we have
\begin{align}
    \frac{c}{\max_{k\in [K]}\|\Omega_{\I_k}^*\|_2^2}\sum_{t\in \mclI}\|\widehat{\Omega}_{\I} - \Omega^*_t\|_F^2 
    &\leq \widetilde{\gamma} + \sum_{i=k-1}^k|\I_i|{\rm Tr}[(\Omega_{\I_i}^* - \widehat{\Omega}_{\I})^\top (\widehat{\Sigma}_{\I_i}  - \Sigma^*_{\I_i})] \nonumber \\
    &\leq \widetilde{\gamma} + \sum_{i=k-1}^k {|\mclI_{i}|}\|\widehat{\Sigma}_{\I_i} - \Sigma^*_{\I_i}\|_F\|\widehat{\Omega}_{\I} - \Omega^*_{\I_i}\|_F \nonumber \\
    &\leq \widetilde{\gamma} + C_1\|X\|_{\psi_2}^2 p\log^{\frac{1}{2}}(np)\left[ \sum_{i=k-1}^k \sqrt{|\mclI_{i}|}\|\widehat{\Omega}_{\I} - \Omega^*_{\I_i}\|_F \right] \nonumber \\
    &\leq \widetilde{\gamma} + C_1\|X\|_{\psi_2}^2 p\log^{\frac{1}{2}}(np) \sqrt{\sum_{t\in \mclI}\|\widehat{\Omega}_{\I} - \Omega^*_t\|_F^2}.
\end{align}
The inequality above implies that
\begin{equation}
    \sum_{t\in \mclI}\|\widehat{\Omega}_{\I} - \Omega^*_t\|_F^2 \leq \frac{2}{c}\max\|\Omega_{\I_k}^*\|_2^2\left[\widetilde{\gamma} + \max\|\Omega_{\I_k}^*\|_2^2\|X\|^4_{\psi_2} p^{2}\log(np)\right].
\end{equation}
On the other hand,
\begin{equation}
    \sum_{t\in \mclI}\|\widehat{\Omega}_{\I} - \Omega^*_t\|_F^2\geq \frac{|\mclI_{k-1}||\mclI_{k}|}{|\mclI|}\|\Omega^*_{\I_{k-1}} - \Omega^*_{\I_k}\|_F^2,
\end{equation}
which implies that
\begin{equation}
    \min\{|\mclI_{k-1}|,|\mclI_{k}|\}\leq C_2C_{\gamma} \|X\|_{\psi_2}^4\frac{C_X^2}{c_X^6}\frac{p^2\log(np)}{\kappa_k^2} + C_2\|X\|_{\psi_2}^4\frac{C_X^6}{c_X^6}\tr.
\end{equation}
\eprf



\bnlem[Two change point]
\label{lem:cov two cp}
Suppose the good events 
$\mathcal L (\tr ) $ and  $\mathcal R ( \tr ) $ defined  in  \Cref{eq:left and right approximation of change points} hold. Let   $ \I=(s,e] \in \mathcal {\widehat P}  $  be an interval that contains exactly two change points $ \eta_k,\eta_{k+1}$. Suppose in addition that $\gamma \geq C_{\gamma}\|X\|_{\psi_2}^4\max_{k\in [K]}\|\Omega_{\I_k}^*\|_2^2p^2\log(np)$, and
\begin{equation}
    \Delta \kappa^2 \geq \mathcal{B}_n \frac{\|X\|_{\psi_2}^4}{c_X^4}p^2\log(np),
\end{equation}
then it holds with probability at least $1 - n^{-5}$ that
\begin{equation}
    \max\{\eta_k - s, e - \eta_{k + 1}\}\leq \htr.
\end{equation}
\enlem
\bprf
Since the events $\mathcal L ( \tr  ) $ and  $\mathcal R ( \tr ) $ hold, let $ s_u, s_v$ be such that 
 $\eta_k \le s_u \le s_v \le \eta_{k+1} $ and that 
 $$ 0 \le s_u-\eta_k \le   \tr ,  \quad  0\le  \eta_{k+1} - s_v \le \tr   .    $$

 \begin{center}
 \begin{tikzpicture} 
\draw[ - ] (-10,0)--(1,0);
 \node[color=black] at (-8,-0.3) {\small s};
 \draw[  (-, ultra thick, black] (-8,0) -- (-7.99,0);
  \draw[ { -]}, ultra thick, black] (-1.0002,0) -- (-1,0);

   \node[color=black] at (-7,-0.3) {\small $\eta_k$};
\draw(-7 ,0)circle [radius=2pt] ;

  \node[color=black] at (-6.5,-0.3) {\small $s_u$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-6.5,0)  }; 
 

  \node[color=black] at (-2.3,-0.3) {\small $\eta_{k+1}$};
\draw(-2.3 ,0)circle [radius=2pt] ;
  \node[color=black] at (-3 ,-0.3) {\small $s_v$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-3,0)  }; 
  
   \node[color=black] at (-1,-0.3) {\small $e$};

 
\end{tikzpicture}
\end{center} 

Denote 
$$ \mathcal I_ 1= (  s, s _u], \quad \I_2  =(s_u, s_v] \quad \text{and} \quad \I_3  = (s_v,e]. $$
In addition, denote 
$$ \J_1  = (s,\eta_k ], \quad \J_2=(\eta_k, \eta_{k} + \frac{ \eta_{k+1}   -\eta_k  }{2}], \quad \J_3 =  ( \eta_k+ \frac{ \eta_{k+1}   -\eta_k  }{2},\eta_{k+1 } ]  \quad \text{and} \quad \J_4 = (\eta_{k+1}  , e] .$$
Since 
$s, e,  s_u ,s_v  \in  \{ s_q\}_{q=1}^\Q  $, by the event $\mclL(p^{-1}\tr)$ and $\mclR(p^{-1}\tr)$, it holds with probability at least $1 - n^{-3}$ that
$$
0\leq s_u - \eta_k\leq p^{-1}\tr,\ 0\leq \eta_{k+1} - s_v\leq p^{-1}\tr.
$$
Denote
$$\I_1 = (s ,\eta_k], \I_2 = (\eta_k, \eta_{k + 1}], \I_3 = (\eta_{k + 1}, e].$$
By the definition of DP and $\widehat{\Omega}_{\I}$, it holds that
\begin{align}
        \F(\hat{\Omega}_{\I},\I)
        \leq & \sum_{i = 1}^3 \F(\hat{\Omega}_{\I_i},\I_i) + 2\gamma \\
        \leq & \sum_{i = 1}^3 \F({\Omega}_{\I_i}^*,\I_i) +  2\gamma + \frac{C_X^6 p}{c_X^4} \frac{|\J_1|(s_u - \eta_k)}{|\J_1|+s_u - \eta_k} \kappa_k^2 + \frac{C_X^6 p}{c_X^4} \frac{|\J_4|(\eta_{k + 1} - s_v)}{|\J_4|+\eta_{k + 1} - s_v} \kappa_k^2 + C\frac{\|X\|_{\psi_2}^4 C_X^2}{c_X^4}p^2\log(np) \\
        \leq & \sum_{i = 1}^3 \F({\Omega}_{\I_i}^*,\I_i) +  2\gamma + \frac{C_X^6}{c_X^4} \tr \kappa_k^2 + C\frac{\|X\|_{\psi_2}^4 C_X^2}{c_X^4}p^2\log(np).
\end{align}
% which implies that
% \begin{align}
%     & \sum_{t\in \I}{\rm Tr}(\widehat{\Omega}_{\I}^\top (X_tX_t^\top)) - |\I|\log|\widehat{\Omega}_{\I}| \nonumber  \\
%     \leq & \sum_{i=1}^3 \sum_{t\in \I_i}{\rm Tr}(({\Omega}_{\I_i}^*)^\top (X_tX_t^\top)) - \sum_{i=1}^3|\I_i|\log|{\Omega}_{\I_i}^*| + 2\gamma.
% \end{align}
Let
$$
\widetilde{\gamma} = 2\frac{C_X^6}{c_X^4}\mclB_n^{-1}\Delta\kappa_k^2 +  C\frac{\|X\|_{\psi_2}^4 C_X^2}{c_X^4}p^2\log(np) +  2\gamma.
$$,
Then by Taylor expansion and \Cref{lem:estimation covariance} we have
\begin{align}
    cc_X^2\sum_{t\in \mclI}\|\widehat{\Omega}_{\I} - \Omega^*_t\|_F^2 &\leq \widetilde{\gamma} + \sum_{i=1}^3|\I_i|{\rm Tr}[(\Omega_{\I_i}^* - \widehat{\Omega}_{\I})^\top (\widehat{\Sigma}_{\I_i}  - \Sigma^*_{\I_i})] \nonumber \\
    &\leq \widetilde{\gamma} + C\|X\|_{\psi_2}^2 p\log^{\frac{1}{2}}(np)\left[ \sum_{i=1}^3 \sqrt{|\mclI_{i}|}\|\widehat{\Omega}_{\I} - \Omega^*_{i}\|_F \right]  \nonumber \\
    &\leq \widetilde{\gamma} + C\|X\|_{\psi_2}^2 p\log^{\frac{1}{2}}(np) \sqrt{\sum_{t\in \mclI}\|\widehat{\Omega}_{\I} - \Omega^*_t\|_F^2}.
\end{align}
The inequality above implies that
\begin{equation}
    \sum_{t\in \mclI}\|\widehat{\Omega}_{\I} - \Omega^*_t\|_F^2 \leq \frac{C_1}{c_X^2}\left[\widetilde{\gamma} + \frac{1}{c_X^2}\|X\|^4_{\psi_2} p^{2}\log(np)\right].
\end{equation}
By the choice of $\gamma$, it holds that
\begin{equation}
    \sum_{t\in \I_1\cup\I_2}\|\widehat{\Omega}_{\I} - \Omega^*_t\|_F^2 \leq \frac{C_1C_{\gamma}}{c_X^4} \|X\|^4_{\psi_2} p^{2}\log(np).
\end{equation}
On the other hand,
\begin{equation}
    \sum_{t\in \I_1\cup\I_2}\|\widehat{\Omega}_{\I} - \Omega^*_t\|_F^2\geq \frac{|\mclI_{1}||\mclI_{2}|}{|\mclI|}\|\Omega^*_{k-1} - \Omega^*_k\|_F^2\geq \frac{1}{2}\min\{|\I_1|,|\I_2|\}\|\Omega^*_{k-1} - \Omega^*_k\|_F^2.
\end{equation}
Suppose $|\I_1|\geq |\I_2|$, then the inequality above leads to
\begin{equation*}
    \Delta \kappa^2\leq \frac{C_1C_{\gamma}}{c_X^4} \|X\|^4_{\psi_2} p^{2}\log(np),
\end{equation*}
which is contradictory to the assumption on $\Delta$. Therefore, $|\I_1|<|\I_2|$ and we have 
\begin{equation}
    s-\eta_k = |\I_1|\leq CC_{\gamma} \frac{\|X\|_{\psi_2}^4}{c_X^4\|\Omega_k^* - \Omega_{k-1}^*\|_F^2}p^2\log(np).
\end{equation}
The bound for $e - \eta_{k+1}$ can be proved similarly.
\eprf














\bnlem[Three or more change points]
Suppose the assumptions in \Cref{assp:DCDP_covariance} hold. Then with probability at least $1-(np)^{-3}$, there is no interval $\widehat { \mathcal P}$ containing three or more true change points.   
 \enlem 
\bprf
We prove by contradiction. Suppose    $ \I=(s,e] \in \mathcal {\widehat P}  $  be such that $ \{ \eta_1, \ldots, \eta_M\} \subset \I $ with $M\ge 3$. Throughout the proof, $M$ is assumed to be a parameter that can potentially change with $n$. 
Since the events $\mathcal L ( \tr  ) $ and  $\mathcal R ( \tr ) $ hold, by relabeling $\{ s_q\}_{q=1}^\Q  $ if necessary,   let $ \{ s_m\}_{m=1}^M $ be such that 
 $$ 0 \le s_m  -\eta_m  \le \tr    \quad \text{for} \quad 1 \le m \le M-1  $$ and that
 $$ 0\le \eta_M  - s_M \le \tr .$$ 
 Note that these choices ensure that  $ \{ s_m\}_{m=1}^M  \subset \I . $
 
 \begin{center}
 \begin{tikzpicture} 
\draw[ - ] (-10,0)--(1,0);
 \node[color=black] at (-8,-0.3) {\small s};
 \draw[  (-, ultra thick, black] (-8,0) -- (-7.99,0);
  \draw[ { -]}, ultra thick, black] (-1.0002,0) -- (-1,0);

   \node[color=black] at (-7,-0.3) {\small $\eta_1$};
\draw(-7 ,0)circle [radius=2pt] ;

  \node[color=black] at (-6.5,-0.3) {\small $s_1$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-6.5,0)  }; 

  \node[color=black] at (-5,-0.3) {\small $\eta_2$};
\draw(-5 ,0)circle [radius=2pt] ;
  \node[color=black] at (-4.5,-0.3) {\small $s_2$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-4.5,0)  }; 
 

  \node[color=black] at (-2.5,-0.3) {\small $\eta_3$};
\draw(-2.5 ,0)circle [radius=2pt] ;
  \node[color=black] at (-3 ,-0.3) {\small $s_3$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-3,0)  }; 
  
   \node[color=black] at (-1,-0.3) {\small $e$};

 
\end{tikzpicture}
\end{center}

{\bf Step 1.}
 Denote 
 $$ \mathcal I_ 1= (  s, s _1], \quad \I_m   =(s_{m-1} , s_m] \text{ for }  2 \le m \le M     \quad \text{and} \quad \I_{M+1}   = (s_M,e]. $$
Then since 
$ s , e,  \{ s_m \}_{m=1}^M  \subset   \{ s_q\}_{q=1}^\Q  $,   it follows that 



Suppose $\I = (s,e]\in \widehat{\mclP}$ and there are $M\geq 3$ true change points $\{\eta_{q + i}\}_{i\in [M]}$ inside $\I$, and denote
\begin{equation*}
    \I_1 = (s, \eta_{q + 1}],\ \I_m = (\eta_{q + m - 1},\eta_{q + m}],\ \I_{M+1} = (\eta_{q + M},e].
\end{equation*}
Then by the definition of $\widehat{\mclP}$ and $\widehat{\Omega}_{\I_m}$, it holds that
\begin{equation*}
    \F(\hat{\Omega}_{\I},\I)\leq \sum_{i = 1}^{M+1} \F(\hat{\Omega}_{\I_i},\I_i) + M\gamma\leq \sum_{i = 1}^{M+1} \F({\Omega}_{\I_i}^*,\I_i) + M\gamma,
\end{equation*}
which implies that
\begin{align}
    & \sum_{t\in \I}{\rm Tr}(\widehat{\Omega}_{\I}^\top (X_tX_t^\top)) - |\I|\log|\widehat{\Omega}_{\I}| \nonumber  \\
    \leq & \sum_{i=1}^{M+1} \sum_{t\in \I_i}{\rm Tr}(({\Omega}_{\I_i}^*)^\top (X_tX_t^\top)) - \sum_{i=1}^{M+1}|\I_i|\log|{\Omega}_{\I_i}^*| + M\gamma.
\end{align}
By Taylor expansion and \Cref{lem:estimation covariance} we have
\begin{align}
    cc_X^2\sum_{t\in \mclI}\|\widehat{\Omega}_{\I} - \Omega^*_t\|_F^2 &\leq M\gamma + \sum_{i=1}^{M+1}|\I_i|{\rm Tr}[(\Omega_{\I_i}^* - \widehat{\Omega}_{\I})^\top (\widehat{\Sigma}_{\I_i}  - \Sigma^*_{\I_i})] \nonumber \\
    &\leq M\gamma + C\|X\|_{\psi_2}^2 p\log^{\frac{1}{2}}(np)\left[ \sum_{i=1}^{M+1} \sqrt{|\mclI_{i}|}\|\widehat{\Omega}_{\I} - \Omega^*_{i}\|_F \right]  \nonumber \\
    &\leq M\gamma + C\|X\|_{\psi_2}^2 p\log^{\frac{1}{2}}(np) \sqrt{\sum_{t\in \mclI}\|\widehat{\Omega}_{\I} - \Omega^*_t\|_F^2}.
\end{align}
The inequality above implies that
\begin{equation}
    \sum_{t\in \mclI}\|\widehat{\Omega}_{\I} - \Omega^*_t\|_F^2 \leq \frac{C_1}{c_X^2}\left[M\gamma + \frac{1}{c_X^2}\|X\|^4_{\psi_2} p^{2}\log(np)\right].
\end{equation}
On the other hand, for each $i\in [M]$, we have
\begin{equation}
    \sum_{t\in \I_i\cup\I_{i +1}}\|\widehat{\Omega}_{\I} - \Omega^*_t\|_F^2\geq \frac{|\mclI_{i}||\mclI_{i + 1}|}{|\mclI|}\|\Omega^*_{\eta_{q + i + 1}} - \Omega^*_{\eta_{q + i}}\|_F^2.
\end{equation}
In addition, for each $i\in \{2,\cdots,M\}$, by definition, it holds that $\min\{|\I_i|,|\I_{i + 1}|\}\geq \Delta$. Therefore, we have
\begin{align*}
    (M-2)\Delta \kappa^2\leq \frac{C_1}{c_X^2}\left[M\gamma + \frac{1}{c_X^2}\|X\|^4_{\psi_2} p^{2}\log(np)\right].
\end{align*}
Since $M/(M-2)\leq 3$ for any $M\geq 3$, it holds that
\begin{equation}
    \Delta \leq CC_{\gamma} \frac{\|X\|_{\psi_2}^4}{c_X^4\|\Omega_k^* - \Omega_{k-1}^*\|_F^2}p^2\log(np),
\end{equation}
which is contradictory to the assumption on $\Delta$, and the proof is complete.
\eprf






 \bnlem[Two consecutive intervals]
 \label{lem:cov two consecutive interval}
 Under \Cref{assp:DCDP_covariance} and the choice that $$\gamma\geq C_{\gamma}\|X\|_{\psi_2}^4\max_{k\in [K+1]}\|\Omega_{\eta_k}^*\|_2^2 p^2\log(np),$$ with probability at least $1-(np)^{-3}$, there are no  two consecutive intervals $\I_1= (s,t ] \in \widehat{\mathcal P}$, $\I_2=(t, e] \in   \widehat{\mathcal P}$ such that $\I_1 \cup \I_2$ contains no change points.  
 \enlem 
 \begin{proof} 
 We prove by contradiction. Suppose that $\I_1,\I_2\in \widehat{\mclP}$ and
 $$ \I :  =\I_1\cup  \I_2 $$
 contains no change points. 
 By the definition of $\widehat{\mclP}$ and $\widehat{\Omega}_{\I}$, it holds that
 $$ \F(\widehat{\Omega}_{\I_1},\I_1)  + \F(\widehat{\Omega}_{\I_2},\I_2) + \gamma \leq  \F(\widehat{\Omega}_{\I},\I)\leq \F({\Omega}_{\I}^*,\I)$$
 By \Cref{lem:cov no cp}, it follows that 
\begin{align*} 
\F({\Omega}^*_{\I_1}, \mclI_1)\leq &  \F(\widehat{\Omega}_{\I_1}, \mclI_1) + C\frac{\|X\|_{\psi_2}^4}{c_X^2} p^2\log(np),
 \\
\F({\Omega}^*_{\I_2}, \mclI_2)\leq &  \F(\widehat{\Omega}_{\I_2}, \mclI_2) +  C\frac{\|X\|_{\psi_2}^4}{c_X^2} p^2\log(np) 
 \end{align*}
 So
 $$\F({\Omega}^*_{\I_1}, \mclI_1) +\F({\Omega}^*_{\I_2}, \mclI_2) -2C\frac{\|X\|_{\psi_2}^4}{c_X^2} p^2\log(np)  +\gamma    \leq  \F({\Omega}_{\I}^*,\I).  $$
 Since $\I$ does not contain any change points, ${\Omega}^*_{\I_1} = {\Omega}^*_{\I_2} = {\Omega}^*_{\I}$, and it follows that 
 $$ \gamma \leq 2C\frac{\|X\|_{\psi_2}^4}{c_X^2} p^2\log(np).$$
 This is a contradiction when $C_\gamma> 2C$.
 \end{proof} 






























%%%% location indicator %%%%
%%%% start of regression part %%%%









\clearpage
\subsection{High-dimensional regression}


Throughout this section, unless specified otherwise, for the output of \Cref{algorithm:DCDP_divide}, we always set the loss function $\mclF(\cdot, \cdot)$ to be
\begin{equation}
\mathcal F  (\beta, \I) :  = \begin{cases} 
 \sum_{i \in \I } (y_i - X_i^\top \beta) ^2  &\text{if } |\I|\ge C_\mclF\s \log(np) ,
 \\ 
 0 &\text{otherwise,}
 \end{cases}
\end{equation} 
where $C_{\mclF}$ is a universal constant which is larger than $C_s$, the constant in sample size in \Cref{lemma:interval lasso} and \Cref{lemma:consistency}.


% From now on without loss of generality we assume $\sigma_{\epsilon} = 1$.

 \bnprop\label{prop:regression local consistency}
 Suppose  \Cref{assp:dcdp_linear_reg} holds. Let 
 $\widehat { \mathcal P }  $ denote the output of  \Cref{algorithm:DCDP_divide} with

Suppose that $\gamma \ge C_\gamma  K\tr\kappa^2$. Uniformly with probability  at least $1 - C n ^{-3}$, the following conditions hold.
	\begin{itemize}
		\item [(i)] For each interval  $ \I = (s, e] \in \widehat{\mathcal{P}}$    containing one and only one true 
		   change point $ \eta_k $, it must be the case that
 $$\min\{ \eta_k -s ,e-\eta_k \}  \lesssim \frac{\sigma_{\epsilon}^2\vee 1  }{\kappa^2 }\bigg(  \s \log(np) +\gamma \bigg) +  \tr.$$
	\item [(ii)] For each interval  $  \I = (s, e] \in \widehat{\mathcal{P}}$ containing exactly two true change points, say  $\eta_ k  < \eta_ {k+1} $, it must be the case that
\begin{align*} 
 \eta_k -s    \lesssim   \frac{\sigma_{\epsilon}^2\vee 1  }{\kappa^2 }\bigg(  \s \log(np) +\gamma \bigg) +  \tr      \ \text{and} \ 
 e-\eta_{k+1}   \le  C   \frac{\sigma_{\epsilon}^2\vee 1  }{\kappa^2 }\bigg(  \s \log(np) +\gamma \bigg) +  \tr. 
 \end{align*} 
		 
\item [(iii)] No interval $\I \in \widehat{\mathcal{P}}$ contains strictly more than two true change points; and 


	\item [(iv)] For all consecutive intervals $ \I_1 $ and $ \I_2 $ in $\widehat{ \mathcal P}$, the interval 
		$ \I_1 \cup  \I_2 $ contains at least one true change point.
				
	 \end{itemize}
\enprop 

 

\bnprop\label{prop:regression change points partition size consistency}
Suppose  \Cref{assp:dcdp_linear_reg} holds. Let 
 $\widehat { \mathcal P }  $ denote the output of  \Cref{algorithm:DCDP_divide}. Suppose 
$\gamma \ge  C_\gamma K \tr  \kappa^2$  for sufficiently large constant $C_\gamma$. Then
 with probability  at least $1 - C n ^{-3}$,  $| \widehat { \mathcal P} | =K $.
\enprop



\begin{proof}[Proof of   \Cref{prop:regression change points partition size consistency}] 
Denote $\mathfrak{G} ^*_n = \sum_{ i =1}^n (y_i  -  X_i^\top \beta^*_i)^2$.  Given any collection $\{t_1, \ldots, t_m\}$, where $t_1 < \cdots < t_m$, and $t_0 = 0$, $t_{m+1} = n$, let 
	\begin{equation}\label{regression eq-sn-def}
		\G _n(t_1, \ldots, t_{m}) = \sum_{k=1}^{m} \sum_{ i = t_k +1}^{t_{k+1}} \mclF(\widehat{\beta} _  {(t_{k}, t_{k+1}]}, (t_{k}, t_{k+1}]). 
	\end{equation}
For any collection of time points, when defining \eqref{regression eq-sn-def}, the time points are sorted in an increasing order.

Let $\{ \widehat \eta_{k}\}_{k=1}^{\widehat K}$ denote the change points induced by $\widehat {\mathcal P}$.  Suppose we can justify that 
	\begin{align}
		\G^*_n + K\gamma  \ge  &\G _n(s_1,\ldots,s_K)   + K\gamma - C_1 ( K +1)  \s \log(np) - C_1\sum_{k\in [K]}\kappa_k^2\tr  \label{eq:regression K consistency step 1} \\ 
		\ge & \G_n (\widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } ) +\widehat K \gamma - C_1 ( K +1)  \s \log(np) - C_1\sum_{k\in [K]}\kappa_k^2\tr  \label{eq:regression K consistency step 2} \\ 
		\ge &  \G _n ( \widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K ) + \widehat K \gamma    - C_1 ( K +1)  \s \log(np)- C_1\sum_{k\in [K]}\kappa_k^2\tr  \label{eq:regression K consistency step 3}
	\end{align}
	and that 
	\begin{align}\label{eq:regression K consistency step 4}
		\G ^*_n   -\G _n ( \widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K ) \le C_2 (K + \widehat{K} + 2) \s \log(np) .
	\end{align}
	Then it must hold that $| \hatp | = K$, as otherwise if $\widehat K \ge K+1 $, then  
	\begin{align*}
		C _2 (K + \widehat{K} + 2)  \s \log(np)  & \ge   \G ^*_n  -\G _n ( \widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K ) \\
		& \ge      (\widehat K - K)\gamma  -C_1 ( K +1)  \s \log(np) - C_1\sum_{k\in [K]}\kappa_k^2\tr.
	\end{align*} 
	Therefore due to the assumption that $| \hatp|  =\widehat K\le 3K $, it holds that 
	\begin{align} \label{eq:regression Khat=K} 
		C_2 (4K + 2) \s \log(np)  + C_1(K+1) \s \log(np) +C_1\sum_{k\in [K]}\kappa_k^2\tr \ge  (\widehat K - K)\gamma \geq \gamma,
	\end{align}
	Note that \eqref{eq:regression Khat=K} contradicts the choice of $\gamma$.


\
\\
{\bf Step 1.} Note that \eqref{eq:regression K consistency step 1}  is implied by 
	\begin{align}\label{eq:regression step 1 K consistency}  
		\left| 	\G ^*_n   -   \G_n(s_1,\ldots,s_K)    \right| \le  C_3(K+1) \lambda^2 + C_3\sum_{k\in [K]}\kappa_k^2\tr ,
	\end{align}
	which is  an  immediate consequence  of \Cref{lam:regression one change deviation bound}. 
	\
	\\
	\\
	{\bf Step 2.} Since $\{ \widehat \eta_{k}\}_{k=1}^{\widehat K}$ are the change points induced by $\widehat {\mathcal P}$, \eqref{eq:regression K consistency step 2} holds because $\hatp$ is a minimizer.
\\
\\
	{\bf Step 3.}
For every $ \I  =(s,e]\in \hatp$, by \Cref{prop:regression local consistency}, we know that with probability at least $1 - (np)^{-5}$, $\I$ contains at most two change points. We only show the proof for the two-change-point case as the other case is easier. Denote
	\[
		 \I =  (s ,\eta_{q}]\cup (\eta_{q},\eta_{q+1}] \cup  (\eta_{q+1} ,e]  = \J_1 \cup \J_2 \cup \J_{3},
	\]
where $\{ \eta_{q},\eta_{q+1}\} =\I \, \cap \, \{\eta_k\}_{k=1}^K$. 

For each $m\in\{1,2,3\}$, by \Cref{lam:regression one change deviation bound}, it holds that
\[
\sum_{ i \in \J_m }(y_ i - X_i^\top \widehat{\beta} _{\J_m}    )^2   \leq \sum_{ i \in \J_ m } (y_ i  - X_i^\top \beta^*_i   )^2 + C\sigma_{\epsilon}^2\s \log(np).
\]
By \Cref{lam:regression goodness of fit J superset of I}, we have
\[
\sum_{ i \in \J_m }(y_ i - X_i^\top\widehat {\beta} _\I    )^2   \ge \sum_{ i \in \J_ m } (y_ i  - X_i^\top \beta_i^*   )^2 - C\sigma_{\epsilon}^2\s \log(np).
\]
 Therefore the above inequality implies that 
	\begin{align} \label{eq:regression K consistency step 3 inequality 3}  \sum_{i \in \I }  (y_ i - X_i^*\widehat {\beta} _\I    )^2   \ge \sum_{m=1}^{3} \sum_{ i \in \J_m }(y_ i - X_i^\top\widehat {\beta} _{\J_m}    )^2  -C\sigma_{\epsilon}^2\s\log(np).  
	\end{align}
Note that   \eqref{eq:regression K consistency step 3} is an immediate consequence of   \eqref{eq:regression K consistency step 3 inequality 3}.

	{\bf Step 4.}
Finally, to show \eqref{eq:regression K consistency step 4},   let  $\widetilde { \mathcal P}$ denote    the partition induced by $\{\widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K\}$. Then 
$| \widetilde { \mathcal P} | \le K + \widehat K+2   $ and that $\beta^*_i$ is unchanged in every interval $\I \in \widetilde { \mathcal P}$. 
	So  \Cref{eq:regression K consistency step 4} is an immediate consequence of   \Cref{lam:regression one change deviation bound}.
\end{proof} 






\begin{proof}[Proof of \Cref{cor:regression local refinement}]
For each $k\in [K]$, let $\hat{\beta}_t = \hat{\beta}^{(1)}$ if $s_k<t< \hat{\eta}_k$ and $\hat{\beta}_t =\hat{\beta}^{(2)}$ otherwise. Let ${\beta}^*_t$ be the true parameter at time point $t$, and $\beta^{(1)} = \beta^*_{\eta_k}$ and $\beta^{(2)} = \beta^*_{\eta_k + 1}$. First we show that under conditions $\tilde{K} = K$ and $\max_{k\in [K]}|\tilde{\eta}_k - \eta_k|\leq \Delta / 5$, there is only one true change point $\eta_k$ in $(s_k, e_k)$. It suffices to show that
\begin{equation}
    |\tilde{\eta}_k - \eta_k|\leq \frac{2}{3}(\tilde{\eta}_{k+1} - \tilde{\eta}_{k}),\ \text{and}\ |\tilde{\eta}_{k+1} - \eta_{k+1}|\leq \frac{1}{3}(\tilde{\eta}_{k+1} - \tilde{\eta}_{k}).
    \label{tmp_eq:goal_lr}
\end{equation}
Denote $R = \max_{k\in [K]}|\tilde{\eta}_k - \eta_k|$, then
\begin{align*}
    \tilde{\eta}_{k+1} - \tilde{\eta}_{k} &= \tilde{\eta}_{k+1} - {\eta}_{k+1} + {\eta}_{k+1} - {\eta}_{k} + {\eta}_{k} - \tilde{\eta}_{k} \\
    &= ({\eta}_{k+1} - {\eta}_{k}) + (\tilde{\eta}_{k+1} - {\eta}_{k+1}) + ({\eta}_{k} - \tilde{\eta}_{k})\in [{\eta}_{k+1} - {\eta}_{k} - 2R,{\eta}_{k+1} - {\eta}_{k} + 2R].
\end{align*}
Therefore, \Cref{tmp_eq:goal_lr} is guaranteed as long as
\begin{equation*}
    R\leq \frac{1}{3}(\Delta - 2R),
\end{equation*}
which is equivalent to $R\leq \Delta/5$.

Now without loss of generality, assume that $s_k<\eta_k<\hat{\eta}_k<e_k$. Denote $\mclI_k = \{s_k + 1, \cdots, e_k\}$. Consider two cases:

\textbf{Case 1.} If
\begin{equation*}
    \hat{\eta}_k - \eta_k < \max\{C_s(\sigma_{\epsilon}^2\vee 1)\s\log(np), C_s(\sigma_{\epsilon}^2\vee 1)\s\log(np)/\kappa^2\},
\end{equation*}
then the proof is done.

\textbf{Case 2.} If
\begin{equation*}
    \hat{\eta}_k - \eta_k \geq \max\{C_s(\sigma_{\epsilon}^2\vee 1)\s\log(np), C_s(\sigma_{\epsilon}^2\vee 1)\s\log(np)/\kappa^2\},
\end{equation*}
then we proceed to prove that $|\hat{\eta}_k - \eta_k|\leq C(\sigma_{\epsilon}^2\vee 1)\s\log(np)/\kappa^2$ with probability at least $1 - (np)^{-5}$. Then we either prove the result or get an contradiction, and complete the proof in either case. The first step is to prove that with probability at least $1 - (np)^{-5}$,
	\[
		\sum_{t = s_k + 1}^{e_k}\|\widehat{\beta}_t - \beta^*_t\|_2^2 \leq C_1\s \zeta^2.
	\]
Due to \Cref{eq-g-lasso}, it holds that
	\begin{align}\label{eq:reg local refine 1}
		& \sum_{t = s_k + 1}^{e_k} \|y_t - X_t^{\top}\widehat{\beta}_t\|_2^2 + \zeta \sum_{i = 1}^p \sqrt{\sum_{t = s_k + 1}^{e_k} \bigl(\widehat{\beta}_t\bigr)_i^2} \leq \sum_{t = s_k + 1}^{e_k} \|y_{t} - X_t^{\top}\beta^*_t \|_2^2 + \zeta \sum_{i = 1}^p \sqrt{\sum_{t = s_k + 1}^{e_k} \bigl(\beta^*_t\bigr)_{i}^2}.
	\end{align}
	Let $\delta_t = \widehat{\beta}_t - \beta^*_t$. It holds that $\sum_{t = s_k + 1}^{e_k - 1}\mathbbm{1}\left\{\delta_t \neq \delta_{t+1}\right\} = 2$.	Then \Cref{eq:reg local refine 1} implies that
	\begin{align}\label{eq:reg local refine 2}
		\sum_{t = s_k + 1}^{e_k} \|\delta_t^{\top} X_t\|_2^2 + \zeta  \sum_{i = 1}^p \sqrt{\sum_{t = s_k + 1}^{e_k} \bigl(\widehat{\beta}_t\bigr)_{i}^2}\leq 2\sum_{t = s_k + 1}^{e_k} (y_t - X_t^{\top}\beta^*_t)\delta_t^{\top} X_t + \zeta \sum_{i = 1}^p \sqrt{\sum_{t = s_k + 1}^{e_k} \bigl(\beta^*_t\bigr)_{i}^2}.
	\end{align}
Note that
	\begin{align}
		& \sum_{i = 1}^p \sqrt{\sum_{t = s_k + 1}^{e_k} \bigl(\beta^*_t\bigr)_{i}^2} - \sum_{i = 1}^p \sqrt{\sum_{t = s_k + 1}^{e_k} \bigl(\widehat{\beta}_t\bigr)_{i}^2} \nonumber \\
		=& \sum_{i \in S} \sqrt{\sum_{t = s_k + 1}^{e_k} \bigl(\beta^*_t\bigr)_{i}^2} - \sum_{i \in S} \sqrt{\sum_{t = s_k + 1}^{e_k} \bigl(\widehat{\beta}_t\bigr)_{i}^2}  - \sum_{i \in S^c} \sqrt{\sum_{t = s_k + 1}^{e_k} \bigl(\widehat{\beta}_t\bigr)_{i}^2} \nonumber \\
		\leq & \sum_{i \in S} \sqrt{\sum_{t = s_k + 1}^{e_k} \bigl(\delta_t\bigr)_{i}^2}  - \sum_{i \in S^c} \sqrt{\sum_{t = s_k + 1}^{e_k} \bigl(\delta_t\bigr)_{i}^2}.\label{eq:reg local refine 3}
	\end{align}
We then examine the cross term, with probability at least $1 - (np)^{-5}$, which satisfies the following
	\begin{align}
		& \left|\sum_{t = s_k + 1}^{e_k} (y_t - X_t^{\top}\beta^*_t)\delta_t^{\top} X_t\right| = \left|\sum_{t = s_k + 1}^{e_k} \epsilon_{t} \delta_t^{\top} X_t\right| = \sum_{i = 1}^p \left\{\left|\frac{\sum_{t = s_k + 1}^{e_k} \epsilon_{t} (\delta_t)_i (X_t)_i}{\sqrt{\sum_{t = s_k + 1}^{e_k} (\delta_t)^2_i}}\right| \sqrt{\sum_{t = s_k + 1}^{e_k} (\delta_t)^2_i}\right\} \nonumber \\
		\leq & \sup_{i = 1, \ldots, p} \left|\frac{\sum_{t = s_k + 1}^{e_k} \epsilon_{t} (\delta_t)_i (X_t)_i}{\sqrt{\sum_{t = s_k + 1}^{e_k} (\delta_t)^2_i}}\right| \sum_{i = 1}^p \sqrt{\sum_{t = s_k + 1}^{e_k} (\delta_t)^2_i} \leq (\zeta/4) \sum_{i = 1}^p \sqrt{\sum_{t = s_k + 1}^{e_k} (\delta_t)^2_i}, \label{eq:reg local refine 4}
	\end{align}
	where the second inequality follows from \Cref{lem:deviation piecewise constant}.

Combining \eqref{eq:reg local refine 1}, \eqref{eq:reg local refine 2}, \eqref{eq:reg local refine 3} and \eqref{eq:reg local refine 4} yields
	\begin{equation}\label{eq:reg local refine 5}
		\sum_{t = s_k + 1}^{e_k} \|\delta_t^{\top} X_t\|_2^2	 + \frac{\zeta}{2}\sum_{i \in S^c} \sqrt{\sum_{t = s_k + 1}^{e_k} \bigl(\delta_t\bigr)_{i}^2} \leq \frac{3\zeta}{2}\sum_{i \in S} \sqrt{\sum_{t = s_k + 1}^{e_k} \bigl(\delta_t\bigr)_{i}^2}.
	\end{equation}
Now we are to explore the restricted eigenvalue inequality. Let
	\[
		\I_1 = (s_k, \eta_k], \quad \I_2 = (\eta_k, \widehat{\eta}_k], \quad \I_3 = (\widehat{\eta}_k, e_k].
	\]
Then for $\I_1$, it holds that
	\begin{align}
		& \eta_k - s_k = \eta_k - \frac{2}{3}\widetilde{\eta}_k - \frac{1}{3}\widetilde{\eta}_k \nonumber \\
		= & \frac{2}{3}(\eta_k - \eta_{k-1}) + \frac{2}{3}(\widetilde{\eta}_k - \eta_k) -  \frac{2}{3}(\widetilde{\eta}_{k-1} - \eta_{k-1}) + (\eta_k - \widetilde{\eta}_k) \nonumber \\
		\geq & \frac{2}{3}\Delta - \frac{1}{3}\Delta = \frac{1}{3}\Delta, \label{tmp_eq:regression I_1}
	\end{align}	
where the inequality follows from \Cref{assp:dcdp_linear_reg} and \Cref{eq-lr-cond-1}. 

For $\I_3$, by the design of the local refinement algorithm in \Cref{algo:local_refine_general}, we have $|\I_3|\geq C_s \s\log(np)$. Since $\min\{|\I_1|,|\I_3|\}\geq C_s\s\log(np)$, by \Cref{lem:restricted eigenvalue}, it holds with probability at least $1 - (np)^{-5}$ that,
	\begin{align*}
		& \sum_{i = 1, 3}\sum_{t \in \I_i}\|\delta_{\I_i}^{\top}X_t\|_2^2 \\
		\geq & \sum_{i = 1, 3} \left(c'_1\sqrt{|\I_i|} \|\delta_{\I_i}\|_2 - c_2 \sqrt{\log(p)} \|\delta_{\I_i}\|_1\right)^2 \\
		\geq & \sum_{i = 1, 3} \left(c_1\sqrt{|\I_i|} \|\delta_{\I_i}\|_2 - c_2 \sqrt{\log(p)} \|(\delta_{\I_i})_{S^c}\|_1\right)^2,
	\end{align*}
	where the last inequality follows from $\|(\delta_{\I})_S\|_1\leq \sqrt{\s}\|\delta_{\I}\|_2$ and the fact that $\min\{|\I_1|,|\I_3|\}>C_s \s \log(np)$. Similarly, since $|\I_2| > \Delta> C_s \s \log(np)$, we have
	\[
		\sqrt{\sum_{t \in \I_2}\|\delta_{\I_2}^{\top}X_t\|_2^2} \geq {c_1\sqrt{|\I_2|}} \|\delta_{\I_2}\|_2 - c_2 \sqrt{\log(p)} \|\delta_{\I_2}(S^c)\|_1.
	\]
Denote $n_0 = C_s\s\log(np)$. We first bound the terms with $\|\cdot\|_1$. Note that
	\begin{align*}
	&\sum_{i = 1}^3\sum_{j\in S^c}|(\delta_{\I_i})_j|
		\leq \sqrt{3}\sqrt{\sum_{i = 1}^3 (\sum_{j \in S^c} |(\delta_{\I_i})_j|)^2 } \\ 
		\leq & \sqrt{3}\sqrt{\sum_{i = 1}^3{\frac{|\I_i|}{n_0}} (\sum_{j \in S^c}|(\delta_{\I_i})_j| )^2}	
		\leq  \sqrt{\frac{3}{n_0}} \sum_{i = 1}^3   \sqrt{|\I_i|}(\sum_{j \in S^c}|(\delta_{\I_i})_j| ) \\
		\leq &
		\sqrt{\frac{3}{n_0}} \sum_{j \in S^c}  \sqrt{\sum_{t = s_k + 1}^{e_k} (\delta_t)_j^2}
		\leq \frac{3\sqrt{3}}{\sqrt{n_0}}\sum_{j \in S}  \sqrt{\sum_{t = s_k + 1}^{e_k} (\delta_t)_j^2}
		\\
		\leq & \frac{3\sqrt{3}}{\sqrt{n_0}} \sqrt{\s \sum_{j \in S} \sum_{t = s_k + 1}^{e_k} (\delta_t)_j^2} \leq \frac{c}{ \sqrt{\log(np)}} \sqrt{\sum_{t = s_k + 1}^{e_k} \|\delta_t\|_2^2}.
	\end{align*}
Therefore,
	\begin{align*}
		& c_1\sqrt{\sum_{t = s_k + 1}^{e_k} \|\delta_t\|_2^2} - \frac{c_2}{ \sqrt{\log(np)}} \sqrt{\sum_{t = s_k + 1}^{e_k} \|\delta_t\|_2^2} \\
		\leq & \sum_{i = 1}^3 c_1 \|\delta_{I_i}\|_2 - \frac{c_2}{ \sqrt{\log(np)}} \sqrt{\sum_{t = s_k + 1}^{e_k} \|\delta_t\|_2^2} \leq \sqrt{3} \sqrt{ \sum_{t = s_k + 1}^{e_k} \|\delta_t^{\top} X_t\|_2^2 } \\
		\leq & \frac{3\sqrt{\zeta}}{\sqrt{2}}\s^{1/4} \left(\sum_{t = s_k + 1}^{e_k} \|\delta_t\|_2^2\right)^{1/4} \leq \frac{9\zeta \s^{1/2}}{4c_1} + \frac{c_1}{2}\sqrt{\sum_{t = s_k + 1}^{e_k} \|\delta_t\|_2^2}
	\end{align*}
	where the third inequality follows from \eqref{eq:reg local refine 5} and the fact that $\sum_{i\in S}\sqrt{\sum_{t=s_k + 1}^{e_k}(\delta_t)_i^2}\leq \sqrt{s}\sqrt{\sum_{t=s_k + 1}^{e_k}\|\delta_t\|_2^2}$. The inequality above implies that
	\[
		\frac{c_1}{4}\sqrt{\sum_{t = s_k + 1}^{e_k} \|\delta_t\|_2^2} \leq \frac{9\zeta \s^{1/2}}{4c_1}
	\]	
	Therefore,
	\[
		\sum_{t = s_k + 1}^{e_k}\|\widehat{\beta}_t - \beta^*_t\|_2^2 \leq 81\zeta^2\s/c_1^4.
	\]
  Recall that $\beta^{(1)} = \beta^*_{\eta_k}$ and $\beta^{(2)} = \beta^*_{\eta_k + 1}$. We have that
	\[
		\sum_{t = s_k + 1}^{e_k}\|\widehat{\beta}_t - \beta^*_t\|_2^2 = |I_1| \|\beta^{(1)} - \widehat{\beta}^{(1)}\|_2^2 + |I_2| \|\beta^{(2)} - \widehat{\beta}^{(1)}\|_2^2 + |I_3| \|\beta^{(2)} - \widehat{\beta}^{(2)}\|_2^2.
	\]
Since $\eta_k - s_k \geq\frac{1}{3}\Delta$ as is shown in \Cref{tmp_eq:regression I_1}. we have that
	\[
		\Delta\|\beta^{(1)} - \widehat{\beta}^{(1)}\|_2^2/3 \leq |I_1| \|\beta^{(1)} - \widehat{\beta}^{(1)}\|_2^2 \leq \frac{C_1 C_{\zeta}^2\Delta \kappa^2} {\s K \sigma^2_{\epsilon} \Bn } \leq c_3 \Delta \kappa^2,
	\]
	where $1/4 > c_3 > 0$ is an arbitrarily small positive constant.  Therefore we have
	\[
		\|\beta^{(2)} - \widehat{\beta}_1\|_2^2 \leq 3c_3 \kappa^2.
	\]
In addition we have
	\[
		\|\beta^{(2)} - \widehat{\beta}^{(1)}\|_2 \geq \|\beta^{(2)} - \beta^{(1)}\|_2 - \|\beta^{(1)} - \widehat{\beta}^{(1)}\|_2 \geq \kappa/2.
	\]	
	Therefore, it holds that 	
	\[
		\kappa^2 |I_2|/4 \leq |I_2| \|\beta^{(2)} - \widehat{\beta}^{(1)}\|_2^2 \leq C_2\s\zeta^2,
	\]
	which implies that 
	\[
		|\widehat{\eta}_k - \eta_k| \leq \frac{4C_2\s \zeta^2}{\kappa^2},
	\]
which gives the bound we want. 
\end{proof}














\subsubsection{Technical lemmas}

Throughout this section, let $\widehat { \mathcal P }  $ denote the output of  \Cref{algorithm:DCDP_divide}.
 
 
 

\bnlem
Let $\mathcal{S}$ be any linear subspace in $\mathbb{R}^n$ and $\mathcal{N}_{1/4}$	be a $1/4$-net of $\mathcal{S} \cap B(0, 1)$, where $B(0, 1)$ is the unit ball in $\mathbb{R}^n$.  For any $u \in \mathbb{R}^n$, it holds that
	\[
		\sup_{v \in \mathcal{S} \cap B(0, 1)} \langle v, u \rangle \leq 2 \sup_{v \in \mathcal{N}_{1/4}} \langle v, u \rangle,
	\]
	where $\langle \cdot, \cdot \rangle$ denotes the inner product in $\mathbb{R}^n$.
\enlem

\begin{proof}
Due to the definition of $\mathcal{N}_{1/4}$, it holds that for any $v \in \mathcal{S} \cap B(0, 1)$, there exists a $v_k \in \mathcal{N}_{1/4}$, such that $\|v - v_k\|_2 < 1/4$.  Therefore,
	\begin{align*}
		\langle v, u \rangle = \langle v - v_k + v_k, u \rangle = \langle x_k, u \rangle + \langle v_k, u \rangle \leq \frac{1}{4} \langle v, u \rangle + \frac{1}{4} \langle v^{\perp}, u \rangle + \langle v_k, u \rangle,
	\end{align*}
	where the inequality follows from  $x_k = v - v_k = \langle x_k, v \rangle v + \langle x_k, v^{\perp} \rangle v^{\perp}$.  Then we have
	\[
		\frac{3}{4}\langle v, u \rangle \leq \frac{1}{4} \langle v^{\perp}, u \rangle + \langle v_k, u \rangle.
	\]
	It follows from the same argument that 
	\[
		\frac{3}{4}\langle v^{\perp}, u \rangle \leq \frac{1}{4} \langle v, u \rangle + \langle v_l, u \rangle,
	\]
	where $v_l \in \mathcal{N}_{1/4}$ satisfies $\|v^{\perp} - v_l\|_2 < 1/4$.  Combining the previous two equation displays yields
	\[
		\langle v, u \rangle \leq 2 \sup_{v \in \mathcal{N}_{1/4}} \langle v, u \rangle,
	\]
	and the final claims holds.
\end{proof}

 

\Cref{lem:deviation piecewise constant} is an adaptation of Lemma 3 in \cite{wang2021_jmlr}.

\bnlem\label{lem:deviation piecewise constant}
	Given any interval $I = (s, e] \subset \{1, \ldots, n\}$. Let $\mclR_m := \{v \in \mathbb{R}^{(e-s)}| \|v\|_2 = 1, \sum_{t = 1}^{e-s-1} \mathbf{1}\{v_i \neq v_{i+1}\} = m\}$. Then for data generated from \Cref{assp:dcdp_linear_reg}, it holds that for any $\delta > 0$, $i \in \{1, \ldots, p\}$, 
	\[
		\mathbb{P}\left\{\sup_{v\in \mclR_m} \left|\sum_{t = s+1}^e v_t \epsilon_t (X_t)_i\right| > \delta \right\} \leq C(e-s-1)^m 9^{m+1} \exp \left\{-c \min\left\{\frac{\delta^2}{4C_x^2}, \, \frac{\delta}{2C_x \|v\|_{\infty}}\right\}\right\}.
	\]
\enlem

\begin{proof}
For any $v \in \mathbb{R}^{(e-s)}$ satisfying $\sum_{t = 1}^{e-s-1}\mathbbm{1}\{v_i \neq v_{i+1}\} = m$, it is determined by a vector in $\mathbb{R}^{m+1}$ and a choice of $m$ out of $(e-s-1)$ points.  Therefore we have,
	\begin{align*}
		& \mathbb{P}\left\{\sup_{\substack{v \in \mathbb{R}^{(e-s)}, \, \|v\|_2 = 1\\ \sum_{t = 1}^{e-s-1} \mathbf{1}\{v_i \neq v_{i+1}\} = m}} \left|\sum_{t = s+1}^e v_t \epsilon_t (X_t)_i\right| > \delta \right\} \\
		\leq & {(e-s-1) \choose m} 9^{m+1} \sup_{v \in \mathcal{N}_{1/4}}	\mathbb{P}\left\{\left|\sum_{t = s+1}^e v_t \epsilon_t (X_t)_i\right| > \delta/2 \right\} \\
		\leq & {(e-s-1) \choose m} 9^{m+1} C\exp \left\{-c \min\left\{\frac{\delta^2}{4C_x^2}, \, \frac{\delta}{2C_x \|v\|_{\infty}}\right\}\right\} \\
		\leq & C(e-s-1)^m 9^{m+1} \exp \left\{-c \min\left\{\frac{\delta^2}{4C_x^2}, \, \frac{\delta}{2C_x \|v\|_{\infty}}\right\}\right\}.
	\end{align*}

\end{proof}






 












 \bnlem\label{lam:regression goodness of fit J superset of I}
Let $\I\subset [1,T]$ be any interval that contains no change point. Then under \Cref{assp:dcdp_linear_reg}, for any interval $\J \supset \I$, it holds with probability at least $1 - (np)^{-5}$ that
\begin{equation*}
    \mclF(\mu^*_{\I},\I)\leq \mclF(\widehat{\mu}_\J,\I) + C(\sigma_{\epsilon}^2\vee 1)\s\log(np).
\end{equation*}
 \enlem
\begin{proof} 
\noindent \textbf{Case 1.} If $ |\I| < C_{\mclF} \s \log(n p)$, then by the definition of $\mclF(\beta, \mclI)$, we have $\mclF(\beta^*_{\I},\I)= \mclF(\widehat{\beta}_\J,\I) =0$ and the inequality holds automatically.
 
\noindent \textbf{Case 2.} If 
	\begin{equation}\label{eq-lem16-i-cond} 
		|\I| \geq  C_{\mclF} \s \log(n p),
	\end{equation}
	then letting $\delta_\I = \beta^*_\I  -\widehat \beta_\J$ and consider the high-probability event given in \Cref{lem:restricted eigenvalue}, we have
	\begin{align}
		& \sqrt{\sum_{t \in \I} (X_t^{\top} \delta_\I)^2} \geq {c_1'\sqrt{|\I|}} \|\delta_\I\|_2 - c_2'\sqrt{\log(p)} \|\delta_\I\|_1 \nonumber \\
		= & {c_1'\sqrt{|\I|}} \|\delta_\I\|_2 - c_2'\sqrt{\log(p)} \|(\delta_I)_{S}\|_1 - c_2'\sqrt{\log(p)} \|(\delta_\I)_{S^c}\|_1 \nonumber \\
		\geq & c_1'\sqrt{|\I|} \|\delta_\I\|_2 - c_2'\sqrt{\s\log(p)} \|\delta_\I\|_2 - c_2'\sqrt{\log(p)} \|(\delta_\I)_{S^c}\|_1 \nonumber \\
		\geq & \frac{c_1'}{2}\sqrt{|\I|} \|\delta_\I\|_2 - c_2'\sqrt{\log(p)} \|(\widehat{\beta}_\J)_{S^c}\|_1 \geq c_1\sqrt{|\I|} \|\delta_\I\|_2 - c_2\sqrt{\log(p)} \frac{\s \lambda}{\sqrt{|\I|}}, \label{eq-lem16-pf-1}
	\end{align} 
	where the last inequality follows from \Cref{lemma:interval lasso}t and the assumption that $(\beta^*_t)_i = 0$, for all $t\in [T]$ and $i\in S^c$. Then by the fact that $(a - b)^2\geq \frac{1}{2}a^2 - b^2$ for all $a,b\in \mathbb{R}$, it holds that
	\begin{equation}
	    \sum_{t \in \I} (X_t^{\top} \delta_\I)^2\geq \frac{c_1^2}{2}{|\I|} \|\delta_\I\|_2^2 - \frac{c_2^2  \lambda^2\s^2\log(p)}{|\I|}.
	\end{equation}
	Notice that
	\begin{align*}
	    & \sum_{t \in \I} (y_t - X_t^{\top} \beta^*_\I)^2 - \sum_{t \in \I} (y_t - X_t^{\top} \widehat{\beta}_\J)^2  = 2 \sum_{t \in \I} \epsilon_t X_t^{\top}\delta_\I  - \sum_{t \in \I} (X_t^{\top}\delta_\I)^2 \\
	\leq & 2\|\sum_{t \in \I }  X_t \epsilon_t \|_{\infty }  \left( \sqrt {\s} \| (\delta_\I)_{S} \|_2  + \| (\widehat \beta_\J)_{S^c} \|_1  \right)- \sum_{t \in \I} (X_t^{\top}\delta_\I)^2.
	\end{align*}
	Since for each $t$, $\epsilon_t$ is subgaussian with $\|\epsilon_t\|_{\psi_2}\leq \sigma_{\epsilon}$ and for each $i\in [p]$, $(X_t)_i$ is subgaussian with $\|(X_t)_i\|_{\psi_2}\leq C_x$, we know that $(X_t)_i\epsilon_t$ is subexponential with $\|(X_t)_i\epsilon_t\|_{\psi_1}\leq C_x\sigma_{\epsilon}$. Therefore, by Bernstein's inequality (see, e.g., Theorem 2.8.1 in \cite{vershynin2018high}) and a union bound, for $\forall u\geq 0$ it holds that
	\begin{equation*}
	    \mathbb{P}(\|\sum_{t \in \I }  X_t \epsilon_t \|_{\infty }> u)\leq 2p\exp(-c\min\{\frac{u^2}{|\I|C_x^2\sigma_{\epsilon}^2}, \frac{u}{C_x\sigma_{\epsilon}}\}).
	\end{equation*}
	Take $u = cC_x\sigma_{\epsilon}\sqrt{|\I|\log(np)}$, then by the fact that $|\I|\geq C_{\mclF}\s\log(np)$, it follows that with probability at least $1 - (np)^{-7}$,
	\begin{equation*}
	    \|\sum_{t \in \I }  X_t \epsilon_t \|_{\infty } \leq CC_x\sigma_{\epsilon}\sqrt{|\I|\log(np)}\leq \lambda \sqrt{|\I|},
	\end{equation*}
	where we use the fact that $\lambda=C_{\lambda}(\sigma_{\epsilon}\vee 1)\sqrt{\log(np)}$. Therefore, we have
	\begin{align*}
	& \sum_{t \in \I} (y_t - X_t^{\top} \beta^*_\I)^2 - \sum_{t \in \I} (y_t - X_t^{\top} \widehat{\beta}_\J)^2 \\
	\leq & 2\lambda\sqrt{|\I|\s}\|\delta_\I\|_2 + 2\lambda\sqrt{|\I|}\cdot \frac{\lambda \s}{ \sqrt{|\I|}} - \frac{c_1^2 |\I|}{2}\|\delta_\I\|_2^2 + \frac{c_2^2 \lambda^2 \s^2\log(p)}{|\I|}\\  
	\leq & 2\lambda\sqrt{|\I|\s}\|\delta_\I\|_2 + {2\lambda^2 \s} - \frac{c_1^2 |\I|}{2}\|\delta_\I\|_2^2 + \frac{c_2^2 \lambda^2 \s^2\log(p)}{|\I|} \\
	\leq & \frac{4}{c_1^2}\lambda^2\s + \frac{c_1^2}{4}|\I| \|\delta_\I\|^2_2 + {2\lambda^2 \s} - \frac{c_1^2}{2}|\I|\|\delta_\I\|^2_2 + \frac{c_2^2 \lambda^2 \s^2\log(p)}{C_{\mclF}\s\log(np)} \\
	\leq & {c_3\lambda^2\s} + {2\lambda^2 \s} + \frac{c_2^2 \lambda^2 \s^2\log(p)}{C_{\mclF}\s\log(np)}\\
	\leq & c_4\lambda^2 \s.
	\end{align*}
	where the third inequality follows from $2ab \leq a^2 + b^2$. 

\end{proof} 










 
 
 
 \bnlem \label{lemma: regression dcdp one change point}
Suppose the good events 
$\mathcal L (\tr ) $ and  $\mathcal R (\tr) $ defined  in \Cref{eq:left and right approximation of change points} hold. 
Let   $ \I=(s,e] \in \mathcal {\widehat P}  $  be such that $\I$ contains exactly  one  true  change point $ \eta_k $. 
Suppose $\gamma \geq C_\gamma K\tr \kappa^2   $.  Then  with probability  at least $1- n^{-3}$,   it holds that 
\begin{equation*}
    \min\{ \eta_k -s ,e-\eta_k \}   \lesssim \frac{\sigma_{\epsilon}^2\vee 1  }{\kappa^2 }\bigg(  \s \log(np) +\gamma \bigg)  +  \tr.
\end{equation*}
\enlem
\begin{proof}    
If either $ \eta_k -s \le  C_\mclF \s \log(np)   $ or $e-\eta_k\le C_\mclF \s \log(np)  $, then 
$$ \min\{ \eta_k -s ,e-\eta_k \}   \le C_\mclF \s \log(np)  $$
and there is nothing to show. So assume that 
$$  \eta_k -s  > C_\mclF \s \log(np)  \quad \text{and} \quad   e-\eta_k  >C_\mclF \s \log(np)  . $$
By event $\mathcal R (\tr )$, there exists  $ s_ u  \in \{ s_q\}_{q=1}^\Q$ such that 
$$0\le s_u - \eta_k \le \tr. $$

\begin{center}
 \begin{tikzpicture} 
\draw[ - ] (-10,0)--(-1,0);
 \node[color=black] at (-8,-0.3) {\small s};
 \draw[  (-, ultra thick, black] (-8,0) -- (-7.99,0);
  \draw[ { -]}, ultra thick, black] (-3.0002,0) -- (-3,0);

   \node[color=black] at (-7,-0.3) {\small $\eta_k$};
\draw(-7 ,0)circle [radius=2pt] ;

  \node[color=black] at (-6.5,-0.3) {\small $s_u$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-6.5,0)  }; 
  
  \node[color=black] at (-3 ,-0.3) {\small $e$};
\end{tikzpicture}
\end{center} 

{\bf Step 1.} Denote 
$$ \I_ 1 = (s,s_u] \quad \text{and} \quad \I_2 = (s_u, e] .$$
Since 
$ \eta_k-s \ge C_\mclF \s \log(np)    , $
it follows that 
   $ |\I| \ge C_\mclF \s \log(np)   $ and $ |\I_1| \ge C_\mclF \s \log(np)   $. Thus 
$$ \mathcal F  (\I)  = \sum_{ i \in \I } (y_i - X_i^\top \widehat \beta_\I )^2 \quad \text{and} \quad \mathcal F  (\I_1)  = \sum_{ i \in {\I_1}  } (y_i - X_i^\top \widehat \beta_{\I_1}  )^2  .$$
Since $\I\in \widehat { \mathcal P}$, it holds that 
\begin{align}\label{eq:regression one change basic inequality step 1} \mathcal F  (\I)  \le  \mathcal F  (\I_1)  +  \mathcal F  (\I_2)  + \gamma. 
\end{align}

{\bf Case a.} Suppose $|\I_2| <C_\mclF \s \log(np)      $.
It follows from \Cref{eq:regression one change basic inequality step 1} that 
\begin{align}\nonumber
\sum_{i \in \I }(y_i - X_i^\top \widehat \beta _\I ) ^2 \le &  \sum_{i \in \I_1 }(y_i -X_i^\top  \widehat \beta _{\I_1}  ) ^2 +  0  + \gamma 
\\ \nonumber 
\le &  \sum_{i \in \I_1 }(y_i -  X_i^\top  \beta^*  _i  ) ^2 + C_1 \big ( (s_u -\eta_k) \kappa_k^2   + \s  \log(np)  \big )   +    \gamma
\\ \nonumber 
\le &  \sum_{i \in \I _1}(y_i -  X_i^\top  \beta^*  _i ) ^2  +C_1 \big (  \tr  \kappa_k^2   +  \s \log(np )    \big ) +  \gamma
\\
\le &   \sum_{i \in \I  }(y_i -  X_i^\top  \beta^*  _i  ) ^2  +C_1 \big (  \tr  \kappa_k^2   +  \s \log(np )    \big ) +  \gamma  , \label{eq:regression one change point step 1  case a}
\end{align}
where the first inequality follows from the fact that $  \mathcal F  (\I_2)  = 0  $ when $|\I_2| < C_\mclF \s \log(np)   $,    the second inequality follows from \Cref{lam:regression one change deviation bound}   {\bf b}, the third inequality follows from  the assumption  that 
$   (s_u-\eta_k) \le  \tr   $,   and the inequality holds because $ \sum_{i \in \I _2 }(y_i -  X_i^\top  \beta^*  _i  ) ^2\ge 0 $.

{\bf Case b.} Suppose $|\I_2|  \ge C_\mclF \s \log(np)   $.
It follows from \Cref{eq:regression one change basic inequality step 1} that  
\begin{align}\nonumber
\sum_{i \in \I }(y_i - X_i^\top \widehat \beta _\I ) ^2 \le &  \sum_{i \in \I_1 }(y_i -X_i^\top  \widehat \beta _{\I_1}  ) ^2 +  \sum_{i \in \I_2  }(y_i -X_i^\top  \widehat \beta _{\I_2 }  ) ^2   + \gamma 
\\ \nonumber 
\le &  \sum_{i \in \I_1 }(y_i -  X_i^\top  \beta^*  _i  ) ^2 + C_1 \big ( (s_u -\eta_k) \kappa_k^2   + \s  \log(np)  \big )  
\\  \nonumber 
+ & \sum_{i \in \I_2 }(y_i -  X_i^\top  \beta^*  _i  ) ^2 + C_1     \s  \log(np)     + 2  \gamma
\\ 
\le &  \sum_{i \in \I }(y_i -  X_i^\top  \beta^*  _i ) ^2  +C_2 \big (  \tr  \kappa_k^2   +  \s \log(np )    \big ) +  \gamma, \label{eq:regression one change point step 1 case b}
\end{align}
where    the second inequality follows from \Cref{lam:regression one change deviation bound}  {\bf a} and {\bf b}, and the third inequality follows from  the assumption  that 
$   (s_u-\eta_k) \le  \tr   $. Combing two cases leads to 
\begin{align} 
\sum_{i \in \I }(y_i - X_i^\top \widehat \beta _\I ) ^2  
\le     \sum_{i \in \I  }(y_i -  X_i^\top  \beta^*  _i  ) ^2  +C_2 \big (  \tr  \kappa_k^2   +  \s \log(np )    \big ) +  \gamma . \label{eq:two change point step 1}
\end{align}
\\
\\
{\bf Step 2.}
Denote 
$$ \J_1  = (s,\eta_k ] \quad \text{and} \quad \J_2 = (\eta_k , e] .$$
\Cref{eq:one change point step 1}  gives 
\begin{align}  \nonumber 
& \sum_{i \in \J_1 }(y_i  -X_i^\top  \widehat \beta _\I ) ^2 +\sum_{i \in \J_2 }(y_i - X_i^\top  \widehat \beta _\I  ) ^2  
\\ 
 \le \label{eq:regression step 2 first term} & \sum_{i \in \J_1  }(y_i -  X_i^\top    \beta _{\J _1}  ^*    ) ^2   +\sum_{i \in \J_2  }(y_i - X_i^\top    \beta _{\J _1}  ^*  ) ^2  +C_2  \big (     \tr \kappa_k^2  +\s \log(np)  \big )  +   \gamma 
\end{align}
The above display  leads to 
\begin{align} \nonumber
&\sum_{i \in \J_1 } \big\{ X_i^\top  (  \widehat \beta _\I  -  \beta^* _{\J_1 }) \big\}  ^2 +\sum_{i \in \J_2  } \big\{ X_i^\top  (  \widehat \beta _\I  -  \beta^* _{\J_2 }) \big\}  ^2  
\\ \nonumber 
 \le  & 2 \sum_{i \in \J_1  } \epsilon_i  X_i^\top (  \widehat \beta _\I  -  \beta^* _{\J_1 })     +2 \sum_{i \in \J_2  } \epsilon_i  X_i^\top (  \widehat \beta _\I  -  \beta^* _{\J_2 })      +C_2  \big (     \tr   \kappa_k^2   +\s\log(np)  \big )  +  \gamma 
 \\ \label{eq:regression one change step 2 term 2}
 \le  & C_3  \sqrt { \log(np)    |\J_1| }  \|  \widehat \beta _\I  -  \beta^* _{\J_1 }\| _1  + C_3  \sqrt { \log(np)  |\J_2| }  \|  \widehat \beta _\I  -  \beta^* _{\J_2  }\| _1+ C_2  \big (     \tr \kappa_k^2  +\s \log(np)  \big ) +    \gamma 
\end{align} 
where the last inequality follows from \Cref{lemma:consistency} and  that  $|\J_1|   \ge  C_\mclF \s \log(np)   $ and $|\J_2|  \ge C_\mclF \s \log(np)   $.
Note that 
\begin{align*} 
\|  ( \widehat \beta _\I  -  \beta _{\J_1}^* )_{S^c } \|_1 = \|  ( \widehat \beta _\I )_{S^c} \|_{1} 
=   \|  ( \widehat \beta _\I -\beta _\I ^* )_{S^c} \|_{1}  \le 3 \|  ( \widehat \beta _\I -\beta _\I ^* )_{S } \|_{1}   \le C_5 \s \sqrt { \frac{ \log(np)}{| \I|} }    , 
\end{align*} 
where the last two inequalities follows from \Cref{lemma:interval lasso}.  So
\begin{align}  \label{eq:regression one change step 2 term 1}
\|   \widehat \beta _\I  -  \beta _{\J_1}^*   \|_1 = \|  ( \widehat \beta _\I  -  \beta _{\J_1}^* )_{S  } \|_1 +\|  ( \widehat \beta _\I  -  \beta _{\J_1}^* )_{S^c } \|_1  \le \sqrt {\s }  \|  \widehat \beta _\I  -  \beta _{\J_1}^*   \|_2 + C_5 \s \sqrt { \frac{ \log(np)}{| \I|} } .
\end{align} 
Therefore  \Cref{eq:regression one change step 2 term 2} gives 
\begin{align} \nonumber 
& \sum_{i \in \J_1 } \big\{ X_i^\top  (  \widehat \beta _\I  -  \beta^* _{\J_1 }) \big\}  ^2 +\sum_{i \in \J_2  } \big\{ X_i^\top  (  \widehat \beta _\I  -  \beta^* _{\J_2 }) \big\}  ^2   
\\  \nonumber 
\le & C_3  \sqrt { \log(np)    |\J_1| }   \bigg(  \sqrt {\s }  \|  \widehat \beta _\I  -  \beta _{\J_1}^*   \|_2 + C_5 \s \sqrt { \frac{ \log(np)}{| \I|} } \bigg) 
\\ \nonumber  
+ & C_3  \sqrt { \log(np)    |\J_2| }   \bigg(  \sqrt {\s }  \|  \widehat \beta _\I  -  \beta _{\J_2}^*   \|_2 + C_5 \s \sqrt { \frac{ \log(np)}{| \I|} } \bigg)  +2\gamma 
\\ \nonumber  
\le & \frac{ c_x | \J_1|}{64} \|  \widehat \beta _\I  -  \beta _{\J_1}^*   \|_2  ^2 + \frac{ c_x | \J_2|}{64} \|  \widehat \beta _\I  -  \beta _{\J_2}^*   \|_2  ^2   + C_5'   \s \log(np)
\\ +&C_2  \big (     \tr \kappa_k^2  +\s \log(np)  \big )   +2\gamma,
 \label{eq:regression one change step 2 term 3}
\end{align}
   $ |\J_1| \le |\I| , |\J_2| \le |\I|  $ are used in the last inequality. 
\\
\\
{\bf Step 3.}  Since     $|\J_1|   \ge  C_\mclF  \s \log(np)   $ and $|\J_2|  \ge C_\mclF \s \log(np)   $, for $\ell=1, 2$,
  it holds that
 \begin{align}\nonumber 
		&  \sum_{i \in \J_\ell  } \big\{ X_i^\top  (  \widehat \beta _\I  -  \beta^* _{\J_ \ell  }) \big\}  ^2 
		 \\  \nonumber  
		  \ge&  \frac{c_x|\J_\ell | }{16} \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_2^2 - C_6  \log(p) \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_1  ^2 
		 \\\nonumber  
		 \ge & \frac{c_x|\J_\ell | }{16} \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_2^2 - C_6' \s   \log(p) \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_ 2   ^2  - C_6'  \frac{  \s^2 \log(p) \log(np)  }{|\I| }
		 \\ \label{eq:regression one change step 3 term 1}
		 \ge &  \frac{c_x|\J_\ell | }{32} \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_2^2 - C_7  \s \log(np),
	\end{align} 
	where the first inequality follows from   
 \Cref{lem:restricted eigenvalue},  the second inequality follows from \Cref{eq:regression one change step 2 term 1}   and the last inequality follows from the observation that 
 $$ |\I| \ge |\J_\ell|  \ge   C_\mclF \s \log(np). $$
 \Cref{eq:regression one change step 2 term 3} and \Cref{eq:regression one change step 3 term 1} together lead to 
 $$   |\J_1  |   \|\widehat \beta _\I  -  \beta^* _{\J_ 1  } \|_2^2  + |\J_2  |   \|\widehat \beta _\I  -  \beta^* _{\J_ 2  } \|_2^2  \le C_8(\s \log(np) + \tr \kappa_k^2 + \gamma) .$$
Observe  that 
$$ \inf_{  \beta  \in \mathbb R ^p   }  |\J_1 |  \| \beta    -  \beta^* _{\J_ 1  } \|_2^2  + |\J_2 | \|  \beta    -  \beta^* _{\J_ 2  } \|_2^2    = \kappa_k ^2  \frac{|\J_1| |\J_2|}{| \I| }   \ge \frac{ \kappa_k^2 }{2} \min\{ |\J_1| ,|\J_2| \}    . $$ 
This leads to 
$$  \frac{ \kappa_k^2 }{2}\min\{ |\J_1| ,|\J_2| \}    \le  C_8(\s \log(np)+\tr  + \gamma)  .$$
Since $\kappa_k \asymp \kappa $, it follows that 
$$ \min\{ |\J_1| ,|\J_2| \}   \le C_9 \bigg( \frac{\s \log(np) + \gamma  }{\kappa 	^2 } +  \tr  \bigg) .$$
 \end{proof} 
  


 \bnlem  \label{lemma:regression two change points}
Suppose the good events 
$\mathcal L (\tr ) $ and  $\mathcal R ( \tr ) $  in  \Cref{eq:left and right approximation of change points} hold. 
Let   $ \I=(s,e] \in \mathcal {\widehat P}  $  be such that $\I$ contains  exactly two  change points $ \eta_k,\eta_{k+1}  $.  Suppose in addition that 
\begin{align} \label{eq:regression two change points snr}
\Delta \kappa^2 \ge  C     \big( \sigma_{\epsilon}^2\s \log(np) + \gamma)    
\end{align} 
for sufficiently large constant $C   $ and that 
$\gamma \ge  C_\gamma \Bn^{-1}\Delta\kappa^2   $.
 Then  with probability  at least $1- n^{-3}$,   it holds that 
\begin{align*} 
 \eta_k -s     \lesssim  \frac{\sigma_{\epsilon}^2\vee 1  }{\kappa^2 }\bigg(  \s \log(np) +\gamma \bigg) +  \tr   \quad \text{and} \quad 
 e-\eta_{k+1}   \lesssim \frac{\sigma_{\epsilon}^2\vee 1  }{\kappa^2 }\bigg(  \s \log(np) +\gamma \bigg) +  \tr  ,
 \end{align*} 
 where $C_0\ge 1 $ is some sufficiently large constant.
 \enlem 
\begin{proof} 
By symmetry, it suffices to show that $\eta_k-s\lesssim \frac{\sigma_{\epsilon}^2\vee 1  }{\kappa^2 }\bigg(  \s \log(np) +\gamma \bigg) +  \tr$.  If 
$$\eta_k-s  \le  C_\mclF \s \log(np) , $$
then the desired result follows immediately.  
So it suffices to assume that 
$$\eta_k-s > C_\mclF \s \log(np) .  $$
Since the events $\mathcal L ( \tr  ) $ and  $\mathcal R ( \tr ) $ hold, let $ s_u, s_v$ be such that 
 $\eta_k \le s_u \le s_v \le \eta_{k+1} $ and that 
 $$ 0 \le s_u-\eta_k \le   \tr ,  \quad  0\le  \eta_{k+1} - s_v \le \tr   .    $$
 \
 \\
 \begin{center}
 \begin{tikzpicture} 
\draw[ - ] (-10,0)--(1,0);
 \node[color=black] at (-8,-0.3) {\small s};
 \draw[  (-, ultra thick, black] (-8,0) -- (-7.99,0);
  \draw[ { -]}, ultra thick, black] (-1.0002,0) -- (-1,0);

   \node[color=black] at (-7,-0.3) {\small $\eta_k$};
\draw(-7 ,0)circle [radius=2pt] ;

  \node[color=black] at (-6.5,-0.3) {\small $s_u$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-6.5,0)  }; 
 

  \node[color=black] at (-2.3,-0.3) {\small $\eta_{k+1}$};
\draw(-2.3 ,0)circle [radius=2pt] ;
  \node[color=black] at (-3 ,-0.3) {\small $s_v$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-3,0)  }; 
  
   \node[color=black] at (-1,-0.3) {\small $e$};

 
\end{tikzpicture}
\end{center} 
\
\\
{\bf Step 1.} Denote 
 $$ \mathcal I_ 1= (  s, s _u], \quad \I_2  =(s_u, s_v] \quad \text{and} \quad \I_3  = (s_v,e]. $$
 \
 \\
Since  $ |\I| \ge \eta_{k+1} -\eta_k \ge C_\mclF \s \log(np)   $, 
$$ \mathcal F(\I ) = \sum_{i \in \I }(y_i - X_i^\top \widehat \beta _\I ) ^2  . $$
Since 
 $ |\I_1|  \ge  \eta_k-s      \ge C_\mclF \s \log(np)   , $ 
it follows that 
 $$ \mathcal F(\I_1 ) = \sum_{i \in \I_1 }(y_i - X_i^\top \widehat \beta _{\I_1}  ) ^2  . $$
In addition   since  $ |\I_1| \ge C_\mclF \s \log(np)  $, then 
 \begin{align*}\mathcal F(\I_1)  = & \sum_{i \in \I_1 }(y_i - X_i^\top \widehat \beta _{\I_1}  ) ^2 
 \\
 \le & \sum_{i \in \I_1 }(y_i - X_i^\top   \beta ^*  _i   ) ^2  + C_1  \bigg\{ \frac{( \eta_k-s) (s_u -\eta_k ) }{ ( \eta_k-s)  + (s_u -\eta_k )  } \kappa ^2 + \s\log(np)  \bigg\} 
 \\
  \le & \sum_{i \in \I_1 }(y_i - X_i^\top   \beta ^*  _i   ) ^2  +  C_1 \bigg\{ (s_u -\eta_k )   \kappa ^2 +  \s\log(np)  \bigg\} 
  \\
  \le & \sum_{i \in \I_1 }(y_i - X_i^\top   \beta ^*  _ i   ) ^2  + C_1 \bigg\{  \tr   \kappa ^2 +  \s\log(np)  \bigg\} ,
 \end{align*}
where the first  inequality follows  from \Cref{lam:regression one change deviation bound}  and that $ \kappa_{k} \asymp \kappa$.
 Similarly, since 
 $ |\I_2|  \ge \Delta /2 \ge   C_\mclF \s \log(np)   , $ 
it follows that 
 $$ \mathcal F(\I_2 ) = \sum_{i \in \I_2 }(y_i - X_i^\top \widehat \beta _{\I_2}  ) ^2  . $$
  Since $|\I_2| \ge C_\mclF \s \log(np)   $ and  $\I_2$ contains no change points, by \Cref{lam:regression one change deviation bound},
  \begin{align*}\mathcal F(\I_2)  \le \sum_{i \in \I_2 }(y_i - X_i^\top   \beta ^*  _ i  ) ^2   + C_1\s\log(np).
  \end{align*}  
  \\
  \\
 {\bf Step 2.} If $ |\I_3 | \ge C_\mclF \s \log(np)   $, then 
  \begin{align*}\mathcal F(\I_3)  = & \sum_{i \in \I_3 }(y_i - X_i^\top \widehat \beta _{\I_3}  ) ^2 
 \\
 \le & \sum_{i \in \I_3 }(y_i - X_i^\top   \beta ^*  _i   ) ^2  + C_1  \bigg\{ \frac{( \eta_{k+1}-s_v) (e -\eta_{k+1} ) }{ ( \eta_{k+1}-s_v)+  (e -\eta_{k+1} )  } \kappa ^2 + \s\log(np)  \bigg\} 
 \\
  \le & \sum_{i \in \I_3 }(y_i - X_i^\top   \beta ^*  _i   ) ^2  +  C_1 \bigg\{ ( \eta_{k+1}-s_v)    \kappa ^2 +  \s\log(np)  \bigg\} 
  \\
  \le & \sum_{i \in \I_3 }(y_i - X_i^\top   \beta ^*  _ i   ) ^2  + C_1 \bigg\{  \tr   \kappa ^2 +  \s\log(np)  \bigg\} ,
 \end{align*}
 where the first inequality follows from \Cref{lam:regression one change deviation bound}{\bf b} and that $ \kappa_{k+1} \asymp \kappa$. 
 If $|\I_3| < C_\mclF \s \log(np)   $, then 
$\mathcal F(\I_3)  =  0 $.
 So 
both cases imply that  
 $$\mathcal F(\I_3)  \le \sum_{i \in \I_3 }(y_i - X_i^\top   \beta ^*  _ i   ) ^2  + C_1 \bigg\{  \tr   \kappa_k^2 +  \s\log(np)  \bigg\}  .$$
 \
 \\
 {\bf Step 3.} Since $\I \in \widehat{\mathcal P} $, we have
 \begin{align}\label{eq:regression two change points local min} \mathcal F(\I ) \le \mathcal F(\I_1  ) +\mathcal F(\I_2 )+\mathcal F(\I_3 ) + 2\gamma. 
 \end{align} The above display and the calculations in  {\bf Step 1} and  {\bf Step 2} implies that
\begin{align} 
 \sum_{i \in \I }(y_i -  X_i^\top \widehat \beta _\I ) ^2  
\le   \sum_{i \in \I  }(y_i -   X_i^\top \beta_i^*   ) ^2  
 +   3  C_1 \bigg\{  \tr   \kappa ^2 +  \s\log(np) \bigg\}
+2\gamma  .
  \label{eq:regression two change points step 2 term 1}
\end{align}
Denote 
$$ \J_1  = (s,\eta_k ], \quad \J_2=(\eta_k, \eta_{k} +   \eta_{k+1}    ]  \quad \text{and} \quad \J_3 = (\eta_{k+1}  , e] .$$
\Cref{eq:regression two change points step 2 term 1}  gives 
\begin{align} 
 \sum_{\ell=1}^3 \sum_{i \in \J_{\ell}  }(y_i - X_i^\top  \widehat \beta _\I ) ^2 
 \le& \sum_{\ell=1}^3 \sum_{i \in \J_ \ell  }(y_i -  X_i^\top    \beta^*  _{\J_\ell }  ) ^2    
 +  3  C_1 \bigg\{  \tr   \kappa ^2 +  \s\log(np) \bigg\} 
+2\gamma     \label{eq:regression two change points first}
\end{align} 
\
\\
{\bf Step 4.} 
Note that for $\ell\in \{1,2,3\}$, 
\begin{align*} 
\|  ( \widehat \beta _\I  -  \beta _{\J_\ell }^* )_{S^c } \|_1 = \|  ( \widehat \beta _\I )_{S^c} \|_{1} 
=   \|  ( \widehat \beta _\I -\beta _\I ^* )_{S^c} \|_{1}  \le 3 \|  ( \widehat \beta _\I -\beta _\I ^* )_{S } \|_{1}   \le C_2 \s \sqrt { \frac{ \log(np)}{| \I|} }    , 
\end{align*} 
where the last two inequalities follows from \Cref{lemma:interval lasso}.  So
\begin{align}  \label{eq:regression two change step 3 term 1}
\|   \widehat \beta _\I  -  \beta _{\J_\ell}^*   \|_1 = \|  ( \widehat \beta _\I  -  \beta _{\J_\ell }^* )_{S  } \|_1 +\|  ( \widehat \beta _\I  -  \beta _{\J_\ell}^* )_{S^c } \|_1  \le \sqrt {\s }  \|  \widehat \beta _\I  -  \beta _{\J_\ell}^*   \|_2 + C_2 \s \sqrt { \frac{ \log(np)}{| \I|} } .
\end{align} 
Note that by assumptions,
$$|\J_1|\ge C_\mclF \s \log(np)    \quad \text{and} \quad |\J_2 |\ge C_\mclF \s \log(np) .$$
 So for $\ell\in \{ 1, 2\} $,
  it holds that
 \begin{align}\nonumber 
		&  \sum_{i \in \J_\ell  } \big\{ X_i^\top  (  \widehat \beta _\I  -  \beta^* _{\J_ \ell  }) \big\}  ^2 
		 \\  \nonumber  
		  \ge&  \frac{c_x|\J_\ell | }{16} \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_2^2 - C_3 \log(p) \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_1  ^2 
		 \\\nonumber  
		 \ge & \frac{c_x|\J_\ell | }{16} \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_2^2 - C_3' \s   \log(p) \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_ 2   ^2  - C_3'  \frac{  \s^2 \log(p) \log(np)  }{|\I| }
		 \\ \label{eq:regression two change step 3 term 2}
		 \ge &  \frac{c_x|\J_\ell | }{32} \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_2^2 - C_4  \s \log(np),
	\end{align} 
	where the first inequality follows from \Cref{lem:restricted eigenvalue}, the second inequality follows from \Cref{eq:regression two change step 3 term 1}   and the last inequality follows from the observation that 
 $$  |\I|\ge  |\J_\ell|   \ge C_\gamma \s \log(np). 
 $$ 
 So for $\ell\in \{ 1,2\}$, 
\begin{align*} &\sum_{i \in \J_\ell  }(y_i - X_i^\top  \widehat \beta _\I ) ^2  - \sum_{i \in \J_\ell   }(y_i - X_i^\top    \beta^*  _{\J_\ell }  ) ^2
=  \sum_{i \in \J_\ell    }\big\{ X_i^\top (\widehat \beta _\I -\beta^*  _{\J_4} )\big\}^2 -2 \sum_{i \in \J_\ell   } \epsilon_i X_i^\top (\widehat \beta _\I -\beta^*  _{\J_\ell  }  )
\\
\ge  & \sum_{i \in \J_\ell   }\big\{ X_i^\top (\widehat \beta _\I -\beta^*  _{\J_\ell  } )\big\}^2  - 2 \| \sum_{i \in \J_\ell   }  \epsilon_i X_i^\top \|_\infty \| \widehat \beta _\I -\beta^*  _{\J_\ell  }  \|_1
\\
\ge &\sum_{i \in \J_\ell   }\big\{ X_i^\top (\widehat \beta _\I -\beta^*  _{\J_\ell  } )\big\}^2  - C_5 \sqrt{ \log(np) |\J_\ell|   }\bigg(\sqrt {\s }  \|  \widehat \beta _\I  -  \beta _{\J_1}^*   \|_2 + C_2 \s \sqrt { \frac{ \log(np)}{| \I|} } \bigg) 
\\
\ge &  \frac{c_x|\J_\ell | }{32} \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_2^2 - C_4  \s \log(np)  - C_5 \sqrt{ \log(np) |\J_\ell|  }\bigg(\sqrt {\s }  \|  \widehat \beta _\I  -  \beta _{\J_1}^*   \|_2 + C_2 \s \sqrt { \frac{ \log(np)}{| \I|} } \bigg)  
\\
\ge & \frac{c_x|\J_\ell | }{32} \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_2^2 -\frac{c_x|\J_\ell | }{64} \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_2^2 -C_6 \s \log(np)  
= \frac{c_x|\J_\ell | }{64} \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_2^2     -C_6 \s \log(np)  ,
\end{align*}
where the second inequality follows from the standard sub-Exponential tail bound and \Cref{eq:regression two change step 3 term 1}, the third inequality follows from \Cref{eq:regression two change step 3 term 2}, and the fourth inequality follows from  $ \J_\ell \subset \I $ and so $ |\I | \ge |\J_\ell|$.
\\
\\
So for $\ell \in \{1,2 \}$, 
\begin{align} \label{eq:regression change point step 3 last item}\sum_{i \in \J_\ell  }(y_i - X_i^\top  \widehat \beta _\I ) ^2  - \sum_{i \in \J_\ell   }(y_i - X_i^\top    \beta^*  _{\J_\ell }  ) ^2 
\ge \frac{c_x|\J_\ell | }{64} \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_2^2     -C_6 \s \log(np).
\end{align} 
\
\\
\\
{\bf Step 5.} For $\J_3$, if $|\J_3| \ge C_\mclF \s \log(np)  $,  following the same calculations as in {\bf Step 4}, 
$$\sum_{i \in \J_ 3 }(y_i - X_i^\top  \widehat \beta _\I ) ^2  - \sum_{i \in \J_ 3 }(y_i - X_i^\top    \beta^*  _{\J_3   }  ) ^2 \ge \frac{c_x|\J_3   | }{64} \|\widehat \beta _\I  -  \beta^* _{\J_ 3  } \|_2^2     -C_6 \s \log(np)  \ge -C_6 \s\log(np). 
$$
If $|\J_3 | < C_\mclF \s \log(np) $, then
\begin{align} & \sum_{i \in \J_3   }(y_i - X_i^\top  \widehat \beta _\I ) ^2  - \sum_{i \in \J_3   }(y_i - X_i^\top    \beta^*  _{\J_ 3}  ) ^2 \nonumber 
=   \sum_{i \in \J_ 3   }\big\{ X_i^\top (\widehat \beta _\I -\beta^*  _{\J_3} )\big\}^2 -2 \sum_{i \in \J_3   } \epsilon_i X_i^\top (\widehat \beta _\I -\beta^*  _{\J_3 }  )
\\  \nonumber 
\ge  & \sum_{i \in \J_3   }\big\{ X_i^\top (\widehat \beta _\I -\beta^*  _{\J_3 } )\big\}^2  -\frac{1}{2 }\sum_{i \in \J_3   }\big\{ X_i^\top (\widehat \beta _\I -\beta^*  _{\J_3 } )\big\}^2  - 4   \sum_{i \in \J_3   }\epsilon_i^2 
\\  \nonumber 
\ge & \frac{1}{2 }\sum_{i \in \J_3   }\big\{ X_i^\top (\widehat \beta _\I -\beta^*  _{\J_3 } )\big\}^2  -C_7\bigg(  \sqrt { \gamma   \log(n)} + \log(n)+ \gamma  \bigg) 
\\  \nonumber  
\ge & \frac{1}{2 }\sum_{i \in \J_3   }\big\{ X_i^\top (\widehat \beta _\I -\beta^*  _{\J_3 } )\big\}^2  -C_7' \bigg(     \log(n)+ \gamma   \bigg)  
\\ \ge 
& \frac{1}{2 }\sum_{i \in \J_3   }\big\{ X_i^\top (\widehat \beta _\I -\beta^*  _{\J_3 } )\big\}^2  -C_8    ( \s\log(np) + \gamma) 
\ge -C_8    (  \s\log(np) +\gamma)   \label{eq:regression change point step 4 last item}
\end{align}
where the second inequality follows from the standard sub-exponential deviation bound.
\
\\
\\
{\bf Step 6.} Putting \Cref{eq:regression two change points first}, \eqref{eq:regression change point step 3 last item} and \eqref{eq:regression change point step 4 last item} together, it follows that 
 $$  \sum_{\ell =1}^2 \frac{c_x|\J_\ell | }{64} \|\widehat \beta _\I  -  \beta^* _{\J_ \ell  } \|_2^2      \le C_9(\s \log(np) + \tr \kappa ^2 + \gamma) .$$
 This leads to 
  $$     |\J_1 |   \|\widehat \beta _\I  -  \beta^* _{\J_ 1  } \|_2^2     + |\J_2 |   \|\widehat \beta _\I  -  \beta^* _{\J_ 2  } \|_2^2       \le C_9(\s \log(np) + \tr \kappa ^2 + \gamma) .$$ 
Observe  that 
$$ \inf_{  \beta  \in \mathbb R ^p   }  |\J_1 |  \| \beta    -  \beta^* _{\J_ 1  } \|_2^2  + |\J_2 | \|  \beta    -  \beta^* _{\J_ 2  } \|_2^2    = \kappa_k   ^2  \frac{|\J_1| |\J_2|}{| \J_1| +|\J_2|  }   \ge \frac{ \kappa_k  ^2 }{2} \min\{ |\J_1| ,|\J_2| \}   \ge   \frac{ c \kappa   ^2 }{2} \min\{ |\J_1| ,|\J_2| \}   . $$ 
Thus
$$    \kappa ^2 \min\{ |\J_1| ,|\J_2| \}    \le  C_{10} (\s \log(np)+\tr \kappa^2  + \gamma)  ,$$
which is 
$$ \min\{ |\J_1| ,|\J_2| \}   \le C_5 \bigg( \frac{\s \log(np) + \gamma  }{\kappa ^2 } +  \tr  +\frac{ \gamma}{\kappa ^2} \bigg) .$$ 
Since  $ |\J_2  | \ge \Delta \ge     \frac{  C     ( \s \log(np) + \gamma) }{   \kappa^{2}}   $
 for sufficiently large constant $C$, 
 it follows that
 $$ |\J_2| \ge \Delta>  C_5 \bigg( \frac{\s \log(np) + \gamma  }{\kappa ^2 } +  \tr  +\frac{ \gamma}{\kappa ^2} \bigg) .$$  So it holds that 
 $$   |\J_1|    \le C_5 \bigg( \frac{\s \log(np) + \gamma  }{\kappa ^2 } +  \tr  \bigg) .$$ 
 \end{proof} 

 \bnlem 
Suppose the good events 
$\mathcal L (\tr ) $ and  $\mathcal R ( \tr ) $ defined  in  \Cref{eq:left and right approximation of change points} hold. 
 Suppose in addition that 
\begin{align} \label{eq:regression three change points snr}
\Delta \kappa^2 \ge C      \big( \s \log(np) + \gamma)    
\end{align} 
for sufficiently large constant $C $. 
 Then  with probability  at least $1- n^{-3}$,    there is no intervals in   $  \widehat { \mathcal P}  $  containing three or more true change points.   
 \enlem  
 


\begin{proof} For  contradiction,  suppose    $ \I=(s,e] \in \mathcal {\widehat P}  $  be such that $ \{ \eta_1, \ldots, \eta_M\} \subset \I $ with $M\ge 3$.  
\\
\\ 
Since the events $\mathcal L ( \tr  ) $ and  $\mathcal R ( \tr ) $ hold, by relabeling $\{ s_q\}_{q=1}^\Q  $ if necessary,   let $ \{ s_m\}_{m=1}^M $ be such that 
 $$ 0 \le s_m  -\eta_m  \le \tr    \quad \text{for} \quad 1 \le m \le M-1  $$ and that
 $$ 0\le \eta_M  - s_M \le \tr .$$ 
 Note that these choices ensure that  $ \{ s_m\}_{m=1}^M  \subset \I . $
 \
 \\
 \begin{center}
 \begin{tikzpicture} 
\draw[ - ] (-10,0)--(1,0);
 \node[color=black] at (-8,-0.3) {\small s};
 \draw[  (-, ultra thick, black] (-8,0) -- (-7.99,0);
  \draw[ { -]}, ultra thick, black] (-1.0002,0) -- (-1,0);

   \node[color=black] at (-7,-0.3) {\small $\eta_1$};
\draw(-7 ,0)circle [radius=2pt] ;

  \node[color=black] at (-6.5,-0.3) {\small $s_1$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-6.5,0)  }; 

  \node[color=black] at (-5,-0.3) {\small $\eta_2$};
\draw(-5 ,0)circle [radius=2pt] ;
  \node[color=black] at (-4.5,-0.3) {\small $s_2$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-4.5,0)  }; 
 

  \node[color=black] at (-2.5,-0.3) {\small $\eta_M$};
\draw(-2.5 ,0)circle [radius=2pt] ;
  \node[color=black] at (-3 ,-0.3) {\small $s_M$};
\draw plot[mark=x, mark options={color=black, scale=1.5}] coordinates {(-3,0)  }; 
  
   \node[color=black] at (-1,-0.3) {\small $e$};

 
\end{tikzpicture}
\end{center}
\
\\
{\bf Step 1.}
 Denote 
 $$ \mathcal I_ 1= (  s, s _1], \quad \I_m   =(s_{m-1} , s_m] \text{ for }  2 \le m \le M     \quad \text{and} \quad \I_{M+1}   = (s_M,e]. $$
 Then since $|\I| \ge \Delta \ge  C_s \s \log(np)  $, it follows that 
 Since  $ |\I| \ge \eta_{k+1} -\eta_k \ge  C_s \s \log(np) $, 
$$ \mathcal F(\I ) = \sum_{i \in \I }(y_i - X_i^\top \widehat \beta _\I ) ^2  . $$
Since  $ | \I_m | \ge \Delta /2 \ge   C_s \s \log(np) $ for all $ 2 \le m \le M $,  it follows  from the same argument as   {\bf Step 1} in the proof  of  \Cref{lemma:regression two change points} that 
 \begin{align*}\mathcal F(\I_m)  = & \sum_{i \in \I_m }(y_i - X_i^\top \widehat \beta _{\I_m}  ) ^2
  \le   \sum_{i \in \I_m }(y_i - X_i^\top   \beta ^*  _ i   ) ^2  + C_1 \bigg\{  \tr   \kappa ^2 +  \s\log(np)  \bigg\} \quad \text{for all } 2 
  \le m \le M.
 \end{align*}
 \
 \\
 {\bf Step 2.} It follows  from the same argument as   {\bf Step 2} in the proof  of  \Cref{lemma:regression two change points} that    
  \begin{align*}
  &\mathcal F(\I_1)  
  \le   \sum_{i \in \I_1 }(y_i - X_i^\top   \beta ^*  _ i   ) ^2  + C_1 \bigg\{  \tr   \kappa ^2 +  \s\log(np)  \bigg\} , \text{ and}
  \\
  &\mathcal F(\I_{M+1} )  
  \le   \sum_{i \in \I_{M+1} }(y_i - X_i^\top   \beta ^*  _ i   ) ^2  + C_1 \bigg\{  \tr   \kappa ^2 +  \s\log(np)  \bigg\}  
 \end{align*}
 \
 \\
 {\bf Step 3.} Since $\I \in \widehat{\mathcal P} $, we have
 \begin{align}\label{eq:regression three change points local min} \mathcal F(\I ) \le \sum_{m=1}^{M+1}\mathcal F(\I_m  )  +  M\gamma. 
 \end{align} The above display and the calculations in  {\bf Step 1} and  {\bf Step 2} implies that
\begin{align} 
 \sum_{i \in \I }(y_i -  X_i^\top \widehat \beta _\I ) ^2  
\le   \sum_{i \in \I  }(y_i -   X_i^\top \beta_i^*   ) ^2  
 +   (M +1) C_1 \bigg\{  \tr   \kappa ^2 +  \s\log(np) \bigg\}
+M\gamma  .
  \label{eq:regression three change points step 2 term 1}
\end{align}
Denote 
   $$  \J_1 =(s,  \eta_1], \ \J_m = (\eta_{m-1}, \eta_m]  \quad \text{for}\quad  2 \le m \le M , \ \J_{M+1}  =(\eta_M, e]. $$  
\Cref{eq:regression three change points step 2 term 1}  gives 
\begin{align} 
 \sum_{m=1}^{M+1}  \sum_{i \in \J_m   }(y_i - X_i^\top  \widehat \beta _\I ) ^2 
 \le& \sum_{m=1}^{M+1} \sum_{i \in \J_  m   }(y_i -  X_i^\top    \beta^*  _{\J_m  }  ) ^2    
 +  (M+1)   C_1 \bigg\{  \tr   \kappa ^2 +  \s\log(np) \bigg\} 
+M\gamma     \label{eq:regression three change points first}
\end{align}  
 \
 \\
 {\bf Step 4.} Using the same argument as in the {\bf Step 4} in the proof  of  \Cref{lemma:regression two change points},
it follows that 
\begin{align} \label{eq:regression three change point step 3 last term}\sum_{i \in \J_m   }(y_i - X_i^\top  \widehat \beta _\I ) ^2  - \sum_{i \in \J_m   }(y_i - X_i^\top    \beta^*  _{\J_m }  ) ^2 
\ge \frac{c_x|\J_m | }{64} \|\widehat \beta _\I  -  \beta^* _{\J_ m  } \|_2^2     -C_2 \s \log(np) \quad \text{for all}  \   2 \le m \le M. 
\end{align} 
 \
 \\
 {\bf Step 5.}
  Using the same argument as in the {\bf Step 4} in the proof  of  \Cref{lemma:regression two change points},  it follows that 
\begin{align} \label{eq:regression three change point step 5 first term}& \sum_{i \in \J_ 1 }(y_i - X_i^\top  \widehat \beta _\I ) ^2  - \sum_{i \in \J_ 1 }(y_i - X_i^\top    \beta^*  _{\J_1   }  ) ^2  \ge -C_3  ( \s\log(np)  +\gamma) \text{ 
 and }
\\\label{eq:regression three change point step 5 second term}
& \sum_{i \in \J_ {M+ 1} }(y_i - X_i^\top  \widehat \beta _\I ) ^2  - \sum_{i \in \J_  {M+ 1}  }(y_i - X_i^\top    \beta^*  _{\J_ {M+ 1}   }  ) ^2  \ge -C_3 ( \s\log(np)  +\gamma) 
 \end{align}
\
\\
{\bf  Step 6.} Putting \Cref{eq:regression three change points first}, \eqref{eq:regression three change point step 3 last term}, \eqref{eq:regression three change point step 5 first term} and  \eqref{eq:regression three change point step 5 second term}, 
 it follows that 
\begin{align} \label{eq:regression three change points step six} \sum_{ m  =2}^M \frac{c_x|\J_m  | }{64} \|\widehat \beta _\I  -  \beta^* _{\J_  m  } \|_2^2      \le C_4M (\s \log(np) + \tr \kappa ^2 + \gamma) .
\end{align} 
 For any $  m \in\{2, \ldots, M\}$, it holds that
\begin{align}  \label{eq:regression three change points signal lower bound} \inf_{  \beta  \in \mathbb R^p   }  |\J_{m-1} |  \|   \beta - \beta^* _{\J_ {m-1}   }  \|  ^2 + |\J_{m} | \|   \beta - \beta^* _{\J_ m  }  \|  ^2   =&     \frac{|\J_{m-1}| |\J_m|}{ |\J_{m-1}| +  |\J_m| } \kappa_m ^2  \ge \frac{1}{2} \Delta \kappa^2,
\end{align}  
where the last inequality follows from the assumptions that $\eta_k - \eta_{k-1}\ge \Delta  $ and $ \kappa_k \asymp \kappa$  for all $1\le k \le K$. So
\begin{align}   \nonumber &2 \sum_{ m=1}^{M }   |\J_m |\|\widehat \beta _\I  -  \beta^* _{\J_ m  } \|_2^2   
\\ 
\ge &  \nonumber    \sum_{m=2}^M  \bigg(  |\J_{m-1}  \|\widehat \beta _\I  -  \beta^* _{\J_ {m-1}   } \|_2^2      + |\J_m |\|\widehat \beta _\I  -  \beta^* _{\J_ m  } \|_2^2    \bigg) 
\\ \label{eq:regression three change points signal lower bound two} 
\ge & (M-1)  \frac{ 1}{2} \Delta \kappa^2  \ge \frac{M}{4} \Delta \kappa^2 ,
\end{align} 
where the second inequality follows from  \Cref{eq:regression three change points signal lower bound} and the last inequality follows from $M\ge 3$. \Cref{eq:regression three change points step six} and  \Cref{eq:regression three change points signal lower bound two} together imply that 
\begin{align}\label{eq:regression three change points signal lower bound three} 
 \frac{M}{4} \Delta \kappa^2 \le 2  C_5  M\bigg(  \s   \log(np ) +    \tr \kappa^2
+   \gamma \bigg) .
\end{align}
Since $\Bn\to \infty $, it follows that for sufficiently large $n$,   \Cref{eq:regression three change points signal lower bound three} gives 
$$ \Delta\kappa^2 \le C_5 \big(  \s \log(np) +\gamma),$$  
which contradicts \Cref{eq:regression three change points snr}. 
 
  
 \end{proof} 
 
 \bnlem Suppose $ \gamma \ge C_\gamma \s  \log(np) $ for sufficiently large constant $C_\gamma $. 
With probability  at least $1- n^{-3}$,    there is no  two consecutive intervals $\I_1= (s,t ] \in \widehat {\mathcal  P}  $,   $ \I_2=(t, e]  \in   \widehat  {\mathcal  P}  $    such that $\I_1 \cup \I_2$ contains no change points.  
 \enlem 
 \begin{proof} 
 For contradiction, suppose that 
 $$ \I :  =\I_1\cup  \I_2 $$
 contains no change points. 
For $\I_1$, note that if $|\I_1| \ge  C_\zeta \s \log(np) $, then 
 by \Cref{lam:regression one change deviation bound} {\bf a}, it follows that 
 \begin{align*} 
 \bigg|   \mathcal F(\I_1)   -  \sum_{i\in \I_1} (y_i - X_i^\top  \beta^*  _{i} )^2 \bigg|  = \bigg|   \sum_{i\in \I_1} (y_i - X_i^\top \widehat \beta _{\I_1} )^2- \sum_{i\in \I_1} (y_i - X_i^\top \beta_i^*   )^2    \bigg| \le  C_1 \s \log(np)  .
 \end{align*}
 If $|\I_1| <  C_\zeta \s \log(np)  $, then
\begin{align*} 
& \bigg|   \mathcal F(\I_1)   -  \sum_{i\in \I_1} (y_i - X_i^\top  \beta^*  _{i} )^2 \bigg|   =   \bigg|     \sum_{i\in \I_1} (y_i - X_i^\top  \beta^*  _{i} )^2  \bigg|  
=\sum_{i\in \I_1}   \epsilon_i^2 
 \\ 
 \le & |\I_1| E(\epsilon^2_1) + C_2 \sqrt {  |\I_1|  \log(n)  } + \log(n)  \le C_2' \s \log(np) .
 \end{align*} 
 So
 \begin{align*} 
 \bigg|   \mathcal F(\I_1)   -  \sum_{i\in \I_1} (y_i - X_i^\top  \beta^*  _{i} )^2 \bigg| \le   C_3   \s \log(np)  .
 \end{align*} 
 Similarly, 
\begin{align*} 
&\bigg|   \mathcal F(\I_2)   -  \sum_{i\in \I_2} (y_i - X_i^\top  \beta^*  _{i} )^2 \bigg| \le   C_3   \s \log(np), \quad \text{and}
\\
&\bigg|   \mathcal F(\I )   -  \sum_{i\in \I } (y_i - X_i^\top  \beta^*  _{i} )^2 \bigg| \le   C_3   \s \log(np)  .
 \end{align*} 
 So 
 $$\sum_{i\in \I_1} (y_i - X_i^\top \beta_i^*   )^2  +\sum_{i\in \I_2} (y_i - X_i^\top \beta_i^*    )^2 -2C_1  \s \log(np ) +\gamma    \le \sum_{i\in \I } (y_i - X_i^\top \beta_i^*   )^2 +C_1 \s  \log(np) .  $$
 Since $\beta^* _i$ is unchanged when $i\in \I$, it follows that 
 $$ \gamma \le 3C_1 \s \log(np).$$
 This is a contradiction when $C_\gamma> 3C_1. $
 \end{proof} 
  
  
  
%  \subsection{Proofs related to \Cref{prop:change points partition size consistency}}
%  Throughout this section, for any generic interval $\I \subset (0,n]$, denote  
%  $$ \mathcal F^*(\I) = \sum_{i \in \I } (y_i -X_i^\top \beta_i^* )^2.   $$
%  
%\bnlem
%
%Let $\I \subset \J$ be any two intervals such that $\I  $ contains no true change points. Then with probability at least $1-n^{-5} $,  it holds that
%$$\mathcal  F^*(\I ) - \mathcal F(\J) \le C\s \log(np).  $$ 
%\enlem  
%  \begin{proof}
%  If $\J \le C_\gamma \s \log(np)   $, then $\I \le \J \le C_\gamma \s \log(np)    $. As a result.
%  \begin{align*} 
%  \mathcal  F^*(\I )- \mathcal F(\J) = \sum_{i \in \I } (y_i -X_i^\top \beta_i^* )^2  = \sum_{i \in \I } \epsilon_i^2 \le C_1 \bigg\{\sqrt {|\I|  \log(n) } + \log(n) \bigg\}  \le C_2 \s\log(np). 
%  \end{align*}
%  \end{proof}
  
%
% 
%\begin{proof}[Proof of   \Cref{prop:change points partition size consistency}] 
%Denote $\mathfrak{G} ^*_n = \sum_{ i =1}^n (y_i  -  u_i)^2$.  Given any collection $\{t_1, \ldots, t_m\}$, where $t_1 < \cdots < t_m$, and $t_0 = 0$, $t_{m+1} = n$, let 
%	\begin{equation}\label{eq-sn-def}
%		\G _n(t_1, \ldots, t_{m}) = \sum_{k=1}^{m} \sum_{ i = t_k +1}^{t_{k+1}} \big( y_ i  -   \widehat y _  {(t_{k}, t_{k+1}]} \big )^2. 
%	\end{equation}
%	For any collection of time points, when defining \eqref{eq-sn-def}, the time points are sorted in an increasing order.
%	\
%	\\
%	\\
%Let $\{ \widehat \eta_{k}\}_{k=1}^{\widehat K}$ denote the change points induced by $\widehat {\mathcal P}$.  Suppose we can justify that 
%	\begin{align}
%		\G^*_n + K\gamma  \ge  &\G _n(\eta_1,\ldots,\eta_K)   + K\gamma - C_1 ( K +1)  \log(n)  \label{eq:K consistency step 1} \\ 
%		\ge & \G_n (\widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } ) +\widehat K \gamma - C_1  ( K +1)   \log(n)  \label{eq:K consistency step 2} \\ 
%		\ge &  \G _n ( \widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K ) + \widehat K \gamma    - C_1(K+1)  \log(n)  \label{eq:K consistency step 3}
%	\end{align}
%	and that 
%	\begin{align}\label{eq:K consistency step 4}
%		\G ^*_n   -\G _n ( \widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K ) \le C_2 (K + \widehat{K} + 2) \log(n) .
%	\end{align}
%	Then it must hold that $| \hatp | = K$, as otherwise if $\widehat K \ge K+1 $, then  
%	\begin{align*}
%		C _2 (K + \widehat{K} + 2)  \log(n)  & \ge   \G ^*_n  -\G _n ( \widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K ) \\
%		& \ge      (\widehat K - K)\gamma  -C_1 (K+1) \log(n) .
%	\end{align*} 
%	Therefore due to the assumption that $| \hatp|  =\widehat K\le 3K $, it holds that 
%	\begin{align} \label{eq:Khat=K} 
%		C_1 (5K + 2) \log(n)  + C_1(K+1) \log(n)  \ge  (\widehat K - K)\gamma \geq \gamma,
%	\end{align}
%	Note that \eqref{eq:Khat=K} contradicts the choice of $\gamma$.
%
%
%\
%\\
%{\bf Step 1.} Note that \eqref{eq:K consistency step 1}  is implied by 
%	\begin{align}\label{eq:step 1 K consistency}  
%		\left| 	\G ^*_n   -   \G_n(\eta_1,\ldots,\eta_K)    \right| \le  C_3(K+1) \s \lambda^2,
%	\end{align}
%	which is  an  immediate consequence  of \Cref{lem:mean one change deviation bound}. 
%	\
%	\\
%	\\
%	{\bf Step 2.} Since $\{ \widehat \eta_{k}\}_{k=1}^{\widehat K}$ are the change points induced by $\widehat {\mathcal P}$, \eqref{eq:K consistency step 2} holds because $\hatp$ is a minimizer.
%\\
%\\
%	{\bf Step 3.}
%For every $ \I  =(s,e]\in \hatp$ denote
%	\[
%		 \I =  (s ,\eta_{p+1}]\cup \ldots \cup  (\eta_{p+q} ,e]  = \J_1 \cup \ldots  \cup \J_{M+1},
%	\]
%	where $\{ \eta_{p+ m }\}_{ m =1}^{ M +1}  =\I \, \cap \, \{\eta_k\}_{k=1}^K$. 
%\
%\\
%\\
%For each $ m\in \{1, \ldots, M+1\}$,
%	since 
%	$$ \widehat y_{\J_m}  = \argmin_{a \in \mathbb R}   \sum_{ i \in \J_m }(y_ i - a    )^2 , $$
%it follows that $$
%		\sum_{ i \in \J_m }(y_ i - \widehat y _\I    )^2   \ge \sum_{ i \in \J_ m } (y_ i  - \widehat y_{\J_m}   )^2 . 
%$$ 
% Therefore the above inequality implies that 
%	\begin{align} \label{eq:K consistency step 3 inequality 3}  \sum_{i \in \I }  (y_ i - \widehat y _\I    )^2   \ge \sum_{m=1}^{M+1 } \sum_{ i \in \J_m }(y_ i - \widehat y _\I    )^2   \ge\sum_{m=1}^{M+1 }   \sum_{ i \in \J_m} (y_ i  - \widehat y_{\J_m}   )^2 .  
%	\end{align}
%		Note that   \eqref{eq:K consistency step 3} is an immediate consequence of   \eqref{eq:K consistency step 3 inequality 3}.
%\\
%\\
%	{\bf Step 4.}
%Finally, to show \eqref{eq:K consistency step 4},   let  $\widetilde { \mathcal P}$ denote    the partition induced by $\{\widehat \eta_{1},\ldots, \widehat \eta_{\widehat K } , \eta_1,\ldots,\eta_K\}$. Then 
%$| \widetilde { \mathcal P} | \le K + \widehat K+2   $ and that $u_i$ is unchanged in every interval $\I \in \widetilde { \mathcal P}$. 
%	So  \Cref{eq:K consistency step 4} is an immediate consequence of   \Cref{lem:mean one change deviation bound}.
%\end{proof} 
   
 

\subsection{Additional Results Related to Lasso}

\bnlem \label{lam:regression one change deviation bound}
Let $\mathcal I =(s,e] $ be any generic interval.  
\\
{\bf a.} If $\I$ contains no change points and that 
$|\I| \ge C_s \s \log(np) $ where $C_s$ is the universal constant in \Cref{lemma:interval lasso}. Then it holds that 
$$\p \bigg( \bigg|   \sum_{ i  \in \I } (y_i   - X_i ^\top \widehat  \beta _\I   )^2  - \sum_{ i   \in \I } (y_i      -  X_i^\top \beta^*_\I    )^2  \bigg|  \ge C    \s  \log(np)  \bigg)  \le  n^{-4}. $$
\
\\
{\bf b.}  Suppose that   the   interval $ \I=(s,e]$ contains one  and only change point $ \eta_k $ and that 
$|\I| \ge C_s \s \log(np) $. Denote  $\widehat \mu_\I = \frac{1}{|\I | } \sum_{i\in \I } y_i $ and 
$$  \mathcal J = (s,\eta_k] \quad \text{and} \quad  \mathcal J' =  (\eta_k, e]  .$$   Then it holds that 
$$\p \bigg( \bigg|   \sum_{ i  \in \I } (y_i   - X_i^\top \widehat \beta_\I   )^2  - \sum_{ i   \in \I } (y_i      - X_i^\top \beta^* _i    )^2  \bigg|  \ge  C\bigg\{   \frac{ | \J||\J'| }{ |\I| }  \kappa_k ^2  +  \s \log(np)\bigg\}   \bigg)   \le  n^{-4}. $$
\enlem
\begin{proof} 
We show {\bf b} as {\bf a} immediatelly follows from {\bf b} with $ |\J'| =0$.
 Denote 
$$  \mathcal J = (s,\eta_k] \quad \text{and} \quad  \mathcal J' =  (\eta_k, e]  .$$ 
Denote  $  \beta _\I^*  = \frac{1}{|\I | } \sum_{i\in \I } \beta ^* _i $. Note that 
\begin{align}  \nonumber 
   \bigg|  \sum_{ i  \in \I } (y_i   - X_i^\top \widehat \beta_\I   )^2  - \sum_{ i   \in \I } (y_i      - X_i^\top \beta^* _i    )^2  \bigg|   
 = &\bigg| \sum_{i\in \I } \big\{  X_i^\top  ( \widehat \beta_\I  -   \beta^* _i )   \big\} ^2 -  2 \sum_{i\in \I }  \epsilon_i X_i^\top ( \widehat \beta_\I   -  \beta^*_i ) \bigg| 
 \\ \label{eq:regression one change point deviation bound term 1}
 \le & 2 \sum_{i\in \I } \big\{  X_i^\top  ( \widehat \beta_\I  -    \beta^*_\I  )   \big\}   ^2 
 \\ \label{eq:regression one change point deviation bound term 2}
 + & 2 \sum_{i\in \I } \big\{  X_i^\top  (    \beta^*_\I  -\beta^*_i  )    \big\} ^2  
 \\ \label{eq:regression one change point deviation bound term 3}
 +& 2 \bigg|    \sum_{i\in \I }  \epsilon_i X_i^\top ( \widehat \beta_\I   -  \beta^*_\I ) \bigg|  
 \\ \label{eq:regression one change point deviation bound term 4}
 +&  2 \bigg|    \sum_{i\in \I }  \epsilon_i X_i^\top (   \beta^*_\I -\beta^*_i  ) \bigg|  .
\end{align}
\
\\
Suppose all the good events in \Cref{lemma:interval lasso} holds. 
\\
\\
{\bf Step 1.} By \Cref{lemma:interval lasso},   $\widehat \beta_\I  -    \beta^*_\I  $ satisfies the cone condition that 
$$ \| (\widehat \beta_\I  -    \beta^*_\I  )_{S^c}\|_1 \le 3 \| (\widehat \beta_\I  -    \beta^*_\I )_S  \|_1   .$$
It follows from \Cref{corollary:restricted eigenvalues 2} that with probability at least $ 1-n^{-5}$,
\begin{align*} 
 \bigg| \frac{1}{|\I| } \sum_{i\in \I } \big\{  X_i^\top  ( \widehat \beta_\I  -    \beta^*_\I  )   \big\} ^2    - ( \widehat \beta_\I  -    \beta^*_\I    )^\top \Sigma  ( \widehat \beta_\I  -    \beta^*_\I  )  \bigg|  \le C_1  \sqrt { \frac{\s \log(np) }{|\I| }} \| \widehat \beta_\I  -    \beta^*_\I     \|_2 ^2  .
\end{align*}
The above display   gives
\begin{align*}    \bigg| \frac{1}{|\I| } \sum_{i\in \I } \big\{  X_i^\top  ( \widehat \beta_\I  -    \beta^*_\I  )    \big\}^2 \bigg| \le &  \| \Sigma\|_{\op}   \| \widehat \beta_\I  -    \beta^*_\I     \|_2 ^2   + C_1  \sqrt { \frac{\s \log(np) }{|\I| }} \| \widehat \beta_\I  -    \beta^*_\I     \|_2 ^2 
\\
\le & C_x \| \widehat \beta_\I  -    \beta^*_\I     \|_2 ^2 + C_1  \sqrt { \frac{\s \log(np) }{C_\zeta \s \log(np)  }} \| \widehat \beta_\I  -    \beta^*_\I     \|_2 ^2   
\\
\le &  \frac{ C_2\s\log(np)}{|\I| }   \end{align*} 
where the second inequality follows from the assumption that  $|\I| \ge C_\zeta \s \log(np) $ and the last inequality follows from  \Cref{eq:lemma:interval lasso term 1}  in \Cref{lemma:interval lasso}.
This gives 
$$    \bigg|   \sum_{i\in \I } \big\{  X_i^\top  ( \widehat \beta_\I  -    \beta^*_\I  )    \big\}^2 \bigg| \le  2 C_2\s\log(np) . $$
\
\\
{\bf Step 2.}  Observe that 
$ X_i^\top (\beta_\I ^* - \beta^*_i) $ is Gaussian with mean $0$ and variance 
\begin{align*} \omega_i ^2 = (\beta_\I ^* - \beta^*_i )^\top \Sigma  (\beta_\I ^* - \beta^*_i)  . 
\end{align*}
Since 
$$ \beta_\I ^* = \frac{|\J| \beta^*_\J +|\J'| \beta^*_{\J'}   }{|\I | },$$
it follows that 
$$ \omega_i ^2 = \begin{cases} 
\bigg(  \frac{ | \J'| (\beta^*_\J -\beta^*_{\J'}   ) }{ | \I| }  \bigg)^\top  \Sigma \bigg(  \frac{ | \J'| (\beta^*_\J -\beta^*_{\J'}   ) }{ | \I| }  \bigg)   \le   \frac{| \J'| ^2  \kappa_k^2 }{ |\I|^2 }   &\text{when }  i \in \J ,
\\
\bigg(  \frac{ | \J| (\beta^*_{\J'} -\beta^*_\J    ) }{ | \I| }  \bigg) ^\top  \Sigma \bigg(  \frac{ | \J'| (  \beta^*_{\J'}  -\beta^*_\J   ) }{ | \I| }  \bigg)   \le   \frac{| \J| ^2  \kappa_k^2 }{ |\I|^2 }   &\text{when }  i \in \J'.
\end{cases} $$
 Consequently,
$   \{ X_i^\top (\beta_\I ^* - \beta^*_i)\} ^2 $ is sub-Exponential with parameter $  \omega_i ^2$.  
By standard sub-Exponential tail bounds, it follows that 
\begin{align*}
 &\p \bigg(  \bigg|   \sum_{ i \in \I }\{ X_i^\top (\beta_\I ^* - \beta^*_i)\} ^2 -\E{\sum_{ i \in \I }\{ X_i^\top (\beta_\I ^* - \beta^*_i)\} ^2}    \bigg| \ge C_3 \tau    \bigg)  
 \\
 \le &  \exp\bigg (-c \min\bigg \{ \frac{  \tau^2}{\sum_{i\in \I } \omega_i ^4  }  ,  \frac{ \tau }{ \max_{i\in \I }   \omega_i ^2 } \bigg\}  \bigg)
 \\
 \le &  \exp\bigg (-c' \min\bigg \{ \frac{  \tau^2}{\sum_{i\in \I } \omega_i ^2  }  ,  \frac{ \tau }{ \max_{i\in \I }   |\omega_i | } \bigg\}  \bigg)
 \\
 \le & \exp\bigg (-c ''\min\bigg \{  \tau^2  \bigg( \frac{|\I |   }{| \J'| |\J|  } \kappa_k^{-2}  \bigg)    ,    \tau   \frac{|\I| }{ \max \{|\J|, |\J'|  \}}   \kappa_k ^{-1} \bigg\}  \bigg) ,
 \end{align*}
where the second inequality follows from the observation that 
$$  \omega_i^2     \le \kappa_k |\omega_i| \le  C_\kappa  |\omega_i| \text{ for all } i \in \I , $$
 and the last inequality follows from the observation that 
\begin{align*}
 \sum_{i\in \I} \omega_i ^2    
 \le  C_x | \J| \frac{| \J'| ^2  \kappa_k^2 }{ |\I|^2 } + C_x | \J ' | \frac{| \J| ^2  \kappa_k^2 }{ |\I|^2 }  
=   C_x \frac{| \J'| |\J| }{|\I | } \kappa_k^2 .
 \end{align*} 
 So there exists a sufficiently large constant $C_4$ such that with probability at  least $1- n^{-5}$, 
\begin{align*}
 &  \bigg|   \sum_{ i \in \I }\{ X_i^\top (\beta_\I ^* - \beta^*_i)\} ^2 -\E{\sum_{ i \in \I }\{ X_i^\top (\beta_\I ^* - \beta^*_i)\} ^2}    \bigg|
  \\ 
   \le &  C_ 4   \bigg\{\sqrt { \frac{| \J'| |\J| }{|\I | }  \log(n)  \kappa _k ^2  } + \log(n)    \frac{\max \{|\J|, |\J'|  \}  }{|\I| } \kappa _k  \bigg\}     
 \\
 \le &  C_ 4'  \bigg\{      \frac{| \J'| |\J| }{|\I | }  \kappa_k^2  + \log(n)   +  \log(n)    \frac{\max \{|\J|, |\J'|  \}  }{|\I| } \kappa _k  \bigg\}      
 \\
 \le &C_5  \bigg\{      \frac{| \J'| |\J| }{|\I | }  \kappa_k^2  + \log(n)     \bigg\}      
 \end{align*}
 where $ \kappa_k \asymp \kappa \le C_\kappa $ is used in the last inequality.
Since $ \E{\sum_{ i \in \I }\{ X_i^\top (\beta_\I ^* - \beta^*_i)\} ^2} = \sum_{i\in \I }\omega_i ^2 \le C_x \frac{| \J'| |\J| }{|\I | } \kappa_k^2$, it follows that 
$$ \p \bigg (  \bigg|   \sum_{ i \in \I }\{ X_i^\top (\beta_\I ^* - \beta^*_i)\} ^2    \bigg|  \le ( C_5 +C_x )  \frac{| \J'| |\J| }{|\I | }  \kappa_k^2  + C_5 \log(n) \bigg ) \ge 1-n^{-5}.$$
\
\\
{\bf Step 3.} For \Cref{eq:regression one change point deviation bound term 3},  it follows that with probability at least $1-2n^{-4}$
\begin{align*} 
   \frac{1}{|\I| } \sum_{i\in \I }  \epsilon_i X_i^\top ( \widehat \beta_\I   -  \beta^*_\I )
  \le  C_6 \sqrt { \frac{\log(np) }{ |\I| } } \|  \widehat \beta_\I   -  \beta^*_\I \|_1 \le C_7  \frac{\s \log(np) }{ |\I| } 
\end{align*}
where the first inequality is a consequence of \Cref{eq:independent condition 1c 1}, the second inequality follows from  \Cref{eq:lemma:interval lasso term 3} in \Cref{lemma:interval lasso}. 
\
\\
\\
{\bf Step 4.}  From {\bf Step 2}, we have  that
$ X_i^\top (\beta_\I ^* - \beta^*_i) $ is Gaussian with mean $0$ and variance 
$$ \omega_i ^2 = \begin{cases} 
\bigg(  \frac{ | \J'| (\beta^*_\J -\beta^*_{\J'}   ) }{ | \I| }  \bigg)^\top  \Sigma \bigg(  \frac{ | \J'| (\beta^*_\J -\beta^*_{\J'}   ) }{ | \I| }  \bigg)   \le   \frac{| \J'| ^2  \kappa_k^2 }{ |\I|^2 }   &\text{when }  i \in \J ,
\\
\bigg(  \frac{ | \J| (\beta^*_{\J'} -\beta^*_\J    ) }{ | \I| }  \bigg) ^\top  \Sigma \bigg(  \frac{ | \J'| (  \beta^*_{\J'}  -\beta^*_\J   ) }{ | \I| }  \bigg)   \le   \frac{| \J| ^2  \kappa_k^2 }{ |\I|^2 }   &\text{when }  i \in \J'.
\end{cases} $$
 Consequently,
$   \epsilon_i  X_i^\top (\beta_\I ^* - \beta^*_i)  $ is   centered  sub-Exponential with parameter $  \omega_i \sigma_\epsilon  $.  
By standard sub-Exponential tail bounds, it follows that 
\begin{align*}
 &\p \bigg(  \bigg|   \sum_{ i \in \I } \epsilon_i  X_i^\top (\beta_\I ^* - \beta^*_i)       \bigg| \ge C_8 \tau    \bigg)  
 \\
 \le &  \exp\bigg (-c \min\bigg \{ \frac{  \tau^2}{\sum_{i\in \I } \omega_i ^2  }  ,  \frac{ \tau }{ \max_{i\in \I }  |\omega_i| } \bigg\}  \bigg)
 \\
 \le & \exp\bigg (-c '\min\bigg \{  \tau^2  \bigg( \frac{|\I |   }{| \J'| |\J|  } \kappa_k^{-2}  \bigg)    ,    \tau   \frac{|\I| }{ \max \{|\J|, |\J'|  \}}   \kappa_k ^{-1} \bigg\}  \bigg) ,
 \end{align*}
where the last inequality follows from the observation that 
\begin{align*}
 \sum_{i\in \I} \omega_i ^2    
 \le  C_x | \J| \frac{| \J'| ^2  \kappa_k^2 }{ |\I|^2 } + C_x | \J ' | \frac{| \J| ^2  \kappa_k^2 }{ |\I|^2 }  
=   C_x \frac{| \J'| |\J| }{|\I | } \kappa_k^2 .
 \end{align*} 
 So there exists a sufficiently large constant $C_9$ such that with probability at  least $1- n^{-5}$, 
\begin{align*}
 &  \bigg|   \sum_{ i \in \I } \epsilon_i X_i^\top (\beta_\I ^* - \beta^*_i) \bigg|
  \\ 
   \le &  C_ 9   \bigg\{\sqrt { \frac{| \J'| |\J| }{|\I | }  \log(n)  \kappa _k ^2  } + \log(n)    \frac{\max \{|\J|, |\J'|  \}  }{|\I| } \kappa _k  \bigg\}     
 \\
 \le &  C_ 9'  \bigg\{      \frac{| \J'| |\J| }{|\I | }  \kappa_k^2  + \log(n)   +  \log(n)    \frac{\max \{|\J|, |\J'|  \}  }{|\I| } \kappa _k  \bigg\}      
 \\
 \le &C_9  \bigg\{      \frac{| \J'| |\J| }{|\I | }  \kappa_k^2  + \log(n)     \bigg\}      
 \end{align*}
 where $ \kappa_k \asymp \kappa \le C_\kappa $ is used in the last inequality.
\end{proof} 

 
\bnlem \label{lemma:interval lasso} Suppose  \Cref{assp:dcdp_linear_reg} holds. Let $$ \widehat \beta _{ \mathcal I } = \arg\min_{\beta \in \mathbb R^p }  \frac{1}{ |\mathcal I |  }\sum_{i \in \mathcal I}   (y_i -X_i^\top \beta) ^2 + \lambda \|\beta\|_1$$ with $\lambda = C_\lambda (\sigma_{\epsilon} \vee 1)\sqrt { \log(np) }$ for some sufficiently large constant $C _ \lambda $. There exists a sufficiently large constant $ C_s$ such that for all   $ \mathcal I  \subset (0, n] $   such that $| \mathcal I | \ge C_s\s \log(np)$, it holds with probability at least $ 1-(np)^{-3}$ that 
% \begin{align} \label{eq:lemma:interval lasso term 1}
% &\|\widehat{\beta}_{\mathcal{I}}-\beta_{\mathcal{I}}\|_{2}^{2} \leq \frac{C \sigma_{\epsilon}^2\s \log (np)}{|\I|} \\
% &\|\widehat{\beta}_{\mathcal{I}}-\beta_{\mathcal{I}}\|_{1} \leq C \sigma_{\epsilon}\s \sqrt{\frac{\log (np)}{|\I|}} \\
% &\|(\widehat{\beta}_{\mathcal{I}}-\beta_{\mathcal{I}})_{S^{c}}\|_{1} \leq 3\|(\widehat{\beta}-\beta^{*})_{S}\|_{1},
% \end{align}
\begin{align} \label{eq:lemma:interval lasso term 1}
&   \| \widehat \beta_\I -\beta^*_\I \| _2^2 \le \frac{C (\sigma_{\epsilon}^2\vee 1)\s\log(np)}{ |\I  |  } ;
 \\ \label{eq:lemma:interval lasso term 2}
 &     \| \widehat \beta_\I  -\beta^*_\I \| _1  \le     C(\sigma_{\epsilon}\vee 1) \s\sqrt {  \frac{\log(np)} {|\I  |  } }  ;
 \\ \label{eq:lemma:interval lasso term 3}
 &    \| (\widehat \beta_\I -\beta^*_\I)_{S^c} \| _1 \le  3 \| (\widehat \beta _\I  -\beta^*_\I )_{S } \| _1   .
\end{align} 
where $ \beta^*_\I  = \frac{1}{|\I|} \sum_{i\in \I } \beta^*_i $.
 \enlem 
\begin{proof}  Denote $S=\bigcup_{k=1}^K S_{\eta_k+1} $. Since $K< \infty$, 
$|S| \asymp \s.$ 
  It follows from the definition of $\widehat{\beta}_\I$ that 
	\[
	 \frac{1}{|\I | }	\sum_{ i \in I} (y_i - X_i^{\top}\widehat{\beta}_\I )^2 + \frac{ \lambda}{ \sqrt{  |\I|  }}    \|\widehat{\beta} _\I\|_1 \leq  
	 \frac{1}{|\I | } \sum_{t \in \I} (y_i - X_i^{\top}\beta^*_\I )^2 + \frac{ \lambda}{ \sqrt{  |\I|  }}  \|\beta^*_\I  \|_1.
	\]
	This gives 
	\begin{align*}
		 \frac{1}{|\I | } \sum_{i \in \I} \bigl\{X_i ^{\top}(\widehat{\beta}_\I - \beta^*_\I )\bigr\}^2 +    \frac{ 2 }{|\I | }   \sum_{ i \in \I}(y_i - X_i^{\top}\beta^*_\I)X_i^{\top}(\beta^*_\I  - \widehat{\beta}_\I )  +  \frac{ \lambda}{ \sqrt{  |\I|  }}   \bigl\|\widehat{\beta}_\I \bigr\|_1 
		\leq  \frac{ \lambda}{ \sqrt{  |\I|  }}    \bigl\|\beta^*_\I \bigr\|_1,
	\end{align*}
	and therefore
	\begin{align}
		& \frac{1}{|\I | }	  \sum_{i  \in \I} \bigl\{X_i ^{\top}(\widehat{\beta} _\I  - \beta^*_\I )\bigr\}^2 + \frac{ \lambda}{ \sqrt{  |\I|  }} \bigl\|\widehat{\beta}_\I \bigr\|_1  \nonumber \\
		 \leq  &  \frac{ 2}{|\I | }	 \sum_{i \in  \I } \epsilon_i  X_i ^{\top}(\widehat{\beta}_\I  - \beta^*_\I ) 
+ 2   (\widehat{\beta}_\I  - \beta^*_\I )^{\top}\frac{  1 }{|\I | }	 \sum_{i\in   \I} X_ i  X_i^{\top}(    \beta^*_i -\beta^*_\I   )		 
		+  \frac{ \lambda}{ \sqrt{  |\I|  }}    \bigl\|\beta^*_\I \bigr\|_1   .	 \label{eq-lem10-pf-2}
	\end{align}
To bound	
		$\left\|\sum_{ i  \in \I} X_ i  X_i ^\top (\beta^*  _\I  -\beta^*_i ) \right\|_{\infty},  
$
	note  that  for any $j \in  \{ 1, \ldots, p\}$, the $j$-th entry of 
	\\$\sum_{i \in \I} X _ i X _i^\top (\beta^*_\I   -\beta_i )$ satisfies  
	\begin{align*}
		  E \left\{\sum_{ i  \in \I}   X_i (j) X _ i ^\top (\beta^*_\I   - \beta^*_ i  )\right\} = \sum_{ i \in \I}  E \{X _ i (j  ) X_i ^\top \}\{\beta^*_\I  - \beta^*_ i \}  
		=     \mathbb{E}\{X _1( j ) X _1 ^\top \} \sum_{ i \in \I}\{\beta^*_\I    - \beta^*_ i  \} = 0.
	\end{align*}
	So   $  E\{ \sum_{ i  \in \I} X_ i  X_i ^\top (\beta^*  _\I  -\beta^*_i )\} =0 \in \mathbb R^p.$ 
By \Cref{lemma:consistency}{\bf b},
	\begin{align*}
	  \bigg|  (    \beta^*_i -\beta^*_\I   ) ^\top  \frac{  1 }{|\I | }	 \sum_{i\in   \I} X_t X_t^{\top} (\widehat{\beta}_\I  - \beta^*_\I )	 	   \bigg| \le & C_1 \big(\max_{1\le i \le n }  \|\beta^*_i -\beta^*_\I \|_2 \big) \sqrt { \frac{\log(np) }{ | \I|  }} \| \widehat{\beta}_\I  - \beta^*_\I  \|_1   
	  \\
	  \le & C_2 \sqrt { \frac{\log(np) }{ | \I| }} \| \widehat{\beta}_\I  - \beta^*_\I  \|_1  
	  \\
	  \le &  \frac{\lambda}{8\sqrt { |\I| } }   \|\widehat{\beta}_\I  - \beta^*_\I \|_1 
 	\end{align*}
 	where the second inequality follows from \Cref{lemma:beta bounded 1} and the last inequality follows from $\lambda = C_\lambda\sigma_{\epsilon} \sqrt { \log(np) }$ with sufficiently large constant $C_\lambda$.
	In addition  by \Cref{lemma:consistency}{\bf a},
	\begin{equation*}
	    \frac{ 2}{|\I | }	 \sum_{i \in  \I } \epsilon_i  X_i ^{\top}(\widehat{\beta}_\I  - \beta^*_\I )  \le C  \sigma_{\epsilon}\sqrt { \frac{ \log(np) }{ |\I| } }\|\widehat{\beta}_\I  - \beta^*_\I \|_1  \le  \frac{\lambda}{8\sqrt { |\I| } }   \|\widehat{\beta}_\I  - \beta^*_\I \|_1 .
	\end{equation*}
	So   \eqref{eq-lem10-pf-2}  gives 
	\begin{align*}
		  \frac{1}{|\I | }	  \sum_{i  \in \I} \bigl\{X_i ^{\top}(\widehat{\beta} _\I  - \beta^*_\I )\bigr\}^2 + \frac{ \lambda}{ \sqrt{  |\I|  }} \bigl\|\widehat{\beta}_\I \bigr\|_1  
		 \leq  \frac{\lambda}{4\sqrt { |\I| } }   \|\widehat{\beta}_\I  - \beta^*_\I \|_1  
		+  \frac{ \lambda}{ \sqrt{  |\I|  }}    \bigl\|\beta^*_\I \bigr\|_1   .	 
	\end{align*} 
Let $\Theta = \widehat  \beta _\I   - \beta^*_\I   $. The above inequality implies
\begin{align}
\label{eq:two sample lasso deviation 1} \frac{1}{|\I|} \sum_{i \in \I } \left( X_i^\top  \Theta \right)^2 + \frac{ \lambda}{2\sqrt{  |\I|  } }\|  (\widehat \beta _\I)   _{ S ^c}\|_1  
 \le & \frac{3\lambda}{2\sqrt{  |\I|  }  } \| ( \widehat  \beta _\I  -  \beta^*_\I  )    _{S} \| _1  ,
 \end{align}  
which also implies that 
$$ \frac{\lambda }{2}\| \Theta _{S^c}  \|_1 = \frac{ \lambda}{2 }\|   (\widehat \beta_\I)  _{ S ^c}\|_1    \le  
\frac{3\lambda}{2 } \|  ( \widehat  \beta _\I   - \beta^* _\I  ) _{S} \| _1  = \frac{3\lambda}{2 } \|  \Theta  _{S} \| _1 . $$
The above inequality and  \Cref{corollary:restricted eigenvalues 2} imply that with probability at least $1-n^{-5}$,
$$ \frac{1}{|\I| } \sum_{i \in \I }  \left( X_i^\top  \Theta \right)^2  = \Theta^\top \widehat \Sigma _\I  \Theta  
\ge 
 \Theta^\top \Sigma \Theta - C_3\sqrt{ \frac{ \s\log(np)}{ |\I| }}  \| \Theta\|_2^2   \ge  \frac{c_x}{2} \|\Theta\|_2 ^2   ,$$
 where the last inequality follows from the assumption that $| \mathcal I | \ge C_s \s \log(np)   $ for sufficiently large $C_s$.
Therefore \Cref{eq:two sample lasso deviation 1} gives
\begin{align}
\label{eq:two sample lasso deviation 2}  c'\|\Theta\|_2 ^2  + \frac{ \lambda}{2\sqrt{  |\I|  }  }\| ( \widehat \beta_\I  - \beta^*_\I ) _{ S ^c}\|_1  
 \le   \frac{3\lambda}{2\sqrt{  |\I|  }  } \| \Theta_{S} \| _1  \le \frac{3\lambda \sqrt \s }{2 \sqrt{  |\I|  } } \| \Theta  \| _2 
 \end{align}  
 and so 
 $$ \|\Theta\|_2  \le   \frac{C \lambda \sqrt  \s}{\sqrt{| \I |} } . $$ 
 The above display   gives  
 $$  \| \Theta_{S} \| _1 \le  \sqrt {\s}  \| \Theta_{S} \| _2 \le   \frac{C\lambda \s}{\sqrt{|\I| }}. $$ 
 Since 
  $ \| \Theta_{S^c } \| _1 \le 3 \| \Theta_{S} \| _1 ,$ 
it also holds that 
$$\| \Theta  \| _1 = \| \Theta_{S  } \| _1 +\| \Theta_{S^c } \| _1  \le 4 \| \Theta_{S} \| _1 \le  \frac{4C\lambda \s}{\sqrt{|\I|} } .$$
 \end{proof}

 
 

 
 
\subsection{Additional Technical Results} 
\bnlem
\label{theorem:restricted eigenvalues 2}
Suppose  $\{X_{i } \}_{1\le i \le n } \overset{i.i.d.} {\sim}  N_p (0, \Sigma )  $. 
Denote $\mathcal C_S  := \{ v : \mathbb R^p : \| v_{S^c }\|_1 \le 3\| v_{S}\|_1 \}  $, where $ |S| \le \s $.
Then there exists constants $c$ and $C$ such that for all $\eta\le 1$, 
\begin{align} 
P \left( \sup_{v \in \mathcal C _S , \|v\|_2=1   } \left | v^\top ( \widehat \Sigma -\Sigma )  v \right| \ge C\eta   \Lambda_{\max} (\Sigma)   \right)
\le 2\exp( -c n\eta ^2 + 2\s \log(p) ) .
\end{align}
\enlem
\begin{proof}
This is a well known restricted eigenvalue property for Gaussian design. The proof can be found  in \cite{Basu2015} or \cite{Loh2012}.
\end{proof}  

\bnlem
\label{corollary:restricted eigenvalues 2} Suppose  $\{X_{i } \}_{1\le i \le n } \overset{i.i.d.} {\sim}  N_p (0, \Sigma )  $. 
 Denote $\mathcal C_S  := \{ v : \mathbb R^p : \| v_{S^c }\|_1 \le 3\| v_{S}\|_1 \}  $, where $ |S| \le \s $.  With probability at least $1- n ^{-5}$, it holds that
$$  \left | v^\top ( \widehat \Sigma_\I  -\Sigma )  v \right| \le C \sqrt { \frac{\s\log(np) }{|\I| } }     \|v\|_2^2   
 $$
   for all $v \in \mathcal C _S $ and all $\I \subset  (0, n]$ such that $| \I |\ge C_s \s\log(np)  $, where $ C_s$
is the constant in \Cref{lemma:consistency} which is independent of $n, p$.   
\enlem
\begin{proof} 
For any $\I \subset  (0, n]$ such that $| \I |\ge C_s\s \log(np)   $, by \Cref{theorem:restricted eigenvalues 2}, it holds that 
\begin{align*} 
P \left( \sup_{v \in \mathcal C _S , \|v\|_2=1   } \left | v^\top ( \widehat \Sigma _\I -\Sigma )  v \right| \ge C\eta   \Lambda_{\max} (\Sigma)   \right)
\le 2\exp( -c   |\I| \eta ^2 + 2\s \log(p) ) .
\end{align*}
Let  $\eta= C_1 \sqrt { \frac{\s\log(np) }{|\I | } } $ for sufficiently large constant $C_1$. Note that $\eta< 1$ if $ |\I| > C_1^2 \s\log(np) $. Then   with probability at least 
$(np)^{-7} $, 
$$\sup_{v \in \mathcal C _S , \|v\|_2=1   } \left | v^\top ( \widehat \Sigma _\I -\Sigma )  v \right| \ge C_2 \sqrt { \frac{s\log(np) }{|\I |  } } .$$
Since there are at most $n^2$ many different  choices of $ \I \subset (0,n]$, the desired result follows from a union bound argument. 
\end{proof}  


\bnlem
\label{lem:restricted eigenvalue}
Under \Cref{assp:dcdp_linear_reg}, it holds that
 \begin{align*}
		 \p \bigg( \sum_{t\in \I } ( X_t^\top v )^2 \ge \frac{c_x|\I| }{4} \|v\|_2^2 - C_2 \log(np) \|v\|_1 ^2 \ \forall v \in \mathbb R^p  \text{ and } \forall |\I|\ge C_s \s \log(np)  \bigg)  \le  n^{-5} 
	\end{align*} 
	where $  C_2 > 0$ is an  absolute constant  only depending on $C_x$.
\enlem
\begin{proof}
By the well known restricted eigenvalue condition, for any $\I$, it holds that 
 \begin{align*}
		 \p \bigg( \sum_{t\in \I } ( X_t^\top v )^2 \ge \frac{c_x |\I| }{4} \|v\|_2^2 - C_2 \log(np) \|v\|_1 ^2  \ \  \forall v \in \mathbb R^p    \bigg)  \le  C_3 \exp(-c_3|\I| ).
	\end{align*} 
  Since $|\I|  \ge  C_s \s \log(np) $, 
  \begin{align*}
		 \p \bigg( \sum_{t\in \I } ( X_t^\top v )^2 \ge \frac{c_ x |\I| }{4} \|v\|_2^2 - C_2 \log(np) \|v\|_1^2 \ \ \forall v \in \mathbb R^p    \bigg)  \le  n^{-4}.
	\end{align*} 
	Since there are at most $n^2$ many subinterval $\I \subset (0,n]$, it follows from a union bound argument  that 
	 \begin{align*}
		 \p \bigg( \sum_{t\in \I } ( X_t^\top v )^2 \ge \frac{c_x |\I| }{4} \|v\|_2^2 - C_2 \log(np) \|v\|_1^2  \ \ \forall v \in \mathbb R^p  \text{ and } \forall |\I|\ge C_s \s \log(np)  \bigg)  \le  n^{-2} .
	\end{align*} 
\end{proof} 




\bnlem \label{lemma:consistency}
Suppose  \Cref{assp:dcdp_linear_reg} holds. There exists  a sufficient large constant $ C_s$ such that the following conditions holds.    
\\
\\
{\bf a.} With probability at least $1-n^{-3} $, it holds that
\begin{align}\label{eq:independent condition 1c 1}
   \left |  \frac{1}{|\I | } \sum_{i \in \mathcal I }  \epsilon_i  X_i^\top \beta \right| \le C\sigma_{\epsilon}\sqrt { \frac{\log(np)}{|\I |   } } \|\beta\|_1      
 \end{align}
uniformly  for all $ \beta \in \mathbb R^p$ and all $\mathcal I \subset (0, n]$ such that $|\I|\ge C_s \s \log(np) $, 
\\
\\
 {\bf b.} Let $\{ u_i\}_{i=1}^n \subset  \mathbb R^p$  be a collection of  deterministic vectors. Then with probability at least $1-n^{-3} $, it holds that   
\begin{align}\label{eq:independent condition 1c}
       \left |  \frac{1}{|\I |   } \sum_{i \in \I }    u^\top_i   X_i   X_i^\top \beta  - \frac{1}{ |\I |  } \sum_{i \in \mathcal I }   u^\top  _i  \Sigma \beta  \right| \le C \left(  \max _{1\le i \le n }\|u_i\|_2  \right) \sqrt {  \frac{\log(np)}{|\I |   } } \|\beta\|_1    
 \end{align}
 uniformly for all $ \beta \in \mathbb R^p$ and all $\mathcal I \subset (0, n]$ such that $|\I|\ge  C_s \s \log(np) $.    
\enlem 
 \begin{proof}
   The justification   of the  \eqref{eq:independent condition 1c 1}  is   similar and simpler  than the justification  of \eqref{eq:independent condition 1c}. For conciseness, only the justification  of \eqref{eq:independent condition 1c} is presented.
   
For any $\mathcal I \subset (0, n]$  such  that $|\I|\ge  C_s \s \log(np) $, it holds  that
 \begin{align*}
 &\left|  \frac{1}{ |\I |  } \sum_{i\in \I }  u^\top  _i  X_i   X_i^\top \beta   - \frac{1}{ |\I |  }  \sum_{i\in \I }   u^\top_i  \Sigma  \beta \right| 
 \\
 =
 & \left|  \left(  \frac{1}{|\I |  } \sum_{i\in \I }   u^\top _i    X_i   X_i^\top     - \frac{1}{|\I |  }    \sum_{i\in \I }   u^\top_i  \Sigma  \right) \beta  \right| 
 \\
 \le 
 & \max_{1\le j \le p }  \left |  \frac{1}{|\I |  } \sum_{i\in \I }   u^\top  _i   X_i   X_{i,j}      - \frac{1}{|\I |  }    \sum_{i\in \I }   u^\top_i  \Sigma  (, j)  \right| \|\beta\|_1.
 \end{align*}
 Note that 
 $ E(u^\top  _i  X_i   X_{i,j} ) =u^\top _i \Sigma  (, j)    $ and in addition, 
 $$u^\top _ i   X_i   \sim N(0, u^\top _i  \Sigma u _i )  \quad \text{ and } \quad X_{i,j} \sim N(0, \Sigma({j,j}))  .$$
 So $u^\top _i   X_i X_{i,j} $  is a sub-exponential random variable such that 
 $$ u^\top _i   X_i X_{i,j} \sim SE( u^\top_i  \Sigma u _i  \Sigma ({j,j})).$$
 As a result, for $\gamma<1$ and every $j$,
$$ P \left( \left |  \frac{1}{|\I |  } \sum_{i \in \I }  u^\top _ i     X_i   X_{i,j}      - u^\top \Sigma  (, j)  \right|  \ge \gamma \sqrt {  \max_{1\le i\le n } ( u^\top_i  \Sigma u_i)  \Sigma ( {j,j} ) }\right) \le \exp(-c \gamma^2 |\I |  ). $$
Since 
$$  \sqrt { u^\top _i  \Sigma u _i \Sigma ({j,j} ) } \le C_x  \|u_i \|_2, $$
by union bound,
$$ \p \left(  \max_{1\le j \le p }\left |  \frac{1}{|\I |  } \sum_{i \in \I}  u^\top _ i     X_i   X_{i,j}      - \frac{1}{|\I |  } \sum_{i \in\I}  u^\top _i  \Sigma  (, j)  \right|  \ge \gamma 
C_x  \left(  \max _{1\le i \le n }\|u_i\|_2  \right)  \right) \le p\exp(-c \gamma^2  |\I| ). $$
Let $\gamma =  3\sqrt { \frac{\log(np) }{c  |\I| }  }$. Note that   $ \gamma<1$ if  $|\I|\ge C_s \s \log(np) $ for sufficiently large $C_s$.  Therefore 
$$ \p \left(  \max_{1\le j \le p }\left |  \frac{1}{|\I |  } \sum_{i \in \I}  u^\top _ i     X_i   X_{i,j}      - \frac{1}{|\I |  } \sum_{i \in\I}  u^\top _i  \Sigma  (, j)  \right|  \ge  
C_1\sqrt{ \frac{ \log(np)}{|\I| } } \left(  \max _{1\le i \le n }\|u_i\|_2  \right)  \right) \le p\exp(-9\log(np)  ). $$
Since there are at most $n^2$ many intervals $\I \subset(0,n]$, it follows that 
\begin{align*}
 &\p \left(  \max_{1\le j \le p }\left |  \frac{1}{|\I |  } \sum_{i \in \I}  u^\top _ i     X_i   X_{i,j}      - \frac{1}{|\I |  } \sum_{i \in\I}  u^\top _i  \Sigma  (, j)  \right|  \ge  
C_1\sqrt{ \frac{ \log(np)}{|\I| } } \left(  \max _{1\le i \le n }\|u_i\|_2   \right) \ \forall    |\I| \ge C_s \s \log(np)  \right)
\\
 \le & p n^2 \exp(-9\log(np)  ) \le n^{-3}. 
\end{align*}
This immediately  gives \eqref{eq:independent condition 1c}.
 \end{proof} 
 
 
 
 
 \bnlem\label{lem-x-bound}
Uder \Cref{assp:dcdp_linear_reg}, for any interval $\I \subset (0, n]$, for any 
	\[
		\lambda \geq \lambda_1 := C_{\lambda}\sigma_{\epsilon} \sqrt{\log(n p)},
	\]
	where $C_{\lambda} > 0$ is a large enough absolute constant, it holds with probability at least $1 - n^{-5}$ that
	\[
    \|\sum_{i \in \I} \epsilon_i X_i \|_{\infty} \leq \lambda \sqrt{\max\{|\I|, \, \log(n p)\}}/8,
	\]
	where $c_3 > 0$ is an absolute constant depending only on the distributions of covariants $\{X_i\}$ and $\{\epsilon_i\}$.
\enlem

\begin{proof}
	Since $\epsilon_i$'s are sub-Gaussian random variables and $X_i$'s are sub-Gaussian random vectors, we have that $\epsilon_i X_i$'s are sub-Exponential random vectors with $\|\epsilon_iX_i\|_{\psi_1}\leq C_x \sigma_{\epsilon}$ \citep[see e.g.~Lemma~2.7.7 in][]{vershynin2018high}. It then follows from Bernstein's inequality \citep[see e.g.~Theorem~2.8.1 in][]{vershynin2018high} that for any $t > 0$,
		\[
	\mathbb{P}\left\{\|\sum_{i \in \I} \epsilon_i X_i \|_{\infty} > t\right\} \leq 2p \exp\left\{-c \min\left\{\frac{t^2}{|\I|C_x^2\sigma^2_{\epsilon}}, \, \frac{t}{C_x \sigma_{\epsilon}}\right\}\right\}.
		\]
		Taking 
		\[
			t = C_{\lambda}C_x/4 \sigma_{\epsilon} \sqrt{\log(n p)} \sqrt{\max\{|\I|, \, \log(n p)\}}
		\] 
		yields the conclusion.
\end{proof}
 
 
 
 

\bnlem \label{lemma:beta bounded 1}
Suppose   \Cref{assp:dcdp_linear_reg} holds. Let $\I \subset [1,n] $. Denote 
 $ \kappa = \min_{k\in \{1,\ldots, K\} } \kappa_k,$ 
where $ \{ \kappa_k\}_{k=1}^K$ are defined in  \Cref{assp:dcdp_linear_reg}. Then for any $i\in [T]$,
   $$\|\beta^*_\I - \beta^*_i\|_2  \le C\kappa  \le CC_\kappa,$$
  for some absolute constant $C$ independent of $n$.
\enlem 
 \begin{proof}
 It suffices to consider $\I =[1,n]$  and  $\beta_i^*= \beta_1^*$ as the general case is similar. Observe that  
 \begin{align*}
  \| \beta^*_{[1,n]}  - \beta_ 1^*  \|_2  =& 
  \|  \frac{1}{n} \sum_{i=1}^n \beta_i ^*  - \beta_1^*  
   \|_2 
 = \|  \frac{1}{n} \sum_{k=0}^{K} \Delta_k \beta_{\eta_k+ 1} ^*   -    \frac{1}{n}\sum_{k=0}^{K} \Delta_k  \beta_1 ^*
  \|_2  
  \\
 \le 
 &    \frac{1}{n} \sum_{k=0}^{K} \left\| \Delta_k  (\beta_{\eta_k+ 1} ^* -\beta_1 ^* ) \right\|_2    \le 
 \frac{1}{n}\sum_{k=0}^{K} \Delta_k  (K+1)  \kappa   \le  (K+1)\kappa . 
  \end{align*}
  By \Cref{assp:dcdp_linear_reg}, both $\kappa $ and $K $ bounded above. 
 \end{proof}
 
 \bnlem\label{eq:cumsum upper bound}
 Let $t\in \I =(s,e] \subset [1,n]$. Denote 
 $ \kappa_{\max}= \max_{k\in \{1,\ldots, K\} } \kappa_k,$ 
where $ \{ \kappa_k\}_{k=1}^K$ are defined in  \Cref{assp:dcdp_linear_reg}.  Then   
 $$ \sup_{0< s < t<e\le n  }\| \beta_{ (s, t]}  ^* - \beta_{(t,e] }  ^* \|_2  \le C\kappa  \le CC_\kappa. $$ 
for some absolute constant $C$ independent of $n$. 
 \enlem
 \begin{proof}
 It suffices to consider $(s,e]=(0,n]$, as the general case is similar.  
 Suppose that $\eta_{q} <t \le \eta_{q+1} $.
 Observe that 
 \begin{align*}
&  \| \beta^*_{(1,t]}  - \beta ^* _{(t,n]}  \|_2  
  \\
  =& 
  \left\|  \frac{1}{t } \sum_{i=1}^t \beta_i ^*  - \frac{1}{ n- t } \sum_{i=t+1}^n \beta_i ^*
  \right \|_2 
 \\
 = & \left\|  \frac{1}{t}  \left( \sum_{k=0}^{q-1} \Delta_k \beta_{\eta_k+ 1}  ^*  + (t-\eta_{q} )\beta^*_{\eta_q + 1} \right) -    \frac{1}{n-t } \left( \sum_{k=q+1}^{K}  \Delta_k \beta_{\eta_k+ 1} ^*   + ( \eta_{q+1}-t  )\beta^*_{\eta_q + 1} \right) 
  \right \|_2  
  \\
=
 & \left\|  \frac{1}{t}  \left( \sum_{k=0}^{q-1} \Delta_k (\beta ^* _{\eta_k+ 1}-\beta^*_{\eta_q+1} ) \right)  +  \beta^*_{\eta_q + 1} -    \frac{1}{n-t } \left( \sum_{k=q+1}^{K}  \Delta_k (  \beta ^* _{\eta_k+ 1}  -\beta ^* _{\eta_q+1} ) \right)   -  \beta^*_{\eta_q + 1} 
  \right \|_2 
  \\
  =
  &\left\|  \frac{1}{t}  \left( \sum_{k=0}^{q-1} \Delta_k (\beta_{\eta_k+ 1} ^* -\beta^*_{\eta_q+1} ) \right)    -    \frac{1}{n-t } \left( \sum_{k=q+1}^{K}  \Delta_k (  \beta_{\eta_k+ 1} ^*   -\beta_{\eta_q+1} ^*  ) \right)   
  \right \|_2 
  \\
  \le 
  &\frac{1}{t} \sum_{k=0}^{q-1} \Delta_k    K \kappa      +\frac{1}{n-t} \sum_{k=q+1}^{K} \Delta_k    K  \kappa 
  \le 2K\kappa  . 
  \end{align*}
  
 \end{proof}















\clearpage


\subsection{Local refinement}
In this section, we prove results related to the $O_p(1)$ rates of localization error.
\begin{enumerate}
    \item \Cref{sec:op1 fundations} presents two fundamental lemmas to prove other results.
    \item \Cref{sec:mean op1} prove results for the mean model.
    \item \Cref{sec:cov op1} prove results for the covariance model.
    \item \Cref{sec:regression op1} prove results for the regression model.
\end{enumerate}


\subsubsection{Fundamental lemma}
\label{sec:op1 fundations}


\bnlem
\label{lem:subexp deviation martingale}
Suppose $\left\{z_i\right\}_{i=1}^{\infty}$ is a collection of independent centered sub-exponential random variable with $0<\sup _{1 \leq i<\infty}\left\|z_i\right\|_{\psi_1} \leq 1$. Then for any integer $d>0, \alpha>0$ and any $x>0$
$$
\mathbb{P}\left(\max _{k \in[d,(1+\alpha) d]} \frac{\sum_{i=1}^k z_i}{\sqrt{k}} \geq x\right) \leq \exp \left\{-\frac{x^2}{2(1+\alpha)}\right\}+\exp \left\{-\frac{\sqrt{d} x}{2}\right\} .
$$
\enlem
\bprf
Denote $S_n=\sum_{i=1}^n z_i$. Let $\zeta=\sup _{1 \leq i \leq \infty}\left\|z_i\right\|_{\psi_1}$. For any two integers $m<n$ and any $t \leq \frac{C_1}{\zeta}$
$$
\mathbb{E}\left(\exp \left(t\left(S_n-S_m\right)\right)\right) \leq \prod_{i=m+1}^n \mathbb{E}\left(\exp \left(t z_i\right)\right) \leq \prod_{i=m+1}^n \mathbb{E}\left(C_1^2 t^2 / 2\right)=\mathbb{E}\left[(n-m) C_1^2 t^2 / 2\right].
$$
Let $\mathcal{F}_k$ denote the sigma-algebra generated by $\left(z_1, \ldots, z_k\right)$. Without loss of generality, assume that $C_1=1$. Since $S_k$ is independent of $S_n-S_k$, this implies that when $t \geq 1 / \zeta$
$$
\mathbb{E}\left(\exp \left\{t S_n-\frac{t^2 n}{2}\right\} \mid \mathcal{F}_k\right)=\exp \left\{t S_k-\frac{t^2 k}{2}\right\} \mathbb{E}\left(\exp \left\{t\left(S_n-S_k\right)\right\}-\frac{t^2(n-k)}{2}\right) \leq \exp \left\{t S_k-\frac{t^2 k}{2}\right\}
$$
Therefore $\exp \left\{t S_n-\frac{t^2 n}{2}\right\}$ is a super-Martingale. Let $x$ be given and
$$
A=\inf \left\{n \geq d, S_n \geq \sqrt{n} x\right\} .
$$
Then $S_A \geq \sqrt{A} x \geq \sqrt{d} x$. Thus for $t \geq 1 / \zeta$,
$$
\mathbb{E}\left(\exp \left\{t \sqrt{d} x-\frac{t^2 A}{2}\right\}\right) \leq \mathbb{E}\left(\exp \left\{t S_A-\frac{t^2 A}{2}\right\}\right) \leq \mathbb{E}\left(\exp \left\{t S_1-\frac{t^2}{2}\right\}\right) \leq 1 .
$$
By definition of $A$,
$$
\mathbb{P}\left(\max _{k \in[d,(1+\alpha) d]} \frac{\sum_{i=1}^k z_i}{\sqrt{k}} \geq x\right) \leq \mathbb{P}(A \leq(1+\alpha) d) .
$$
Since $u \rightarrow \exp \left(s \sqrt{d} x-\frac{t^2 u}{2}\right)$ is decreasing, it follows that
$$
\mathbb{P}\left(\max _{k \in[d,(1+\alpha) d]} \frac{\sum_{i=1}^k z_i}{\sqrt{k}} \geq x\right) \leq \mathbb{P}\left(\exp \left\{t \sqrt{d} x-t^2 A / 2\right\} \geq \exp \left\{t \sqrt{d} x-t^2(1+\alpha) d / 2\right\}\right) .
$$
Markov's inequality implies that when $t \geq \frac{1}{\zeta}$,
$$
\mathbb{P}\left(\max _{k \in[d,(1+\alpha) d]} \frac{\sum_{i=1}^k z_i}{\sqrt{k}} \geq x\right) \leq \exp \left\{-t \sqrt{d} x+t^2(1+\alpha) d / 2\right\}
$$
Set
$$
t=\min \left\{\frac{1}{\zeta}, \frac{x}{(1+\alpha) \sqrt{d}}\right\}
$$
If $\frac{1}{\zeta} \geq \frac{x}{(1+\alpha) \sqrt{d}}$. Then $t=\frac{x}{(1+\alpha) \sqrt{d}}$ and therefore
$$
-t \sqrt{d} x+t^2(1+\alpha) d / 2=-\frac{x^2}{2(1+\alpha)}
$$
So
$$
\mathbb{P}\left(\max _{k \in[d,(1+\alpha) d]} \frac{\sum_{i=1}^k z_i}{\sqrt{k}} \geq x\right) \leq \exp \left\{-\frac{x^2}{2(1+\alpha)}\right\} .
$$
If $\frac{1}{\zeta} \leq \frac{x}{(1+\alpha) \sqrt{d}}$. Then $t=\frac{1}{\zeta} \leq \frac{x}{(1+\alpha) \sqrt{d}}$ and so
$$
-t \sqrt{d} x+t^2(1+\alpha) d / 2 \leq \frac{-\sqrt{d} x}{\zeta}+\frac{1}{\zeta} \frac{x}{(1+\alpha) \sqrt{d}} \frac{(1+\alpha) d}{2}=\frac{-\sqrt{d} x}{2 \zeta} .
$$
So
$$
\mathbb{P}\left(\max _{k \in[d,(1+\alpha) d]} \frac{\sum_{i=1}^k z_i}{\sqrt{k}} \geq x\right) \leq \exp \left\{-\frac{\sqrt{d} x}{2 \zeta}\right\} \leq \exp \left\{-\frac{\sqrt{d} x}{2}\right\},
$$
where $\zeta \leq 1$ is used in the last inequality. Putting the two cases together leads the desired result.
\eprf



\bnlem
\label{lem:subexp uniform loglog law}
Suppose $\left\{z_i\right\}_{i=1}^{\infty}$ is a collection of independent centered sub-exponential random variable with $0<\sup _{1 \leq i<\infty}\left\|z_i\right\|_{\psi_1} \leq 1$. Let $\nu>0$ be given. For any $x>0$, it holds that
$$
\mathbb{P}\left(\sum_{i=1}^r z_i \leq 4 \sqrt{r\{\log \log (4 \nu r)+x+1\}}+4 \sqrt{r \nu}\{\log \log (4 \nu r)+x+1\} \text { for all } r \geq 1 / \nu\right) \geq 1-2 \exp (-x) \text {. }
$$
\enlem
\bprf
Let $s \in \mathbb{Z}^{+}$and $\mathcal{T}_s=\left[2^s / \nu, 2^{s+1} / \nu\right]$. By \Cref{lem:subexp deviation martingale}, for all $x>0$,
$$
\mathbb{P}\left(\sup _{r \in \mathcal{T}_s} \frac{\sum_{i=1}^r z_i}{\sqrt{r}} \geq x\right) \leq \exp \left\{-\frac{x^2}{4}\right\}+\exp \left\{-\frac{\sqrt{2^s / \nu} x}{2}\right\} \leq \exp \left\{-\frac{x^2}{4}\right\}+\exp \left\{-\frac{x}{2 \sqrt{\nu}}\right\} .
$$
Therefore by a union bound,
\begin{align}
    & \mathbb{P}\left(\exists s \in \mathbb{Z}^{+}: \sup _{r \in \mathcal{T}_s} \frac{\sum_{i=1}^r z_i}{\sqrt{r}} \geq 2 \sqrt{\log \log ((s+1)(s+2))+x}+2 \sqrt{\nu}\{\log \log ((s+1)(s+2))+x\}\right) \nonumber \\
\leq & \sum_{s=0}^{\infty} 2 \frac{\exp (-x)}{(s+1)(s+2)}=2 \exp (-x) \label{tmp_eq: iterated log}.
\end{align}
For any $r \geq 2^s / \nu, s \leq \log (r \nu) / \log (2)$, and therefore
$$
(s+1)(s+2) \leq \frac{\log (2 r \nu) \log (4 r \nu)}{\log ^2(2)} \leq\left(\frac{\log (4 r \nu)}{\log (2)}\right)^2 .
$$
Thus
$$
\log ((s+1)(s+2)) \leq 2 \log \left(\frac{\log (4 r \nu)}{\log (2)}\right) \leq 2 \log \log (4 r \nu)+1 .
$$
The above display together with \eqref{tmp_eq: iterated log} gives
$$
\mathbb{P}\left(\sup _{r \geq 1 / \nu} \frac{\sum_{i=1}^r z_i}{\sqrt{r}} \geq 2 \sqrt{2 r \log \log (4 r \nu)+x+1}+2 \sqrt{r \nu}\{\log \log (4 r \nu)+x+1\}\right) \leq 2 \exp (-x) .
$$
\eprf

















\clearpage
\subsubsection{Mean}
\label{sec:mean op1}
Suppose $\alpha^*,\beta^*\in \mathbb{R}^p$ and
$$
y_i=\begin{cases}
\alpha^*+\epsilon_i & \text { when } i \in(0, \eta] \\
\beta^*+\epsilon_i & \text { when } i \in(\eta, n]
\end{cases}
$$
where $\{\epsilon_i\}$ is an i.i.d sequence of subgaussian variables such that $\|\epsilon_i\|_{\psi_2}=\sigma_\epsilon<\infty$. In addition, suppose that there exists $\theta \in(0,1)$ such that $\eta=\lfloor n \theta\rfloor$ and that $\|\alpha^*-\beta^*\|_2=\kappa<\infty$. Suppose that $\|\alpha^*\|_0 \leq \mathfrak{s},\|\beta^*\|_0 \leq \mathfrak{s}$ and that
\begin{equation}
    \frac{\mathfrak{s} \log ^{3 / 2}(p)}{\sqrt{n}} \rightarrow 0, \quad \frac{\mathfrak{s}^2 \log ^{3 / 2}(p)}{n \kappa} \rightarrow 0, \quad \frac{\mathfrak{s} \log ^{3 / 2}(p)}{\sqrt{n} \kappa} \rightarrow 0, \quad \frac{\mathfrak{s} \log (p)}{n \kappa^2} \rightarrow 0.
    \label{op1_eq:mean snr}
\end{equation}
Suppose there exists $\widehat{\alpha}$ and $\widehat{\beta}$ such that
\begin{align*}
  & \|\widehat{\alpha}-\alpha^*\|_2^2=O_p\left(\frac{\mathfrak{s} \log (p)}{n}\right) \text{ and } \|\widehat{\alpha}-\alpha^*\|_1=O_p\left(\mathfrak{s} \sqrt{\frac{\log (p)}{n}}\right); \\
& \|\widehat{\beta}-\beta^*\|_2^2=O_p\left(\frac{\mathfrak{s} \log (p)}{n}\right) \text{ and } \|\widehat{\beta}-\beta^*\|_1=O_p\left(\mathfrak{s} \sqrt{\frac{\log (p)}{n}}\right).
\end{align*}
Let
$$
\widehat{\mathcal{Q}}(k)=\sum_{i=1}^k\|y_i- \widehat{\alpha}\|_2^2+\sum_{i=k+1}^n\|y_i-\widehat{\beta}\|_2^2 \quad \text { and } \quad \mathcal{Q}^*(k)=\sum_{i=1}^k\|y_i- \alpha^*\|_2^2+\sum_{i=k+1}^n\|y_i- \beta^*\|_2^2 .
$$

\bnlem[Refinement for the mean model]
Let
$$
\eta+r=\underset{k \in(0, n]}{\arg \max } \widehat{\mathcal{Q}}(k) .
$$
Then under the assumptions above, it holds that
$$
\kappa^2 r=O_p(1) .
$$
\enlem
\bprf
By assumptions above, we have
$$
\frac{\mathfrak{s} \log ^{3 / 2}}{\sqrt{n}} \rightarrow 0, \quad \frac{\mathfrak{s}^2 \log ^{3 / 2}(p)}{n \kappa} \rightarrow 0, \quad \frac{\mathfrak{s} \log ^{3 / 2}(p)}{\sqrt{n} \kappa} \rightarrow 0, \quad \frac{\mathfrak{s} \log (p)}{n \kappa^2} \rightarrow 0 .
$$
Without loss of generality, suppose $r \geq 0$. Since $\eta+r$ is the minimizer, it follows that
$$
\widehat{\mathcal{Q}}(\eta+r) \leq \widehat{\mathcal{Q}}(\eta) .
$$
If $r \leq \frac{1}{\kappa^2}$, then there is nothing to show. So for the rest of the argument, for contradiction, assume that
$$
r \geq \frac{1}{\kappa^2}
$$
Observe that
$$
\begin{aligned}
\widehat{\mathcal{Q}}(\eta + r)-\widehat{\mathcal{Q}}(\eta) &=\sum_{i=\eta+1}^{\eta+r}\|y_i- \widehat{\alpha}\|_2^2-\sum_{i=\eta+1}^{\eta+r}\|y_i-\widehat{\beta}\|_2^2 \\
\mathcal{Q}^*(\eta + r)-\mathcal{Q}^*(\eta) &=\sum_{i=\eta+1}^{\eta+r}\|y_i- \alpha^*\|_2^2-\sum_{i=\eta+1}^{\eta+r}\|y_i- \beta^*\|_2^2
\end{aligned}
$$
\textbf{Step 1}. It follows that
$$
\begin{aligned}
& \sum_{i=\eta+1}^{\eta+r}\|y_i- \widehat{\alpha}\|_2^2-\sum_{i=\eta+1}^{\eta+r}\|y_i-\alpha^*\|_2^2 \\
=& \sum_{i=\eta+1}^{\eta+r}\|\widehat{\alpha}- \alpha^*\|_2^2+2\left(\widehat{\alpha}-\alpha^*\right)^{\top} \sum_{i=\eta+1}^{\eta+r}\left(y_i-\alpha^*\right) \\
=& \sum_{i=\eta+1}^{\eta+r}\|\widehat{\alpha}- \alpha^*\|_2^2+2r\left(\widehat{\alpha}-\alpha^*\right)^{\top} \left(\beta^*-\alpha^*\right) +2\left(\widehat{\alpha}-\alpha^*\right)^{\top} \sum_{i=\eta+1}^{\eta+r}\epsilon_i
\end{aligned}
$$
By assumptions, we have
$$
\sum_{i=\eta+1}^{\eta+r}\|\widehat{\alpha}- \alpha^*\|_2^2 \leq C r \frac{\mathfrak{s} \log (p)}{n} \\
=o_p\left(r \sigma^2_{\epsilon} \kappa^2\right).
$$
Similarly
$$
r\left(\widehat{\alpha}-\alpha^*\right)^{\top}\left(\beta^*-\alpha^*\right)\leq r\|\widehat{\alpha}-\alpha^*\|_2\|\beta^*-\alpha^*\|_2 \leq
O_p\left(r\kappa \sqrt{\frac{\mathfrak{s} \log (p)}{n} } \right)=o_p\left(r\kappa^2\right)
$$
where the second equality follows from $\|\beta^*-\alpha^*\|_2=\kappa$, and the last equality follows from \eqref{op1_eq:mean snr}. In addition,
$$
\begin{aligned}
&\left(\widehat{\alpha}-\alpha^*\right)^{\top} \sum_{i=\eta+1}^{\eta+r} \epsilon_i \leq\|\widehat{\alpha}-\alpha^*\|_1\|\sum_{i=\eta+1}^{\eta+r}\epsilon_i\|_{\infty} \\
=& O_p\left(\mathfrak{s} \sqrt{\frac{\log (p)}{n}}\right) O_p(\sqrt{r \log (p)})=O_p(\kappa \sqrt{r})
\end{aligned}
$$
Therefore
$$
\sum_{i=\eta+1}^{\eta+r}\|y_i- \widehat{\alpha}\|_2^2-\sum_{i=\eta+1}^{\eta+r}\|y_i-\alpha^*\|_2^2=O_p(\kappa \sqrt{r})+o_p\left(r \kappa^2\right) .
$$
\textbf{Step 2}. Using the same argument as in the previous step, it follows that
$$
\sum_{i=\eta+1}^{\eta+r}\|y_i- \widehat{\beta}\|_2^2-\sum_{i=\eta+1}^{\eta+r}\|y_i- \beta^*\|_2^2=O_p(\kappa \sqrt{r})+o_p(r \kappa^2) .
$$
Therefore
\begin{equation}
    \left|\widehat{\mathcal{Q}}(\eta+r)-\widehat{\mathcal{Q}}(\eta)-\left\{\mathcal{Q}^*(\eta+r)-\mathcal{Q}^*(\eta)\right\}\right|=O_p(\kappa \sqrt{r})+o_p\left(r \kappa^2\right)
    \label{tmp_eq:op1 mean main prop eq 1}
\end{equation}
\textbf{Step 3}. Observe that
$$
\begin{aligned}
\mathcal{Q}^*(\eta+r)-\mathcal{Q}^*(\eta) 
=& \sum_{i=\eta+1}^{\eta+r}\|y_i- \alpha^*\|_2^2-\sum_{i=\eta+1}^{\eta+r}\|y_i- \beta^*\|_2^2 \\
=& r\| \alpha^*- \beta^*\|_2^2-2 \sum_{i=\eta+1}^{\eta+r}(y_i- \beta^*)( \alpha^*- \beta^*) \\
=& r\| \alpha^*- \beta^*\|_2^2 -2 (\alpha^*- \beta^*)^\top\sum_{i=\eta+1}^{\eta+r} \epsilon_i
\end{aligned}
$$
Let
$$
w_i=\frac{1}{\sigma_{\epsilon}\kappa} \epsilon_i^\top\left( \alpha^*-\beta^*\right)
$$
Then $\left\{w_i\right\}_{i=1}^{\infty}$ are subgaussian random variables with bounded $\psi_2$ norm. Therefore by \Cref{lem:subexp uniform loglog law}, uniformly for all $r \geq 1 / \kappa^2$,
$$
\sum_{i=1}^r w_i=O_p\left(\sqrt{r\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right)
$$
Since $\kappa<\infty$, it follows that
$$
\sum_{i=\eta+1}^{\eta+r} \epsilon_i^\top \left( \alpha^*-\beta^*\right)=O_p\left(\sqrt{r \kappa^2\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right)
$$
Therefore
\begin{equation}
    \mathcal{Q}^*(\eta+r)-\mathcal{Q}^*(\eta) = r \kappa^2+O_p\left(\sqrt{r \kappa^2\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right)
\label{tmp_eq:op1 mean main prop eq 2}
\end{equation}

\textbf{Step 4}. \Cref{tmp_eq:op1 mean main prop eq 1} and \Cref{tmp_eq:op1 mean main prop eq 2} together give, uniformly for all $r \geq 1 / \kappa^2$,
$$
 r \kappa^2+O_p\left(\sqrt{r \kappa^2\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right) \leq O_p(\kappa \sqrt{r})+o_p\left(r \kappa^2\right)
$$
This implies that
$$
r \kappa^2=O_p()
$$
\eprf

% \bprf
% By assumptions above, we have
% $$
% \frac{\mathfrak{s} \log ^{3 / 2}}{\sqrt{n}} \rightarrow 0, \quad \frac{\mathfrak{s}^2 \log ^{3 / 2}(p)}{n \kappa} \rightarrow 0, \quad \frac{\mathfrak{s} \log ^{3 / 2}(p)}{\sqrt{n} \kappa} \rightarrow 0, \quad \frac{\mathfrak{s} \log (p)}{n \kappa^2} \rightarrow 0 .
% $$
% Without loss of generality, suppose $r \geq 0$. Since $\eta+r$ is the minimizer, it follows that
% $$
% \widehat{\mathcal{Q}}(\eta+r) \leq \widehat{\mathcal{Q}}(\eta) .
% $$
% If $r \leq \frac{1}{\kappa^2}$, then there is nothing to show. So for the rest of the argument, for contradiction, assume that
% $$
% r \geq \frac{1}{\kappa^2}
% $$
% Observe that
% $$
% \begin{aligned}
% \widehat{\mathcal{Q}}(\eta + r)-\widehat{\mathcal{Q}}(\eta) &=\sum_{i=\eta+1}^{\eta+r}\|y_i- \widehat{\alpha}\|_2^2-\sum_{i=\eta+1}^{\eta+r}\|y_i-\widehat{\beta}\|_2^2 \\
% \mathcal{Q}^*(\eta + r)-\mathcal{Q}^*(\eta) &=\sum_{i=\eta+1}^{\eta+r}\|y_i- \alpha^*\|_2^2-\sum_{i=\eta+1}^{\eta+r}\|y_i- \beta^*\|_2^2
% \end{aligned}
% $$
% \textbf{Step 1}. It follows that
% $$
% \begin{aligned}
% & \sum_{i=\eta+1}^{\eta+r}\|y_i- \widehat{\alpha}\|_2^2-\sum_{i=\eta+1}^{\eta+r}\|y_i-\alpha^*\|_2^2 \\
% =& \sum_{i=\eta+1}^{\eta+r}\|\widehat{\alpha}- \alpha^*\|_2^2+2\left(\widehat{\alpha}-\alpha^*\right)^{\top} \sum_{i=\eta+1}^{\eta+r}\left(y_i-\alpha^*\right) \\
% =& \sum_{i=\eta+1}^{\eta+r}\|\widehat{\alpha}- \alpha^*\|_2^2+2r\left(\widehat{\alpha}-\alpha^*\right)^{\top} \left(\beta^*-\alpha^*\right) +2\left(\widehat{\alpha}-\alpha^*\right)^{\top} \sum_{i=\eta+1}^{\eta+r}\epsilon_i
% \end{aligned}
% $$
% By assumptions, we have
% $$
% \sum_{i=\eta+1}^{\eta+r}\|\widehat{\alpha}- \alpha^*\|_2^2 =O_p\left(r \frac{\sigma_{\epsilon}^2\mathfrak{s} \log (p)}{n}\right) \\
% =o_p\left(r \sigma^2_{\epsilon} \kappa^2\right).
% $$
% Similarly
% $$
% r\left(\widehat{\alpha}-\alpha^*\right)^{\top}\left(\beta^*-\alpha^*\right)\leq r\|\widehat{\alpha}-\alpha^*\|_2\|\beta^*-\alpha^*\|_2 \leq
% O_p\left(r\sigma_{\epsilon}\kappa \sqrt{\frac{\mathfrak{s} \log (p)}{n} } \right)=o_p\left(r\sigma_{\epsilon} \kappa^2\right)
% $$
% where the second equality follows from $\|\beta^*-\alpha^*\|_2=\kappa$, and the last equality follows from \eqref{op1_eq:mean snr}. In addition,
% $$
% \begin{aligned}
% &\left(\widehat{\alpha}-\alpha^*\right)^{\top} \sum_{i=\eta+1}^{\eta+r} \epsilon_i \leq\|\widehat{\alpha}-\alpha^*\|_1\|\sum_{i=\eta+1}^{\eta+r}\epsilon_i\|_{\infty} \\
% =& O_p\left(\sigma_{\epsilon}\mathfrak{s} \sqrt{\frac{\log (p)}{n}}\right) O_p(\sigma_{\epsilon}\sqrt{r \log (p)})=O_p(\sigma_{\epsilon}^2\kappa \sqrt{r})
% \end{aligned}
% $$
% Therefore
% $$
% \sum_{i=\eta+1}^{\eta+r}\|y_i- \widehat{\alpha}\|_2^2-\sum_{i=\eta+1}^{\eta+r}\|y_i-\alpha^*\|_2^2=O_p(\kappa \sqrt{r}\sigma_{\epsilon}^2)+o_p\left(r \kappa^2\sigma_{\epsilon}^2\right) .
% $$
% \textbf{Step 2}. Using the same argument as in the previous step, it follows that
% $$
% \sum_{i=\eta+1}^{\eta+r}\|y_i- \widehat{\beta}\|_2^2-\sum_{i=\eta+1}^{\eta+r}\|y_i- \beta^*\|_2^2=O_p(\kappa \sqrt{r}\sigma_{\epsilon}^2)+o_p(r \kappa^2\sigma_{\epsilon}^2) .
% $$
% Therefore
% \begin{equation}
%     \left|\widehat{\mathcal{Q}}(\eta+r)-\widehat{\mathcal{Q}}(\eta)-\left\{\mathcal{Q}^*(\eta+r)-\mathcal{Q}^*(\eta)\right\}\right|=O_p(\kappa \sqrt{r}\sigma_{\epsilon}^2)+o_p\left(r \kappa^2\sigma_{\epsilon}^2\right)
%     \label{tmp_eq:op1 mean main prop eq 1}
% \end{equation}
% \textbf{Step 3}. Observe that
% $$
% \begin{aligned}
% \mathcal{Q}^*(\eta+r)-\mathcal{Q}^*(\eta) 
% =& \sum_{i=\eta+1}^{\eta+r}\|y_i- \alpha^*\|_2^2-\sum_{i=\eta+1}^{\eta+r}\|y_i- \beta^*\|_2^2 \\
% =& r\| \alpha^*- \beta^*\|_2^2-2 \sum_{i=\eta+1}^{\eta+r}(y_i- \beta^*)( \alpha^*- \beta^*) \\
% =& r\| \alpha^*- \beta^*\|_2^2 -2 (\alpha^*- \beta^*)^\top\sum_{i=\eta+1}^{\eta+r} \epsilon_i
% \end{aligned}
% $$
% Let
% $$
% w_i=\frac{1}{\sigma_{\epsilon}\kappa} \epsilon_i^\top\left( \alpha^*-\beta^*\right)
% $$
% Then $\left\{w_i\right\}_{i=1}^{\infty}$ are subgaussian random variables with bounded $\psi_2$ norm. Therefore by \Cref{lem:subexp uniform loglog law}, uniformly for all $r \geq 1 / \kappa^2$,
% $$
% \sum_{i=1}^r w_i=O_p\left(\sqrt{r\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right)
% $$
% Since $\kappa<\infty$, it follows that
% $$
% \sum_{i=\eta+1}^{\eta+r} \epsilon_i^\top \left( \alpha^*-\beta^*\right)=O_p\left(\sqrt{r \kappa^2\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right)
% $$
% Therefore
% \begin{equation}
%     \mathcal{Q}^*(\eta+r)-\mathcal{Q}^*(\eta) = r \kappa^2+O_p\left(\sqrt{r \kappa^2\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right)
% \label{tmp_eq:op1 mean main prop eq 2}
% \end{equation}

% \textbf{Step 4}. \Cref{tmp_eq:op1 mean main prop eq 1} and \Cref{tmp_eq:op1 mean main prop eq 2} together give, uniformly for all $r \geq 1 / \kappa^2$,
% $$
%  r \kappa^2+O_p\left(\sqrt{r \kappa^2\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right) \leq O_p(\kappa \sqrt{r}\sigma_{\epsilon}^2)+o_p\left(r \kappa^2\sigma_{\epsilon}^2\right)
% $$
% This implies that
% $$
% r \kappa^2=O_p(\sigma_{\epsilon}^2)
% $$
% \eprf













\clearpage
\subsubsection{Covariance}
\label{sec:cov op1}
Suppose $G^*,H^*\in \mathbb{R}^d$ and
$$
\mathbb{E}[X_iX_i^\top]=\left\{\begin{array}{ll}
G^* & \text { when } i \in(0, \eta] \\
H^* & \text { when } i \in(\eta, n]
\end{array} .\right.
$$
In addition, suppose that there exists $\theta \in(0,1)$ such that $\eta=\lfloor n \theta\rfloor$ and that $\|G^*-H^*\|_2=\kappa_{\Sigma}<\infty$. Suppose that $c_XI_d \preceq G^* \preceq C_X I_d$, $c_XI_d \preceq H^* \preceq C_X I_d$, and that
\begin{equation}
    \frac{d^{5/2} \log ^{3 / 2}(nd)}{\sqrt{n}} \rightarrow 0, \quad \frac{d^2 \log ^{3 / 2}(nd)}{n \kappa_{\Sigma}} \rightarrow 0, \quad \frac{d \log ^{3 / 2}(nd)}{\sqrt{n} \kappa_{\Sigma}} \rightarrow 0, \quad \frac{d \log (nd)}{n \kappa_{\Sigma}^2} \rightarrow 0.
    \label{op1_eq:cov snr}
\end{equation}
By \Cref{lem:estimation covariance}, there exist $\widehat{G},\widehat{H}$ such that
\begin{align*}
  & \|\widehat{G}-G^*\|_2=O_p\left(\sqrt{\frac{d \log (nd)}{n}}\right) \text{ and } \|\widehat{G}-G^*\|_F=O_p\left(d \sqrt{\frac{\log (nd)}{n}}\right); \\
& \|\widehat{H}-H^*\|_2=O_p\left(\sqrt{\frac{d \log (nd)}{n}}\right) \text{ and } \|\widehat{H}-H^*\|_F=O_p\left(d \sqrt{\frac{\log (nd)}{n}}\right).
\end{align*}
Let
$$
\widehat{\mathcal{Q}}(k)=\sum_{i=1}^k\|X_iX_i^\top- \widehat{G}\|_F^2+\sum_{i=k+1}^n\|X_iX_i^\top-\widehat{H}\|_F^2 \quad \text { and } \quad \mathcal{Q}^*(k)=\sum_{i=1}^k\|X_iX_i^\top- G^*\|_F^2+\sum_{i=k+1}^n\|X_iX_i^\top- H^*\|_F^2 .
$$
Through out this section, we use $\kappa_{\Sigma} = \|G^*-H^*\|_F$ to measure the signal.
\bnlem[Refinement for regression]
Let
$$
\eta+r=\underset{k \in(0, n]}{\arg \max } \widehat{\mathcal{Q}}(k) .
$$
Then under the assumptions above, it holds that
$$
\kappa_{\Sigma}^2 r=O_P(\log(n)) .
$$
\enlem
\bprf
By assumptions above, we have
$$
\frac{d^{5/2} \log ^{3 / 2}(nd)}{\sqrt{n}} \rightarrow 0, \quad \frac{d^2 \log ^{3 / 2}(nd)}{n \kappa_{\Sigma}} \rightarrow 0, \quad \frac{d \log ^{3 / 2}(nd)}{\sqrt{n} \kappa_{\Sigma}} \rightarrow 0, \quad \frac{d \log (nd)}{n \kappa_{\Sigma}^2} \rightarrow 0 .
$$
Without loss of generality, suppose $r \geq 0$. Since $\eta+r$ is the minimizer, it follows that
$$
\widehat{\mathcal{Q}}(\eta+r) \leq \widehat{\mathcal{Q}}(\eta) .
$$
If $r \leq C\frac{\log(n)}{\kappa_{\Sigma}^2}$, then there is nothing to show. So for the rest of the argument, for contradiction, assume that
$$
r \geq C\frac{\log(n)}{\kappa_{\Sigma}^2}
$$
Observe that
$$
\begin{aligned}
\widehat{\mathcal{Q}}(t)-\widehat{\mathcal{Q}}(\eta) &=\sum_{i=\eta+1}^{\eta+r}\|X_iX_i^\top- \widehat{G}\|_F^2-\sum_{i=\eta+1}^{\eta+r}\|X_iX_i^\top- \widehat{H}\|_F^2 \\
\mathcal{Q}^*(t)-\mathcal{Q}^*(\eta) &=\sum_{i=\eta+1}^{\eta+r}\|X_iX_i^\top- {G}^*\|_F^2-\sum_{i=\eta+1}^{\eta+r}\|X_iX_i^\top-{H}^*\|_F^2
\end{aligned}
$$
\textbf{Step 1}. It follows that
$$
\begin{aligned}
& \sum_{i=\eta+1}^{\eta+r}\|X_iX_i^\top- \widehat{G}\|_F^2-\sum_{i=\eta+1}^{\eta+r}\|X_iX_i^\top- {G}^*\|_F^2 \\
=& \sum_{i=\eta+1}^{\eta+r}\|\widehat{G}- G^*\|_F^2+2\left\langle G^*-\widehat{G}, \sum_{i=\eta+1}^{\eta+r}(X_iX_i^\top-G^*)\right\rangle \\
=& r\|\widehat{G}- G^*\|_F^2+2r \left\langle G^* -\widehat{G}, H^*-G^*\right\rangle +2\left\langle G^*-\widehat{G}, \sum_{i=\eta+1}^{\eta+r}(X_iX_i^\top -H^*)\right\rangle
\end{aligned}
$$
By assumptions, we have
$$
r\|\widehat{G}- G^*\|_F^2 =O_p\left(r \frac{d^2 \log (nd)}{n}\right) \\
=o_p\left(r \kappa_{\Sigma}^2\right).
$$
Similarly
$$
\left\langle G^* -\widehat{G}, H^*-G^*\right\rangle\leq r\|G^* -\widehat{G}\|_F\| H^*-G^* \|_F \leq
O_p\left(r\kappa_{\Sigma} d\sqrt{\frac{ \log (nd)}{n} } \right)=o_p\left(r \kappa_{\Sigma}^2\right)
$$
where the second equality follows from $\|G^*-H^*\|_2=\kappa_{\Sigma}$, and the last equality follows from \eqref{op1_eq:cov snr}. In addition,
$$
\begin{aligned}
&\left\langle G^*-\widehat{G}, \sum_{i=\eta+1}^{\eta+r}(X_iX_i^\top -H^*)\right\rangle \leq\| G^*-\widehat{G}\|_F\|\sum_{i=\eta+1}^{\eta+r}(X_iX_i^\top -H^*)\|_{F} \\
=& O_p\left(d \sqrt{\frac{\log (nd)}{n}}\right) O_p(d\sqrt{r\log (nd)}+ d^{3/2}\log (nd))=O_p(\kappa_{\Sigma} \sqrt{r})+O_p(1)
\end{aligned}
$$
Therefore
$$
\sum_{i=\eta+1}^{\eta+r}\|X_iX_i^\top- \widehat{G}\|_F^2-\sum_{i=\eta+1}^{\eta+r}\|X_iX_i^\top- {G}^*\|_F^2=O_p(\kappa_{\Sigma} \sqrt{r})+O_p(1)+o_p\left(r \kappa_{\Sigma}^2\right) .
$$
\textbf{Step 2}. Using the same argument as in the previous step, it follows that
$$
\sum_{i=\eta+1}^{\eta+r}\|X_iX_i^\top- \widehat{H}\|_F^2-\sum_{i=\eta+1}^{\eta+r}\|X_iX_i^\top- {H}^*\|_F^2=O_p(\kappa_{\Sigma} \sqrt{r})+O_p(1)+o_p(r \kappa_{\Sigma}^2) .
$$
Therefore
\begin{equation}
    \left|\widehat{\mathcal{Q}}(\eta+r)-\widehat{\mathcal{Q}}(\eta)-\left\{\mathcal{Q}^*(\eta+r)-\mathcal{Q}^*(\eta)\right\}\right|=O_p(\kappa_{\Sigma} \sqrt{r})+O_p(1)+o_p\left(r \kappa_{\Sigma}^2\right)
    \label{tmp_eq:op1 cov main prop eq 1}
\end{equation}
\textbf{Step 3}. Observe that
$$
\begin{aligned}
\mathcal{Q}^*(\eta+r)-\mathcal{Q}^*(\eta) 
=&\sum_{i=\eta+1}^{\eta+r}\|X_iX_i^\top- {G}^*\|_F^2-\sum_{i=\eta+1}^{\eta+r}\|X_iX_i^\top- {H}^*\|_F^2 \\
=& r\| G^*- H^*\|_F^2-2 \left\langle H^*- G^*, \sum_{i=\eta+1}^{\eta+r}(X_iX_i^\top- H^*) \right\rangle
\end{aligned}
$$
Denote $D^* = H^*- G^*$, then we can write the noise term as
$$
\left\langle H^*- G^*, X_iX_i^\top- H^* \right\rangle = X_i^\top D^* X_i - \mathbb{E}[X_i^\top D^* X_i].
$$
Since $X_i$'s are Gaussian, denote $\Sigma_{i} = \mathbb{E}[X_iX_i^\top] =U_i^\top \Lambda_i U_i$, then
$$
\left\langle H^*- G^*, \sum_{i=\eta+1}^{\eta+r}(X_iX_i^\top- H^*) \right\rangle = Z^\top \tilde{D} Z^\top - \mathbb{E}[Z^\top \tilde{D} Z^\top],
$$
where $Z\in \mathbb{R}^{rd}$ is a standard Gaussian vector and 
$$
\tilde{D} = {\rm diag}\{U_1D^*U_1^\top,U_2D^*U_2^\top,\cdots, U_r D^*U_r^\top\}.
$$
Therefore, by Hanson-Wright inequality, uniformly for all $r\geq C\frac{\log(n)}{\kappa_{\Sigma}^2}$ it holds that
\begin{equation}
    \mathcal{Q}^*(\eta+r)-\mathcal{Q}^*(\eta) \leq r \kappa_{\Sigma}^2 + O_P(\|X\|_{\psi_2}^2\sqrt{r}\kappa_{\Sigma}\log(r\kappa_{\Sigma}^2)),
\label{tmp_eq:op1 cov main prop eq 2}
\end{equation}

\textbf{Step 4}. \Cref{tmp_eq:op1 cov main prop eq 1} and \Cref{tmp_eq:op1 cov main prop eq 2} together give, uniformly for all $r \geq C\log(n) / \kappa_{\Sigma}^2$,
$$
 r \kappa_{\Sigma}^2+O_P(\|X\|_{\psi_2}^2\sqrt{r}\kappa_{\Sigma}\log(r\kappa_{\Sigma}^2)) \leq O_p(\kappa_{\Sigma} \sqrt{r})+O_p(1)+o_p\left(r \kappa_{\Sigma}^2\right),
$$
which leads to contradiction and thus proves that
$$
r \kappa_{\Sigma}^2=O_P(\log(n)).
$$
\eprf



\bnlem
\label{lem:estimation covariance}
Let $\{X_i\}_{i\in [n]}$ be a sequence of subgaussian vectors in $\mathbb{R}^{d}$ with orlitz norm upper bounded $\|X\|_{\psi_2}<\infty$. Suppose $\mathbb{E}[X_i] = 0$ and $\mathbb{E}[X_iX_i^\top] = \Sigma$ for $i\in [n]$. Let $\widehat{\Sigma}_{n} = \frac{1}{n}\sum_{i \in [n]} X_i X_i^\top$. Then for any $u>0$, it holds with probability at least $1 - \exp(-u)$ that
\begin{equation}
    \|\widehat{\Sigma}_{n} - \Sigma\|_2\lesssim \|X\|_{\psi_2}^2(\sqrt{\frac{d + u}{n}}\vee \frac{d + u}{n}).
\end{equation}
\enlem




\bnlem[Hanson-Wright inequality]
Let $X=\left(X_1, \ldots, X_n\right) \in \mathbb{R}^n$ be a random vector with independent, mean zero, sub-gaussian coordinates. Let $A$ be an $n \times n$ matrix. Then, for every $t \geq 0$, we have
$$
\mathbb{P}\left\{\left|X^{\top} A X-\mathbb{E} X^{\top} A X\right| \geq t\right\} \leq 2 \exp \left[-c \min \left(\frac{t^2}{K^4\|A\|_F^2}, \frac{t}{K^2\|A\|}\right)\right],
$$
where $K=\max _i\left\|X_i\right\|_{\psi_2}$
\enlem








\clearpage
\subsubsection{Regression}
\label{sec:regression op1}
Suppose
$$
y_i=\left\{\begin{array}{ll}
X_i^{\top} \alpha^*+\epsilon_i & \text { when } i \in(0, \eta] \\
X_i^{\top} \beta^*+\epsilon_i & \text { when } i \in(\eta, n]
\end{array} .\right.
$$
In addition, suppose that there exists $\theta \in(0,1)$ such that $\eta=\lfloor n \theta\rfloor$ and that $\left|\alpha^*-\beta^*\right|_2=\kappa<\infty$. Suppose that $\left\|\alpha^*\right\|_0 \leq \mathfrak{s},\left\|\beta^*\right\|_0 \leq \mathfrak{s}$ and that
\begin{equation}
    \frac{\mathfrak{s} \log ^{3 / 2}(p)}{\sqrt{n}} \rightarrow 0, \quad \frac{\mathfrak{s}^2 \log ^{3 / 2}(p)}{n \kappa} \rightarrow 0, \quad \frac{\mathfrak{s} \log ^{3 / 2}(p)}{\sqrt{n} \kappa} \rightarrow 0, \quad \frac{\mathfrak{s} \log (p)}{n \kappa^2} \rightarrow 0.
    \label{op1_eq:regression snr}
\end{equation}
Suppose there exists $\widehat{\alpha}$ and $\widehat{\beta}$ such that
\begin{align*}
  & \|\widehat{\alpha}-\alpha^*\|_2^2=O_p\left(\frac{\mathfrak{s} \log (p)}{n}\right) \text{ and } \|\widehat{\alpha}-\alpha^*\|_1=O_p\left(\mathfrak{s} \sqrt{\frac{\log (p)}{n}}\right); \\
& \|\widehat{\beta}-\beta^*\|_2^2=O_p\left(\frac{\mathfrak{s} \log (p)}{n}\right) \text{ and } \|\widehat{\beta}-\beta^*\|_1=O_p\left(\mathfrak{s} \sqrt{\frac{\log (p)}{n}}\right).
\end{align*}
Let
$$
\widehat{\mathcal{Q}}(k)=\sum_{i=1}^k\left(y_i-X_i^{\top} \widehat{\alpha}\right)^2+\sum_{i=k+1}^n\left(y_i-X_i^{\top} \widehat{\beta}\right)^2 \quad \text { and } \quad \mathcal{Q}^*(k)=\sum_{i=1}^k\left(y_i-X_i^{\top} \alpha^*\right)^2+\sum_{i=k+1}^n\left(y_i-X_i^{\top} \beta^*\right)^2 .
$$

\bnlem[Refinement for regression]
Let
$$
\eta+r=\underset{k \in(0, n]}{\arg \max } \widehat{\mathcal{Q}}(k) .
$$
Then under the assumptions above, it holds that
$$
\kappa^2 r=O_p(1) .
$$
\enlem
\bprf
By assumptions above, we have
$$
\frac{\mathfrak{s} \log ^{3 / 2}(p)}{\sqrt{n}} \rightarrow 0, \quad \frac{\mathfrak{s}^2 \log ^{3 / 2}(p)}{n \kappa} \rightarrow 0, \quad \frac{\mathfrak{s} \log ^{3 / 2}(p)}{\sqrt{n} \kappa} \rightarrow 0, \quad \frac{\mathfrak{s} \log (p)}{n \kappa^2} \rightarrow 0 .
$$
Without loss of generality, suppose $r \geq 0$. Since $\eta+r$ is the minimizer, it follows that
$$
\widehat{\mathcal{Q}}(\eta+r) \leq \widehat{\mathcal{Q}}(\eta) .
$$
If $r \leq \frac{1}{\kappa^2}$, then there is nothing to show. So for the rest of the argument, for contradiction, assume that
$$
r \geq \frac{1}{\kappa^2}
$$
Observe that
$$
\begin{aligned}
\widehat{\mathcal{Q}}(t)-\widehat{\mathcal{Q}}(\eta) &=\sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \widehat{\alpha}\right)^2-\sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \widehat{\beta}\right)^2 \\
\mathcal{Q}^*(t)-\mathcal{Q}^*(\eta) &=\sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \alpha^*\right)^2-\sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \beta^*\right)^2
\end{aligned}
$$
\textbf{Step 1}. It follows that
$$
\begin{aligned}
& \sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \widehat{\alpha}\right)^2-\sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \alpha^*\right)^2 \\
=& \sum_{i=\eta+1}^{\eta+r}\left(X_i^{\top} \widehat{\alpha}-X_i^{\top} \alpha^*\right)^2+2\left(\widehat{\alpha}-\alpha^*\right)^{\top} X_i \sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \alpha^*\right) \\
=& \sum_{i=\eta+1}^{\eta+r}\left(X_i^{\top} \widehat{\alpha}-X_i^{\top} \alpha^*\right)^2+2\left(\widehat{\alpha}-\alpha^*\right)^{\top} \sum_{i=1}^r X_i X_i^{\top}\left(\beta^*-\alpha^*\right)+2\left(\widehat{\alpha}-\alpha^*\right)^{\top} \sum_{i=\eta+1}^{\eta+r} X_i \epsilon_i
\end{aligned}
$$
By \Cref{lem:regression op1 base lemma 1}, uniformly for all $r$,
$$
\left\|\frac{1}{r} \sum_{i=1}^r X_i X_i^{\top}-\Sigma\right\|_{\infty} \geq O_p\left(\sqrt{\frac{\log (p)}{r}}+\frac{\log (p)}{r}\right) .
$$
Therefore
$$
\begin{aligned}
\sum_{i=\eta+1}^{\eta+r}\left(X_i^{\top} \widehat{\alpha}-X_i^{\top} \alpha^*\right)^2 &=\sum_{i=\eta+1}^{\eta+r}\left(\widehat{\alpha}-\alpha^*\right)^{\top} \sum_{i=1}^r\left\{X_i X_i^{\top}-\Sigma\right\}\left(\widehat{\alpha}-\alpha^*\right)+r\left(\widehat{\alpha}-\alpha^*\right)^{\top} \Sigma\left(\widehat{\alpha}-\alpha^*\right) \\
& \leq\|\widehat{\alpha}-\alpha^*\|_1^2\left\|\sum_{i=1}^r X_i X_i^{\top}-\Sigma\right\|_{\infty}+\Lambda_{\max } r\|\widehat{\alpha}-\alpha^*\|_2^2\\
&=O_p\left(\frac{\mathfrak{s}^2 \log (p)}{n}\right)O_p(\sqrt{r \log (p)}+\log (p))+O_p\left(r \frac{\mathfrak{s} \log (p)}{n}\right) \\
&=O_p\left(\sqrt{r \kappa^2}\right)+O_p(1)+o_p\left(r \kappa^2\right)
\end{aligned}
$$
where the inequality follows from \Cref{lem:regression op1 base lemma 1} and last equality follows from assumption \eqref{op1_eq:regression snr}. Similarly
$$
\begin{aligned}
\left(\widehat{\alpha}-\alpha^*\right)^{\top} \sum_{i=1}^r X_i X_i^{\top}\left(\beta^*-\alpha^*\right) &=\left(\widehat{\alpha}-\alpha^*\right)^{\top} \sum_{i=1}^r\left\{X_i X_i^{\top}-\Sigma\right\}\left(\beta^*-\alpha^*\right)+r\left(\widehat{\alpha}-\alpha^*\right)^{\top} \Sigma\left(\beta^*-\alpha^*\right) \\
& \leq \|\widehat{\alpha}-\alpha^*\|_1\|\left(\beta^*-\alpha^*\right)^{\top}\left\{\sum_{i=1}^r X_i X_i^{\top}-\Sigma\right\}\|_{\infty}+\Lambda_{\max } r\|\widehat{\alpha}-\alpha^*\|_2\|\beta^*-\alpha^*\|_2 \\
&=O_p\left(\mathfrak{s} \sqrt{\frac{\log (p)}{n}}\right) O_p(\kappa\{\sqrt{r \log (p)}+\log (p)\})+O_p\left(r\kappa \sqrt{\frac{\mathfrak{s} \log (p)}{n} } \right).\\
&=O_p(\kappa \sqrt{r})+O_p(1)+o_p\left(r \kappa^2\right)
\end{aligned}
$$
where the second equality follows from $\|\beta^*-\alpha^*\|_2=\kappa$ and \Cref{lem:regression op1 base lemma 2}, and the last equality follows from \eqref{op1_eq:regression snr}. In addition,
$$
\begin{aligned}
&\left(\widehat{\alpha}-\alpha^*\right)^{\top} \sum_{i=\eta+1}^{\eta+r} X_i \epsilon_i \leq\|\widehat{\alpha}-\alpha^*\|_1\|\sum_{i=\eta+1}^{\eta+r} X_i \epsilon_i\|_{\infty} \\
=& O_p\left(\mathfrak{s} \sqrt{\frac{\log (p)}{n}}\right) O_p(\sqrt{r \log (p)}+\log (p))=O_p(\kappa \sqrt{r})+O_p(1)
\end{aligned}
$$
where the second equality follows from \Cref{lem:regression op1 base lemma 1}. Therefore
$$
\sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \widehat{\alpha}\right)^2-\sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \alpha^*\right)^2=O_p(\kappa \sqrt{r})+O_p(1)+o_p\left(r \kappa^2\right) .
$$
\textbf{Step 2}. Using the same argument as in the previous step, it follows that
$$
\sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \widehat{\beta}\right)^2-\sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \beta^*\right)^2=O_p(\kappa \sqrt{r})+O_p(1)+o_p\left(r \kappa^2\right) .
$$
Therefore
\begin{equation}
    \left|\widehat{\mathcal{Q}}(\eta+r)-\widehat{\mathcal{Q}}(\eta)-\left\{\mathcal{Q}^*(\eta+r)-\mathcal{Q}^*(\eta)\right\}\right|=O_p(\kappa \sqrt{r})+O_p(1)+o_p\left(r \kappa^2\right)
    \label{tmp_eq:op1 regression main prop eq 1}
\end{equation}
\textbf{Step 3}. Observe that
$$
\begin{aligned}
& \mathcal{Q}^*(\eta+r)-\mathcal{Q}^*(\eta) \\
=& \sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \alpha^*\right)^2-\sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \beta^*\right)^2 \\
=& \sum_{i=\eta+1}^{\eta+r}\left(X_i^{\top} \alpha^*-X_i^{\top} \beta^*\right)^2-2 \sum_{i=\eta+1}^{\eta+r}\left(y_i-X_i^{\top} \beta^*\right)\left(X_i^{\top} \alpha^*-X_i^{\top} \beta^*\right) \\
=& \sum_{i=\eta+1}^{\eta+r}\left(\alpha^*-\beta^*\right)^{\top}\left\{X_i^{\top} X_i-\Sigma\right\}\left(\alpha^*-\beta^*\right)+r\left(\alpha^*-\beta^*\right)^{\top} \Sigma\left(\alpha^*-\beta^*\right)-2 \sum_{i=\eta+1}^{\eta+r} \epsilon_i\left(X_i^{\top} \alpha^*-X_i^{\top} \beta^*\right)
\end{aligned}
$$
Note that
$$
z_i=\frac{1}{\kappa^2}\left(\alpha^*-\beta^*\right)^{\top}\left\{X_i^{\top} X_i-\Sigma\right\}\left(\alpha^*-\beta^*\right)
$$
is a sub-exponential random variable with bounded $\psi_1$ norm. Therefore by \Cref{lem:subexp uniform loglog law}, uniformly for all $r \geq 1 / \kappa^2$,
$$
\sum_{i=1}^r z_i=O_p\left(\sqrt{r\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right) .
$$
Since $\kappa<\infty$, it follows that
$$
\sum_{i=\eta+1}^{\eta+r}\left(\alpha^*-\beta^*\right)^{\top}\left\{X_i^{\top} X_i-\Sigma\right\}\left(\alpha^*-\beta^*\right)=O_p\left(\sqrt{r \kappa^2\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right)
$$
Similarly, let
$$
w_i=\frac{1}{\kappa} \epsilon_i\left(X_i^{\top} \alpha^*-X_i^{\top} \beta^*\right)
$$
Then $\left\{w_i\right\}_{i=1}^{\infty}$ are sub-exponential random variables with bounded $\psi_1$ norm. Therefore by \Cref{lem:subexp uniform loglog law}, uniformly for all $r \geq 1 / \kappa^2$,
$$
\sum_{i=1}^r w_i=O_p\left(\sqrt{r\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right)
$$
Since $\kappa<\infty$, it follows that
$$
\sum_{i=\eta+1}^{\eta+r} \epsilon_i\left(X_i^{\top} \alpha^*-X_i^{\top} \beta^*\right)=O_p\left(\sqrt{r \kappa^2\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right)
$$
Therefore
\begin{equation}
    \mathcal{Q}^*(\eta+r)-\mathcal{Q}^*(\eta) \geq \Lambda_{\min } r \kappa^2+O_p\left(\sqrt{r \kappa^2\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right)
\label{tmp_eq:op1 regression main prop eq 2}
\end{equation}
where $\Lambda_{\min }$ is the minimal eigenvalue of $\Sigma$.

\textbf{Step 4}. \Cref{tmp_eq:op1 regression main prop eq 1} and \Cref{tmp_eq:op1 regression main prop eq 1} together give, uniformly for all $r \geq 1 / \kappa^2$,
$$
\Lambda_{\min } r \kappa^2+O_p\left(\sqrt{r \kappa^2\left\{\log \log \left(\kappa^2 r\right)+1\right\}}+\sqrt{r \kappa^2}\left\{\log \log \left(\kappa^2 r\right)+1\right\}\right) \leq O_p(\kappa \sqrt{r})+O_p(1)+o_p\left(r \kappa^2\right)
$$
This implies that
$$
r \kappa^2=O_p(1)
$$
\eprf


\bnlem
\label{lem:regression op1 base lemma 1}
Suppose $\left\{X_i\right\}_{i=1}^n \stackrel{i . i . d}{\sim} N_p(0, \Sigma)$ and $\left\{\epsilon_i\right\}_{i=1}^n \stackrel{i i . d}{\sim} N\left(0, \sigma^2\right)$. Then it holds that
$$
\begin{aligned}
&\mathbb{P}\left(\|\frac{1}{r} \sum_{i=1}^r X_i X_i^{\top}-\Sigma\|_{\infty} \geq C_1\left(\sqrt{\frac{\log (p)}{r}}+\frac{\log (p)}{r}\right) \text { for all } 1 \leq r \leq n\right) \leq n^{-2}, \\
&\mathbb{P}\left(\|\frac{1}{r} \sum_{i=1}^r X_i \epsilon_i\|_{\infty} \geq C_2\left(\sqrt{\frac{\log (p)}{r}}+\frac{\log (p)}{r}\right) \text { for all } 1 \leq r \leq n\right) \leq n^{-2}
\end{aligned}
$$
\enlem
\bprf
Proof. For the first probability bound, observe that for any $j, k \in[1, \ldots, p], X_j X_k-\Sigma_{j k}$ is subexponential random variable. Therefore for any $r>0$,
$$
\mathbb{P}\left\{\left|\frac{1}{r} \sum_{i=1}^r X_{i j} X_{i k}-\Sigma_{j k}\right| \geq x\right\} \leq \exp \left(-r c_1 x^2\right)+\exp \left(-r c_2 x\right)
$$
So
$$
\mathbb{P}\left\{\left\|\frac{1}{r} \sum_{i=1}^r X_{i j} X_{i k}-\Sigma_{j k}\right\|_{\infty} \geq x\right\} \leq p \exp \left(-r c_1 x^2\right)+p \exp \left(-r c_2 x\right) .
$$
This gives, for sufficiently large $C_1>0$,
$$
\mathbb{P}\left\{\left\|\frac{1}{r} \sum_{i=1}^r X_{i j} X_{i k}-\Sigma_{j k}\right\|_{\infty} \geq C_1\left(\sqrt{\frac{\log (p n)}{r}}+\frac{\log (p n)}{r}\right)\right\} \leq n^{-3} .
$$
By a union bound,
$$
\mathbb{P}\left\{\left\|\frac{1}{r} \sum_{i=1}^r X_{i j} X_{i k}-\Sigma_{j k}\right\|_{\infty} \geq C_1\left(\sqrt{\frac{\log (p n)}{r}}+\frac{\log (p n)}{r}\right) \text { for all } 1 \leq r \leq n\right\} \leq n^{-2}
$$
The desired result follows from the assumption that $p \geq n^\alpha$. The second probability bound follows from the same argument and therefore is omitted for brevity.
\eprf




\bnlem
\label{lem:regression op1 base lemma 2}
 Suppose $\left\{X_i\right\}_{i=1}^n \stackrel{2.2 . d}{\sim} N_p(0, \Sigma)$ and $u \in \mathbb{R}^p$ is a deterministic vector such that $|u|_2=1$. Then it holds that
$$
\mathbb{P}\left(\|u^{\top}\left\{\frac{1}{r} \sum_{i=1}^r X_i X_i^{\top}-\Sigma\right\}\|_{\infty} \geq C_1\left(\sqrt{\frac{\log (p)}{r}}+\frac{\log (p)}{r}\right) \text { for all } 1 \leq r \leq n\right) \leq n^{-2} .
$$
\enlem
\bprf
For fixed $j \in[1, \ldots, p]$, let
$$
z_i=u^{\top} X_i X_{i j}-u^{\top} \Sigma_{\cdot j},
$$
where $\Sigma_{\cdot j}$ denote the $j$-th column of $\Sigma$. Note that $z_i$ is a sub-exponential random variable with bounded $\psi_1$ norm. The desired result follows from the same argument as \Cref{lem:regression op1 base lemma 1}.
\eprf









==> backup_version/06_discussion.tex <==
\section{Discussion}
\label{sec:discussion}
